STI: Turbocharge NLP Inference at the Edge via Elastic Pipelining

Natural Language Processing (NLP) inference is seeing increasing adoption by mobile applications, where on-device inference is desirable for crucially preserving user data privacy and avoiding network roundtrips. Yet, the unprecedented size of an NLP model stresses both latency and memory, creating a tension between the two key resources of a mobile device. To meet a target latency, holding the whole model in memory launches execution as soon as possible but increases one app's memory footprints by several times, limiting its benefits to only a few inferences before being recycled by mobile memory management. On the other hand, loading the model from storage on demand incurs IO as long as a few seconds, far exceeding the delay range satisfying to a user; pipelining layerwise model loading and execution does not hide IO either, due to the high skewness between IO and computation delays. To this end, we propose Speedy Transformer Inference (STI). Built on the key idea of maximizing IO/compute resource utilization on the most important parts of a model, STI reconciles the latency v.s. memory tension via two novel techniques. First, model sharding. STI manages model parameters as independently tunable shards, and profiles their importance to accuracy. Second, elastic pipeline planning with a preload buffer. STI instantiates an IO/compute pipeline and uses a small buffer for preload shards to bootstrap execution without stalling at early stages; it judiciously selects, tunes, and assembles shards per their importance for resource-elastic execution, maximizing inference accuracy. Atop two commodity SoCs, we build STI and evaluate it against a wide range of NLP tasks, under a practical range of target latencies, and on both CPU and GPU. We demonstrate that STI delivers high accuracies with 1-2 orders of magnitude lower memory, outperforming competitive baselines.

==> contrib.tex <==
% !TeX root = main.tex

\section{Contributions}

The proposed project makes the following contributions:
\begin{myitemize}
	\item 
	It will identify and characterize the cold start inference problem on multiple platforms;
	it will obtain diverse IO/Compute profiles measured on real hardwares, such as Odroid~\cite{odroid-web}, Raspberry Pi~\cite{rpi3-web}, and Beagleboard X15~\cite{x15-web}.

	
	\item 
	A novel system design for accelerating \tfm{} cold start inference of pretrained models on edge devices.
	It features two novel techniques: 
	1) \textit{structured model sharding}, which partitions the whole pretrained model into multiple attention heads, quantized into different bitwidths;
	2) \textit{device heterogeneity-aware shard planning}, which schedules shards for both low latency and maximum accuracy, based on the specific IO/Compute profile of the hardware and a deadline.
	
	\item
	The implementation and evaluation of the proposed system.
	It will evaluate the system on the pretrained  BERT~\cite{bert} model using the GLUE benchmark suite~\cite{glue-benchmark}.
	The implementation will be made open-source to facilitate future research on the cold start inference problem. 
	
%	\begin{itemize}
%		\item 
%		Pipelining 
%		
%		\item 
%		Deadline-driven dynamic bitwidth selection for encoder layers. 
%		
%		\item 
%		Hierarchical word embedding cache layers. 
%	\end{itemize}
%	Backing the techniques is a co-designed system memory management layer.. 
%	Compared with the vanilla page cache, it is model aware and finer grained: at the granularity of an attention head instead of whole model file; 
%	cache replacement strategy is pipeline-aware...
%	
%	\item 
%	Case studies of \sys{} on a wide range of devices that have diverse hardware characteristics. 
	
\end{myitemize}


%\paragraph{Key ideas.}
%To address the above challenges, we propose \sys{}, a novel transformer-OS co-design.
%The mechanism is as follows.
%\begin{myenumerate}
%	\item
%	Hierarchical, frequency-based word embedding storage. 
%	To start as soon as possible, \sys{} caches XXX most recently used word embeddings in memory ($<1\%$, XXX KB) (Zipf law), and clusters the rest based on their frequency.
%	\sys{} stores each cluster in a number sequential disk blocks (XXX MB, XXX words), which minimizes the loading latency for the platform\Note{platform aware...}.
%	The hierarchical embedding reduces the latency by XX\%.
%	
%	
%	\item 
%	Progressive(evolutionary) weight sharing. 
%	During cold inference, \sys{} only loads one transformer layer, whose parameters are shared across all others, inspired by~\cite{albert};
%	upon each future inference, \sys{} loads one more transformer layer by overlapping its IO with compute on existing, loaded, and shared layers.  
%	Such a model can be viewed as supernet of $N$ transformer layers, which consists of $N$ subnets, each of 1 to $N$ distinct layers.
%	
%	
%	\item 
%	Layer-aware page caching.
%	To support \sys{}, we specialize kernel memory management. 
%	It unifies the model file \textit{with} flatten/loaded model parameters\Note{XXX:forecast double copy}, making them a unified copy;
%	instead of caching the model file as a whole, it caches individual transformer layers. 
%	Doing so saves XXX\% memory during inference. 
%\end{myenumerate}


==> design-bert.tex <==
% !TeX root = main.tex

\subsection{Progressive BERT}


The key idea is 1) to progressively load a BERT model from the smallest to the full one, and 2) to start inference as soon as possible by overlapping an IO task with Compute.

\subsubsection{Key challenges.}
The design raises following challenges:
\begin{myenumerate}
	\item 
	\textit{How to decide an IO/Compute task?}
%	\textit{How to avoid starvation?}
	It is crucial to pipeline efficiency. 
	Displacement of IO/Compute task (e.g. layerwise) leads to starvation and poor performance, as discussed in \sect{motiv:design-explore}. 
%	The problem is high IO/Compute ratio (as high as 10:1, shown in \sect{motiv:char}), which leads to starvation. 
	The ratio needs at least to be close for an effective overlap.

	
	\item 
	\textit{How to cater to different platforms?}
	IO vs Compute ratio is platform-specific, especially for mobile devices which have diverse hardware.
	A universal pipelining strategy cannot fit the different nature of mobile devices. 

	\item
	\textit{How to progressively load parameters?}
	\Note{how to train such a model...}
	The key of our design is weights from sub-trasnformers can be used to collectively and progressively to create a larger super-transformer. 
\end{myenumerate}

\subsubsection{Solutions.}

To address the above challenges, our ideas are as follows. 

\paragraph{Pipelining Transformer slice.}
We set to use an attention head and the slice of its underlying FFN, a \textit{slice} of a transfomer block, as the IO/Compute task.
We pipeline the slice instead of whole layers.
Our rationals are as follows:
\begin{myenumerate}
	\item 
	The slice is finer grained, offering has a much closer IO/Compute gap. 
	\Note{More importantly,} Compute scales much slower than IO.
	For instance, compute on 1 slice vs 5 slices only leads to XX\% increase, which is still closer than IO of 1 slice\Note{need a figure}. 
	This allows us to approximate pipelining strategy on different hardwares. 

	\item 
	Attention heads have been shown to have high redundancy\cite{16heads};
	weight sharing of them all is promising~\cite{albert}.
	This gives us assurance on performance during cold inference, even at the first inference when only one attention head is used. 
\end{myenumerate}

Formally, we define the \textit{slice} as follows:
a (vertical) slice of a transformer block consists of a single attention head of \Note{XXX} dimensions as specified in BERT~\cite{bert}, and the corresponding FFNs of 256 neurons (one twelve-th of 3076 dimensions). 


\paragraph{IO/Compute-adaptive pipelining strategy.}
This is to have an high-overlapping pipeline, adaptive to different hardwares of mobile devices. 
\sys{} profiles the IO and Compute time of a whole vertical slice defined above, then the IO and Compute for FFN of the slice. 
Due to the careful selection, the IO/Compute ratio is in the same magnitude or very close to each other;
from our measurement the ratio varies between \Note{XXX-YYY}.
For instance, it is 1:1 on Odroid.
\sys{} hence adaptively pipelines w.r.t three difference cases: 
\begin{myenumerate}
	\item 
	$IO = Compute$: 
	close enough ratio, \Note{e.g. 1:1 - 2:1}. 
	Pipeline the following: Compute of the \textit{current} loaded vertical slice with IO of \textit{next} to be loaded vertical slice.
	
	\item
	$IO < Compute$:
	\Note{range is ???}
	Pipeline:  Compute of \textit{current} loaded vertical slice with IO of \textit{next} $n$ vertical slices.
	The goal is not to starve IO;
	the $n$ depends on actual  
	
	\item 
	$IO > Compute$:
	\Note{range is XXX}.
	Pipeline: Compute of \textit{current} loaded vertical slice with IO of \textit{next} FFN, while reusing attention from previous slice. 
	The rational is stated before -- redundancy of attention heads makes weight sharing possible. 
\end{myenumerate}

From the three different cases, \sys{} produces the pipelining strategy for individual mobile devices of different IO/Compute ratio, based on the profile of a transfomer slice. 

\paragraph{Progressive Bert SuperTransformer.}
Our Progressive Bert \textit{Super}Transformer has the same architecture as BERT: 12 layers in total, each transformer layer contains \Note{XXX} attention heads, each of XXX dimensions, and 3076 hidden dimensions for FFNs. 

Its key property is: 
each subTransformer is a slice of the superTransformer;
each inference only loads \textit{one extra} slice of the superTransformer, based on the pipelining strategy;
from cold to hot, multiple inferences compose the slices of a full superTransformer architecture which is BERT.

Advancement from the prior arts is how to collocate and unify the multiple pipelining (i.e. weight sharing) strategy under one superTransformer.
Recall HAT has fixed weight sharing of FFN but not attention; 
DynaBert has fixed weight sharing of attention but not FFN. 
Ours -- two different weight sharing strategies, determined by the hardware it runs on: 1) subTransformers do not share param, or 2) share attention \Note{what about share FFN}.


\textbf{Training methods.}
We adopt following training techniques from previous works.

\textbf{Ranking importance of attention heads.}
So that the most important attention head can be loaded as early as possible for cold inference accuracy. 

\textbf{Sampling FFNs.} 
Similar to Albert~\cite{albert}, HAT~\cite{hat}, LayerDrop~\cite{layerdrop}, for the subTransformers which \textit{may} or \textit{may not} share FFN layer, we randomly sample them to share weights during training time.
This helps smooth the parameter distribution in the resultant superTransformer.


\Note{merge below}
\paragraph{Key difference with existing techniques.}
\begin{myitemize}
	\item 
	\textbf{HAT.} hardware-aware, based on a latency goal. But fix the weight sharing strategy to all FFNs, front part of the embedding. 
	To load the next subTransformer, need re-load attention parameters, resulting in cold inference and long latency.
	
	\item 
	\textbf{DynaBert.} Can adjust width \& depth simultaneously. 
	Also does weight sharing of subtransformers, in terms of attention heads and FFN. 
	Can do attention-head-based pipelining. 
	But is not hardware-aware and has the fixed weight sharing strategy -- a special case when IO = Compute. 
	
	\item 
	\textbf{Ours.} Adaptive pipelining strategy -- different weight sharing mechanism w.r.t. different IO/Compute profiles on diverse hardwares, which is our key novelty.
\end{myitemize}


==> design-embedding.tex <==
% !TeX root = main.tex

\section{Confining disk IO of embeddings}
\xzlNote{become part of implementation}

\Note{highlight the uniqueness of word frequencies}
During cold inference, embedding lookup is blocking and slow. 
When untreated, it significantly reduces usable spare IO (\S\ref{sec:design:planning}), e.g. by XXX\%;
the compute might not have enough budgets, leading to inferior accuracy...

\sys{} reduces the disk IO of embedding, which is a key blocker during cold inference.
It does so by reducing both the total number of disk accesses (caching and embedding quantization), as well as access latency by turning slow, random accesses into fast, sequence ones.

\Note{merge below}
During cold inference, embedding lookup is blocking and slow. 
When untreated, it significantly reduces usable spare IO (\S\ref{sec:design:planning}), e.g. by XXX\%. 
To this end, \sys{} retrofits the known storage optimization techniques:
it quantizes them in low-bit (e.g. 3 bits), reducing their sizes by XX $\times$; 
it employs a small cache (5\% of total size) to absorb most accesses; 
it continuous updates their disk layout based on embedding frequency, optimizing for sequential access.

Embedding table -- a solved problem in storage + recommender system community~\cite{recssd, flashembedding, bandana}.
Likely due to embedding table is the major bottleneck for the community.


\subsection{A primer on embeddings}

In NLP, each word is represented by one embedding vector, usually of a few hundred dimensions (e.g. 768). 
The embedding table is a large lookup table storing all embedding vectors of the vocabulary, sizing from 30K to billions in commercial cloud...
Upon each new input (e.g. 128 words), inference engine looks up each vector in the table, and gather them into a tensor (e.g. $1x128x768$ for a single input) for \tfm{} consumption.


\subsection{Key challenges}


The goal is to reduce disk IO incurred by embedding look up, such that spare IO can be spent on compute for maximizing model accuracy.

We face the following challenges. 
\begin{myitemize}
	\item
	\textit{Embedding IO must block.}
	Inference must wait for aggregated embedding vectors to start.
	Yet, the embedding table constitutes one third of the total parameters, consequently taking over 1s to fully load.
	Meanwhile, it cannot be treated like encoder layer (e.g. pipelining by layers), because there is no compute to overlap because embedding table lookup is negligible compared with IO.
		
	\item 
	\textit{Slow random access.}
	Based on input, one may load individual word embeddings on-demand.
	However, each embedding vector contains 768x4 bytes, consuming a 4KB block.
	On-demand loading results in random 4K block accesses, which is an order of magnitude slower than sequential access (XXX vs YYY) on flash storage. 
\end{myitemize}

\subsection{Reducing disk IO size}

\paragraph{Quantize embeddings into low precisions}
As have been demonstrated in~\cite{binarybert,bibert,qbert} and will be further demonstrated by us in \sect{eval}, embedding layer can afford low-bit representations while having minimal impacts on model accuracy;
there is no need for mixed precision because ...

Therefore we quantize the embedding layer in fixed low-bit precision with the same technique described in~\sect{design:sharding:quantize};
we decide its precision based on sensitivity analysis presented in \sect{design:planning}.

This reduces the embedding vectors size by XX$\times$. 
As a result, a 4K disk block can locate XXX embedding vectors, reducing the block access by XXX$\times$.


\subsection{Catering to embedding access pattern}

For compulsory embedding cache misses, \sys{} reduces their disk access delays in the following ways.

\paragraph{Storing embeddings based on frequencies}
\sys{} adds a new frequency column to the existing embedding table, e.g. like a new dimension to each vector.
It stores the embedding table sorted by frequency on disk in contiguous blocks;
it bookkeeping the file offsets of each word, e.g. ``5-th word is stored at offset 1024'', such that words can be looked up individually.
Doing so ensures the spatial locality of disk accesses of embeddings~\cite{flashembedding,recssd} -- words of phrases are likely used together and shall be stored closely. 
For instance, pronouns such as ``I, you, he, she, they'', are likely to be used often, which may be followed by commonly used verbs such as ``eat, see, walk, run''.

During inferences, \sys{} keeps track of the frequencies of individual embedding vectors being used.
When the inference session ends (e.g. app being killed) or remain quiescent for a period (e.g. 60s), \sys{} updates the frequencies of the on-disk embedding table with new ones.
Meanwhile, \sys{} also updates their disk locations by sorting respective entries.
The procedure is brief and low-cost, as we will evaluate in XXX...

\paragraph{Buffered embedding read}
Upon new inputs, \sys{} collects all cache misses.
Instead of issuing lookups for each embedding in an adhoc manner, \sys{} buffers them, sorts them by their file offsets, and attempts to merge any adjacent reads.

For instance, individually reads file offset "4096, 0, 8192" may be translated into three discrete 4K block reads by the block layer. 
With the buffer, \sys{} merges them into one large read spanning three contiguous 4K disk blocks, greatly reducing the disk access delay.
\sect{eval} will present more evidence...

\Note{to merge}
\paragraph{A small embedding cache}
\sys{} employs an in-memory cache, which is a smaller embedding lookup table occupying a small portion of the whole embedding table (e.g. 5\%, only tens of KB);
for simplicity, \sys{} uses an LRU policy for cache eviction, which are effective on words embeddings~\cite{embedding-cache}.
The rationale is the power law (zipf law) of word frequency distribution~\cite{groupreduce,recssd,flashembedding}: XX\% of accesses happen to only YY\% of words.

As will be evaluated, the embedding cache absorbs most accesses, effectively reduces the disk accesses by XXX$\times$, leaving spare IO largely untapped...



==> design-mm.tex <==
% !TeX root = main.tex

\section{Managing model memory}


Model memory management in the background for resident model under different system pressure..
Resemble memory balloons in VM: deflate (downgrade) shards when sys memory pressure is high, inflate (upgrade) shards when memory pres. low...


\paragraph{Use cases}
\begin{myitemize}
	\item 
	Who cares? The system, not the user: 1) user is oblivious to resident model; 2) in the background, does not concern current inference (although it will concern \textit{next} inference) because ...  
	
	\item 
	APIs: Retrofit the ideas from balloon driver. Two primitives: inflate (upgrade)/deflate (downgrade), with one argument -- memory constraint, i.e. how much memory does the system expect the resident model to occupy?
\end{myitemize}



==> design-model.tex <==
% !TeX root = main.tex

\subsection{System model}

We target Arm SoCs capable of floating-point operations. 


==> design-sharding__Liwei_Guo_s_conflicted_copy_2022-07-05_.tex <==
% !TeX root = main.tex

\section{Elastic model sharding}
%\section{Managing the model in elastic shards}
%\section{Managing \Tfm{}s in fine elasticity}
%\section{Building an elastic IO/compute pipeline}
\label{sec:design:sharding}


%\textbf{Key points (structured around resident model):}1
%\begin{itemize}
%	\item 
%	Challenge: how to properly select a model shard? Must meet a list of criteria..
%	
%	\item
%	Model shards. Two things: partition by vertical slice (insights, formal definition), quantization technique (rationale, operation)
%	
%	\item
%	Resident model structure: in-memory representation, how to use, 
%	misc: activations (fixed high bits due to small, negligible).
%\end{itemize}


\xzlNote{moved here, to merge}
where each shard spans one Transformer attention head and $1/M$ FFN neurons of this layer. 
For each shard, it creates $K$ fidelity versions, which are lower-bit representations of this shard's weights. 
For instance, a full-fidelity version that represents each weight with 32 bits, a two-bit version that does so with 2 bits. 
We therefore store $NxMxK$ shard versions on disk. 
The preprocessing is a one-time effort per model; being light transformation of an existing model without pre-training, it can be done on device at the model installation time. 



%The preprocessing is a one-time effort per model; 
%lightweight and requiring no model re-retraining, it can be done on mobile devices. 


\Note{Model shards trade inexpensive disk storage for expensive, scarce memory... }


\subsection{Key challenges}
%\Note{merge challenges to below}
%We solve a key challenge in constructing a resident model: how to choose the proper parameter composition of a shard? %(as a smallest tunable unit for resident model)? 
%We solve a key challenge in constructing a resident model: how to instantiate a model shard? %(as a smallest tunable unit for resident model)? 
%We solve a key challenge: how to instantiate an elastic shard? %(as a smallest tunable unit for resident model)? 
We solve a key challenge: how to partition the model into individual shards? %(as a smallest tunable unit for resident model)? 
%As they are set to enable the engine to manage resident model in fine-granularity: depths, width, and fidelity. \Note{why use multiple fidelity has to be motivated early on}
%As they are 
%Set to enable the elasticity of a model (i.e. depths, widths, fidelity) and management (i.e. IO/computation/memory), they must meet the following criteria: 
Set to enable the resource elasticity of a model (i.e. depths/widths/fidelity), the shards must meet the following criteria: 
\begin{myitemize}	
	\item 
	\textit{Elastic execution.}
	Shards must preserve the same expressiveness of the attention mechanism and can execute partially. 
%	Can execute partially (with existing shards) and incrementally (with newly loaded shards). %Independent, compatible with each other 
	
	\item
	\textit{Tunable IO.} 
	IO compression ratios must be tunable to accommodate IO/computation capability of different hardware (e.g. due to diverse CPU/GPUs and DVFS). 
	Compression should not require further fine-tuning for fast deployment.
%	must not starve computation. 
%	This is to counter skewed IO delays. 
%	\xzlNote{IO delays must be tunable -- accommodate different hardware}
	
%	\item 
%	Support variable compression ratio, no re-finetuning, minimum accuracy loss. 
%	\xzlNote{overlap with point 2? I can see the point of shard importance}
\end{myitemize}

%To exploit the pipeline parallelism and construct the io/compute pipeline, we face the following two challenges.
%\Note{skewed io/compute: within a model; across diff. devices...}

% obsolete 
%\textit{First, pipelining at what granularity?}
%The key requirement is to allow for partial model execution.
%I.e. the inference may start as soon as the small part of the model is loaded.
%In hindsight, one may partition and pipeline the model by layers. 
%Yet, due to large model size, the \tfm{} models have a highly \textit{skewed} io/compute time\Note{TODO: there are more fundamental reasons for this}.
%For instance, io and compute latency of a layer differs by over 10$\times$ as demonstrated in~\S\ref{sec:motiv:char}.
%The naive layerwise partitioning leads to excessive, large pipeline bubbles and starves the CPU;
%as a result, the pipeline is no different from serial execution, failing the deadline..
%This is demonstrated in Figure \Note{XXX}.

%\textit{Second, how to handle device heterogeneity?}
%\Note{Do not need much exposure...}
%Not only the model itself are skewed in io/compute, edge devices are also known to have diverse hardware\Note{cite}. 
%Due to their different io/compute capability, there is no silver-bullet partitioning strategy given a deadline.
%As shown in \sect{motiv:char}, Rpi3 has much slower io compared with Odroid -- one partitioning strategy may have small pipeline bubbles on the latter but much larger bubbles on the former, starving CPUs.

%The \underline{second} research question is how to compress the shards?
%Broadly, three techniques can be used to compress the shards:
%shards may be pruned and discarded~\cite{cnn-entropy-filter-pruning, cnn-prune-nvidia}; 

%We set to shard \textit{pretrained} language models (e.g. BERT) without retraining. 
%The \underline{first} research question is at 
%To do so, there are two design choices. 
%One is \textit{unstructured} sharding~\cite{gordonCompressingBERTStudying2020,ladabert}, that is, viewing the whole (over 100 million) parameters as a large flat data array and splitting it in trunks. % which is common in network pruning

%they may share weights with each other~\cite{transformer-attention-share,nn-weight-share};
%they may be quantized into a lower bitwidth~\cite{binarybert,ibert,bibert}.
%%Our system must navigate through the compression techniques to ensure that shards 
%Our system must shard a model cautiously, navigate through the compression techniques, and ensure a decent model performance. %shards should work well with each other



\subsection{Instantiating model shards on disk}
\label{sec:design:sharding:shard}
%For pretrained \tfm{} models, we propose a retraining-free sharding approach, which is a novel combination of width-adaptive \tfm{} and outlier-aware quantization.
%\textbf{structured}, \textbf{outlier-aware quantization} approach for sharding the pretrained \tfm{} model. 
%Our key idea is to shard the model by layers, and by their attention heads.
%\Note{Our key construct is ...}
%In response, our key construct is \textit{model shards}, where we partition the transformer layers into mixed-precision, finer grained pieces.
To address the challenges, our key idea is to combine two machine learning techniques -- dynamic \tfm{}~\cite{dynabert,hat} and dictionary-based quantization~\cite{deep-compression}, in a novel way.
%To address the challenges, our key idea is to leverage a novel combination of two techniques: dynamic \tfm{}~\cite{dynabert,hat} and dictionary-based quantization~\cite{deep-compression}. 
We next describe details.
%compress a dynamic \tfm{} (e.g. DynaBERT~\cite{dynabert}, HAT~\cite{hat}) with Gaussian-outlier-aware simulated quantization~\cite{quantization-survey}.
%To address the challenges, our key insight is to leverage a dynamic \tfm{} with adaptive widths and depths (e.g. DynaBERT~\cite{dynabert}, HAT~\cite{hat}), with Gaussian-outlier-aware simulated quantization~\cite{gobo}.
%Our rationale is dynamic \tfm{} enables partial and incremental model execution because sub\Tfm{}s (\xzlNote{??}) share weights with the super\Tfm{}; 
%Gaussian-based simulated quantization works with pretrained models and incurs little accuracy degradation by accurately approximating parameter distribution~\cite{gobo,deep-compression}.
%We next describe the details.
%\Note{rationale, merge}
%The former enables partial and incremental model execution because sub\Tfm{}s share weights with the super\Tfm{}; 
%the latter works with pretrained models and incurs little accuracy degradation by exploiting parameter redundancy (\S\ref{sec:motiv:primer}).
%\Note{rationale merge}
%We do so because the parameter distribution of a \tfm{} layer is known to resemble Gaussian distribution~\cite{gobo};
%hence we can approximate the majority of values with a few representatives called centroids, while preserving the rest outliers (i.e. outside the Gaussian distribution). 
%The whole process resembles lossy compression and does not require fine tuning..

%We then partition each version into vertical slices by layers, which are model shards. 
%To address the challenges, our key insight is to leverage a dynamic \tfm{} with adaptive widths and depths (e.g. DynaBERT~\cite{dynabert}, HAT~\cite{hat}), and compress it into different fidelity versions using Gaussian-outlier-aware simulated quantization;
%we then partition each version into vertical slices by layers, which are model shards.

%Our rationale are as follows. 
%Dynamic \tfm{} allows for partial model execution;
%the parameter distribution of a \tfm{} layer 
%by approximating it with Gaussian distribution while preserving outliers resembles lossy compression which incurs little accuracy degradation. 

%integrating a novel combination of two known techniques: structured pruning \& outlier-aware quantization. 

%Compared with partitioning by layers, model shards bridges the gap between the skewed io vs compute (XXX vs XXX), allowing for efficient pipeline execution with small bubbles;
%their variable fidelity further enables elastic IO time.  %adapting to various deadlines on heterogeneous devices.
%\Note{merge below}
%% obsolete 
%\paragraph{\textit{Benefits}} are as follows.
%\begin{myitemize}
%	\item 
%	\textit{Partial model execution.}
%	First (cold) inference may start execution on only a few (e.g. 3) shards per layer, while subsequent inferences may incrementally load more.
%	
%	%Our rationale is as follows.
%	%First, an attention head is an atomic structure of the MHA mechanism~\cite{transformer}, which is learned at training time;
%	%shards conforming to the structure preserves the same mechanism.
%	%%shards can work seamlessly with each other. 
%	
%	\item 
%	\textit{Close and elastic IO/compute.}
%	A typical shard contains only one twelve-th parameter as a layer, thus having the same small portion of its IO (e.g. 40ms), approximating the compute time on a shard per layer (e.g. 30ms).
%	Mixed-precisions allow for multiple other devices..
%	
%\end{myitemize}

\input{fig-sharding}

%\xzlNote{each techniques below shall map back to challenges.}


%\Note{update Figure 5}
\paragraph{First, vertical partitioning per layer}
%\xzlNote{This this should go before quantization}
%The system then partitions each of $B$ fidelity versions into $M$ vertical slices by $K$ layers (in total $b\times m \times k$ such slices). 
The system adopts a pretrained \tfm{} model, which has already been fine-tuned on a downstream task. %(e.g. models from Huggingface~\cite{huggingface)}.
%such models they may be publicly accessible  
The model must have adaptive widths and depths, that is, at run time it may decide differently how many parameters of a layer to use (i.e. widths), as well as the number of layers (i.e. depths).
%The model must have adaptive widths and depths, that is, at run time it may decide differently how many number of attention heads and FFN neurons of a layer (i.e. widths), as well as the number of layers (i.e. depths) to use.
%The system adopts a pretrained dynamic \tfm{} model as the backbone network,  which is already fine-tuned on a downstream task (e.g. sentiment analysis) to have adaptive widths and depths. 
%That is, it can vary the number of attention heads and FFN neurons of a layer, as well as the number of layers.

For each of the $N$ layers, the system partitions it into $M$ vertical slices. %by total $N$ layers.
By construction, each vertical slice is independent, constituting one attention head plus $1/M$ of FFN neurons of the layer. %whose parameters compose a shard.
Table~\ref{tab:vertical_slice} shows the weight compositions of a vertical slice.
Each cell of the table describes the dimension of the weight matrix, where $d$ is hidden state size, $M$ is the number of attention heads, and $d_{ff}$ is the number of FFN neurons;
a shard is therefore one of the $M$ equal slices. 
%as can be seen, the partitioning equally slices the layer 
Doing so warrants model shards elasticity and the same capability to extract linguistic features from inputs, as done by the attention mechanism: 
%Doing so warrants model shards attending to linguistic features of input tokens: 
%Doing so warrants model shards with same attention mechanism linguistic features : 
of an individual shard, its attention head obtains one independent representation of input tokens, which is projected into a higher feature dimension by FFN neurons~\cite{attention-head-acl19,bert-acl19};
jointly, multiple shards attend to information from different representation subspace at different positions~\cite{transformer}.
%jointly, multiple shards recover full semantic features of inputs.
%A slice/shard $S$ can be uniquely identified by a three-tuple $S=(m,k,b)$, where $m, k$ are the indexes for the slice and layer respectively, and $b$ is its fidelity.
Therefore, an arbitrary subset of shards of a layer can be executed to produce meaningful results. % and their results can be combined to produce meaningful output.

%Doing so preserves the language features in the learned structure. \xzlNote{vague, find better rationales from prior work}

\begin{comment}
% below useful...merged 
\xzlNote{Compress the following two paragraphs into a table?}
Following~\cite{dynabert}, we define a shard's weight composition as follows. 
For a \tfm{} layer, 
%it is composed by five key weight matrix $W^Q, W^K, W^V, W^O$ and $FFN$, where
let $d$ denote the hidden state size, $M$ be the total number of attention heads (e.g. $M = 12$), $d_{ff}$ be the number of FFN neurons.
The size of each attention head $d_h$ is given by $d/{M}$, and the neurons of a shard $d_{ff'}$ is given by $d_{ff}/M$.
By equally partitioning the layer, we obtain $M$ vertical slices as model shards, indexed by $[0, M-1]$ from left to right.

The $j$-th shard is hence parameterized by six submatrix: $\{ W_{j}^Q, W_{j}^K, W_{j}^{V}, W_{j}^{O} \} \in \mathbb{R}^{d\times d_h}$ from an attention head, and two from FFN $W_{j}^{FFN1} \in \mathbb{R}^{d_{ff'}\times d},
	 W_{j}^{FFN2} \in \mathbb{R}^{d \times d_{ff'}}$.
The sub-matrix $W_{j}$ are selected by the $j$-th portion from respective $W$ along the non-feature dimension.
For instance, $W_{j}^{Q} = W_{:, j\cdot d_h:j\cdot(d_h+1)}^{Q}$.
Note that the index $j$ explicitly assigns the $j$-th slice of the weight matrix $W$ w.r.t. each shard in an non-overlapping manner.
\end{comment}

To execute a \tfm{} model using shards, \sys{} first decides a \textit{submodel} of $n$ layers; %$\times$ $m$ shards per layer.
mandated by the \tfm{} architecture~\cite{transformer}, each layer must have the same width (i.e. number of shards $m$) for an aligned number of output features.
Although it is possible for a shard to use 0s as placeholder weights, \sys{} expects all $m$ shards to have concrete weights for a good accuracy.
With $m$ shards, \sys{} computes the attention and FFN output of individual shards using the weight composition in Table~\ref{tab:vertical_slice}, concatenates their outputs, and proceeds to next layer.
The process therefore preserves the attention mechanism for producing meaningful results.
For more detailed mathematic formulation, an interested reader may refer to~\cite{16heads,dynabert}.


\input{tab-shard-param}

%The $j$-th model shard at $i$-th layer, $S(i,j)$, is parameterized by:
%%\Note{use a figure}
%
%\begin{equation}
%S(i,j) = \{W_{d_h}^{Q_i}, W_{d_h}^{K}, W_{d_h}^{V}, W_{d_h}^{O}\}\cup\{FFN_{d_h'}\}
%\end{equation}

%\xzlNote{clarify: which subset of a model shards are composable? why partial execution can still give meaningful inference result?}

%\xzlNote{where do we say that in a submodel, each layer must have the same number of shards, and why}

\xzlNote{much of the following (until the end of S4.3) can go to impl. Important things to mention: what is done at a high level; (typically) how many versions per shard; how are they stored on disk and how large (compression ratio); potential accuracy loss; model accuracy has different sensitivities to individual shards and their bitwidth; mixed precision: shards of different bitwidths can be combined in the same submodel; compute cost of compression/decompression..}

\paragraph{Second, simulated quantization per shard}
\label{sec:design:sharding:quantize}
%We next describe in detail how to quantize them into different precisions (bits).
The system compresses the each of the $N \times M$ shards into $K$ fidelity versions (e.g. 5 versions, $b=2\dots 6$). %each of which reduces the model size by a few $\times$.
The goal is to facilitate elastic IO, reduce IO/compute skewness, and give different fidelity per shard importance for maximizing resource utilization on different devices with diverse IO/compute capabilities. 
%\xzlNote{... and to give different fidelity (compression ratio) per shard importance...}

%of  : fidelity versions reduce their IO by a few $\times$, which can overlap with compute with small bubbles while adapting to .
%The goal is to facilitate elastic IO and amortize IO/compute skewness for maximizing resource utilization: fidelity versions reduce their IO by a few $\times$, which can overlap with compute with small bubbles while adapting to diverse IO/compute capability of different devices.


%The compression is feasible due to high parameter redundancy of \tfm{}, allowing accurate approximation via Gaussian distributions~\cite{tenarybert,gobo}.
%\Note{high level}
To compress, we use Gaussian outlier-aware quantization~\cite{gobo}.
%It exploits the Gaussian distribution of \tfm{} weights. 
The key idea is to replace the vast majority (i.e. 99.9\%) of weights which follow a Gaussin distribution with a $k$-bit indice pointing to one of the $2^k$ floating point numbers called \textit{centroids}, and preserve the very few \textit{outliers} (i.e. 0.01\%) as-is.
We choose it for its desirable properties as follows. % it satisfies following properties which we seek: 

\textit{Property I: high compression ratios, low accuracy loss.} 
As 99.9\% of 32-bit weight are replaced by K-bit dictionary indexes, the compression ratio is approximately 32/K.
For instance, at the lowest bitwidth we target (K=2), a shard is compressed by 16$\times$, whose file size is less than 200KB.
The high compression ratios correct IO/compute skewness, make storing all K versions cheap (e.g. adding only a few hundred MBs), and is tunable to cater capabilities of diverse devices. 
Meanwhile, the accuracy loss is minimum
For instance, it incurs less than 1\% accuracy degradation when K=6.
At lower K=2, the accuracy loss may be high, e.g. 10\%, but it can be remedied by \sys{}'s mechanism to load higher bitwidths shards, which we describe and evaluate later.



\Note{property1: can have high compression ratio, minimum accuracy loss. greatly reduces IO... (no more skewness)}
how many versions per shard; how are they stored on disk and how large (compression ratio); potential accuracy loss;


\Note{property2: resembles lossy compression. Work smoothly across different fidelity versions}
model accuracy has different sensitivities to individual shards and their bitwidth;
mixed precision: shards of different bitwidths can be combined in the same submodel


\Note{property3: does not need fine tuning and hardware support}
We choose it because it incurs little accuracy loss (<1\%) even at $10\times$ compression ratio by accurately approximating \tfm{} weights which follow a Gaussian distribution~\cite{gobo,tenarybert}, and that it is dictionary compression (i.e. simulated), which does not require fine-tuning.
%We donot use fixed-point quantization~\cite{binarybert,q8bert} because it is less elastic (e.g. fixed 8/4/2bit versions), needs DSP extension which is only seen on microcontrollers (e.g. Cortex-M4~\cite{m4-dsp}), and requires fine-tuning. 
We donot use fixed-point quantization~\cite{binarybert,q8bert} because it is less elastic (e.g. fixed 8/4/2bit versions), needs DSP extension which is only available on microcontrollers (e.g. Cortex-M4~\cite{m4-dsp}), and requires fine-tuning. 
Alternatively, a model may be compressed by knowledge distillation~\cite{distilbert} or model pruning~\cite{layerdrop,mobilebert}. 
However, they also require fine-tuning for \textit{each} version, and they likely lead to severe accuracy degradation as they must remove over 90\% of weights to achieve the same compression ratio as ours.



%
%For minimal accuracy loss, \sys{} uses \textit{simulated quantization}, \Note{reasons for not using real quantziation, i.e. integer operation: require fine-tuning for performance, not friendly to hardware}... 
%It quantizes the full-fledged shards into different lower-bit representations, reducing sizes by up to 16 $\times$. %inspired by a Gaussian-outlier-based quantization technique~\cite{quantization-survey};
%%With model shards as the key building block, \sys{} constructs an elastic pipeline whose IO and compute time is dependent on number of shards and their respective precisions. 
%\Note{Our novelty comp. w/ prior mixed-precision transformer and dynamic transformer:} the first to combine them to achieve elasticity; our goal is not to find a supernet or an optimal mixed-precision net, but to find building blocks. 




%\xzlNote{clarify: impact on IO and compute. why compute remains unaffected. also compare to other compression techniques that reduce both IO and compute (like distillation, transfer learning. why aren't those desirable)}
%Since the vast majority ($99.9\%$) of 32-bit weights are substituted by $b$-bit indexes to centroids, simulated quantization reduces IO by $\lfloor 32/b \rfloor \times$.
%It, however, does not reduce computation delays because the model maintains the same GFLOPS by computing on floating point centroids and outliers. 
\begin{comment}
% --- old, can merge ---
For each layer, the system fits all its weights into a Gaussian distribution, based on which it divides weights into two groups, an outlier group and a Gaussian group;
it preserves the former in full 32-bit fidelity and represents the latter with $2^b$ centroids, which are 32-bit floating point numbers.
%for the latter, it represents them with $2^b$ centroids. 
A weight is deemed as an outlier if the probability of it belongs to the Gaussian distribution is below a configurable threshold;
the larger the threshold, the more full-fidelity outliers, hence the lower compression ratio.  

Following the same practice in~\cite{gobo}, we use $-4$ which is sufficient in maintaining accuracy while maximizing compression ratio;
under the threshold, the outlier group constitute less than $0.1\%$ of total weights. %which is preserved in full precision (i.e. 32-bit). %and incurring only 1\% accuracy degradation. 
For the Gaussian group which constitute the rest $99.9\%$, the system sorts and splits its weights into $2^b$ clusters with equal population;
each cluster has \textit{one} centroid to represent \textit{all} values within it. 
%It then represents \textit{all} values in each cluster with \textit{one} centroid, which is indexed by a $b$-bit integer.
%It then represents \textit{all} values in each cluster with \textit{one} cluster centroid by substituting them with a $b$-bit index to the centroid.
Doing so caters to the weight distribution: weight-concentrated regions deserve higher resolutions, hence having more clusters and centroids.
%the vast majority ($99.9\%$) of original 32-bit weights are represented by $b$-bit integers, reducing model size by $\lfloor 32/b \rfloor \times$.
To decide cluster centroids, prior work adopt K-means based approaches~\cite{deep-compression, zhaoImprovingNeuralNetwork}, which are time-consuming, e.g. it takes a few hours to converge on our server.
Differently, we have found the arithmetic mean of cluster weights suffices -- a 2-bit version takes a few minutes to converge and incurs only 7\% accuracy degradation compared with the full model. 
We will present more results in \sect{eval}.  
%It uses the Gaussian model to find out a group of ``outliers'' parameters and preserve them in full precision.
%For the rest, the system quantizes them into $n$-bit integers (e.g. typically 2 to 4) using \textit{simulated quantization}~\cite{quantization-survey}, where each integer points to a full-precision FP32 value called a centroid, representing a group of original weights.
%The system decides the centroids by dividing the non-outlier parameters into $2^n$ groups and calculating their arithmetic means.

%The rationale is ....
%\Note{quantization rationale..}
%Second, attention head weights are heavily redundant~\cite{16heads}.
%%Most need only a few bits~\cite{ibert,binarybert} while only outliers need high-precision.
%Preserving the few outliers (e.g. 0.01\%~\cite{gobo}) while representing the most others with a small number of values ensures performance.
\end{comment}

%The system repeats the process for each fidelity version and generates a dictionary as the compression metadata, which specifies the centroids and the outlier mapping of full-fidelity weights.

\Note{how are they stored..}
\Note{compute cost of compression/decompression..}
\paragraph{Third, generating shards per version}
%After partitioning, a shard contains $1/M$ of a layer's total parameters, each is a $b$-bit centroid index.
To generate shards, the system compresses the vertical slices using the dictionaries produced by simulated quantization: 
for \textit{all} 32-bit parameter, the system looks up the dictionary and uniformly substitutes them with $b$-bit integers, each pointing to one of the $2^b$ centroids.
It does not preserve the 32-bit outliers in the newly compressed weight matrix to avoid destroying the $b$-bit data alignment.
It stores the compressed weights as the data and dictionaries (centroids, outliers) as the metadata of model shards on disk.
This is shown in Figure~\ref{fig:design:shards}. %\xzlNote{Fig 4 needs update, showing the workflow}
The system generates $N \times M\times K$ such shards and stores them on disk by their identities using a three-tuple $S=(n, m, b)$, where $n$, $m$ are the indexes of the layer and vertical slice respectively, $b$ is the fidelity.
It co-locates their disk blocks for access locality.
%Instead, it stores the outlier mapping separately to the compressed weights, which specifies 

Note that model shards \xzlNote{quantization} reduces IO but not computation (GFLOPs). \xzlNote{as opposed to XXX techniques. By doing so we avoid tedious per-model retraining as opposed to XXX (is this right?) and ensure to generate adequate compute workloads for high accuracy}
This is because they only change the representations of model parameters but not their amount.
For instance, by substituting 99.9\% of 32-bit weights with $b$-bit centroid indexes, a shard reduces IO by $\lfloor 32/b \rfloor \times$.
At inference time, the model retains GFLOPS by computing on the same amount of floating points decompressed from centroids and outliers;
while being inevitable, the decompression is efficient (10-20ms per layer) and can be further alleviated by designated hardware accelerator~\cite{gobo}.

%In uncompressed, full-fidelity form, their sizes are $1/M$ of a layer (e.g. a few MBs), taking tens of ms to load; 
%in lower fidelities, their IOs are even smaller and elastic w.r.t. bit fidelity. 
%%Hence a model shard equally slices the $j$-th layer it belongs to.
%Note: when in lower fidelities, shards cannot be used directly -- the weights are only indexes. 
%They cannot be used interchangeably, e.g. a 1 in 2-bit and 6-bit shard points to different centroids.  
%For instance, for the 1st layer with 3 shards,  


%Since the vast majority ($99.9\%$) of 32-bit weights can map to centroids, which are indexed by $b$-bit integers, the model size is reduced by $\lfloor 32/b \rfloor \times$.

%Following~\cite{dynabert}, the attention score and output of a layer can be defined as:
%
%\begin{equation}
%	\label{eq:out}
%\end{equation}
%
%Therefore as listed in equation~\ref{eq:out}, the output of a \tfm{} layer can be regarded as the sum of independent model shards, allowing partial execution of the model.

%\paragraph{Storing model shards}
%The system stores all versions of shards and their corresponding centroids on disk. %and pick selectively at run time. 
%Unused ones (e.g. for other tasks) can be further compressed via lossless compression (e.g. Zip). 
%This is possible because of low entropy.
%%Will evaluate its size (smaller than a HD movie) and compression efficiency (>90\%). 
%\Note{why not only store 6bit and derive the others?} 
%Doing so requires to \textit{always} load 6-bit shard IO delays.
%Not elastic, may miss deadline.

%\xzlNote{need cost analysis? }
%At least mention prior work on hardware accelerator


 



==> design-sharding__Liwei_Guo_s_conflicted_copy_2022-07-05_1_.tex <==
% !TeX root = main.tex

\section{Elastic model sharding}
%\section{Managing the model in elastic shards}
%\section{Managing \Tfm{}s in fine elasticity}
%\section{Building an elastic IO/compute pipeline}
\label{sec:design:sharding}


%\textbf{Key points (structured around resident model):}1
%\begin{itemize}
%	\item 
%	Challenge: how to properly select a model shard? Must meet a list of criteria..
%	
%	\item
%	Model shards. Two things: partition by vertical slice (insights, formal definition), quantization technique (rationale, operation)
%	
%	\item
%	Resident model structure: in-memory representation, how to use, 
%	misc: activations (fixed high bits due to small, negligible).
%\end{itemize}


\xzlNote{moved here, to merge}
where each shard spans one Transformer attention head and $1/M$ FFN neurons of this layer. 
For each shard, it creates $K$ fidelity versions, which are lower-bit representations of this shard's weights. 
For instance, a full-fidelity version that represents each weight with 32 bits, a two-bit version that does so with 2 bits. 
We therefore store $NxMxK$ shard versions on disk. 
The preprocessing is a one-time effort per model; being light transformation of an existing model without pre-training, it can be done on device at the model installation time. 



%The preprocessing is a one-time effort per model; 
%lightweight and requiring no model re-retraining, it can be done on mobile devices. 


\Note{Model shards trade inexpensive disk storage for expensive, scarce memory... }


\subsection{Key challenges}
%\Note{merge challenges to below}
%We solve a key challenge in constructing a resident model: how to choose the proper parameter composition of a shard? %(as a smallest tunable unit for resident model)? 
%We solve a key challenge in constructing a resident model: how to instantiate a model shard? %(as a smallest tunable unit for resident model)? 
%We solve a key challenge: how to instantiate an elastic shard? %(as a smallest tunable unit for resident model)? 
We solve a key challenge: how to partition the model into individual shards? %(as a smallest tunable unit for resident model)? 
%As they are set to enable the engine to manage resident model in fine-granularity: depths, width, and fidelity. \Note{why use multiple fidelity has to be motivated early on}
%As they are 
%Set to enable the elasticity of a model (i.e. depths, widths, fidelity) and management (i.e. IO/computation/memory), they must meet the following criteria: 
Set to enable the resource elasticity of a model (i.e. depths/widths/fidelity), the shards must meet the following criteria: 
\begin{myitemize}	
	\item 
	\textit{Elastic execution.}
	Shards must preserve the same expressiveness of the attention mechanism and can execute partially. 
%	Can execute partially (with existing shards) and incrementally (with newly loaded shards). %Independent, compatible with each other 
	
	\item
	\textit{Tunable IO.} 
	IO compression ratios must be tunable to accommodate IO/computation capability of different hardware (e.g. due to diverse CPU/GPUs and DVFS). 
	Compression should not require further fine-tuning for fast deployment.
%	must not starve computation. 
%	This is to counter skewed IO delays. 
%	\xzlNote{IO delays must be tunable -- accommodate different hardware}
	
%	\item 
%	Support variable compression ratio, no re-finetuning, minimum accuracy loss. 
%	\xzlNote{overlap with point 2? I can see the point of shard importance}
\end{myitemize}

%To exploit the pipeline parallelism and construct the io/compute pipeline, we face the following two challenges.
%\Note{skewed io/compute: within a model; across diff. devices...}

% obsolete 
%\textit{First, pipelining at what granularity?}
%The key requirement is to allow for partial model execution.
%I.e. the inference may start as soon as the small part of the model is loaded.
%In hindsight, one may partition and pipeline the model by layers. 
%Yet, due to large model size, the \tfm{} models have a highly \textit{skewed} io/compute time\Note{TODO: there are more fundamental reasons for this}.
%For instance, io and compute latency of a layer differs by over 10$\times$ as demonstrated in~\S\ref{sec:motiv:char}.
%The naive layerwise partitioning leads to excessive, large pipeline bubbles and starves the CPU;
%as a result, the pipeline is no different from serial execution, failing the deadline..
%This is demonstrated in Figure \Note{XXX}.

%\textit{Second, how to handle device heterogeneity?}
%\Note{Do not need much exposure...}
%Not only the model itself are skewed in io/compute, edge devices are also known to have diverse hardware\Note{cite}. 
%Due to their different io/compute capability, there is no silver-bullet partitioning strategy given a deadline.
%As shown in \sect{motiv:char}, Rpi3 has much slower io compared with Odroid -- one partitioning strategy may have small pipeline bubbles on the latter but much larger bubbles on the former, starving CPUs.

%The \underline{second} research question is how to compress the shards?
%Broadly, three techniques can be used to compress the shards:
%shards may be pruned and discarded~\cite{cnn-entropy-filter-pruning, cnn-prune-nvidia}; 

%We set to shard \textit{pretrained} language models (e.g. BERT) without retraining. 
%The \underline{first} research question is at 
%To do so, there are two design choices. 
%One is \textit{unstructured} sharding~\cite{gordonCompressingBERTStudying2020,ladabert}, that is, viewing the whole (over 100 million) parameters as a large flat data array and splitting it in trunks. % which is common in network pruning

%they may share weights with each other~\cite{transformer-attention-share,nn-weight-share};
%they may be quantized into a lower bitwidth~\cite{binarybert,ibert,bibert}.
%%Our system must navigate through the compression techniques to ensure that shards 
%Our system must shard a model cautiously, navigate through the compression techniques, and ensure a decent model performance. %shards should work well with each other



\subsection{Instantiating model shards on disk}
\label{sec:design:sharding:shard}
%For pretrained \tfm{} models, we propose a retraining-free sharding approach, which is a novel combination of width-adaptive \tfm{} and outlier-aware quantization.
%\textbf{structured}, \textbf{outlier-aware quantization} approach for sharding the pretrained \tfm{} model. 
%Our key idea is to shard the model by layers, and by their attention heads.
%\Note{Our key construct is ...}
%In response, our key construct is \textit{model shards}, where we partition the transformer layers into mixed-precision, finer grained pieces.
To address the challenges, our key idea is to combine two machine learning techniques -- dynamic \tfm{}~\cite{dynabert,hat} and dictionary-based quantization~\cite{deep-compression}, in a novel way.
%To address the challenges, our key idea is to leverage a novel combination of two techniques: dynamic \tfm{}~\cite{dynabert,hat} and dictionary-based quantization~\cite{deep-compression}. 
We next describe details.
%compress a dynamic \tfm{} (e.g. DynaBERT~\cite{dynabert}, HAT~\cite{hat}) with Gaussian-outlier-aware simulated quantization~\cite{quantization-survey}.
%To address the challenges, our key insight is to leverage a dynamic \tfm{} with adaptive widths and depths (e.g. DynaBERT~\cite{dynabert}, HAT~\cite{hat}), with Gaussian-outlier-aware simulated quantization~\cite{gobo}.
%Our rationale is dynamic \tfm{} enables partial and incremental model execution because sub\Tfm{}s (\xzlNote{??}) share weights with the super\Tfm{}; 
%Gaussian-based simulated quantization works with pretrained models and incurs little accuracy degradation by accurately approximating parameter distribution~\cite{gobo,deep-compression}.
%We next describe the details.
%\Note{rationale, merge}
%The former enables partial and incremental model execution because sub\Tfm{}s share weights with the super\Tfm{}; 
%the latter works with pretrained models and incurs little accuracy degradation by exploiting parameter redundancy (\S\ref{sec:motiv:primer}).
%\Note{rationale merge}
%We do so because the parameter distribution of a \tfm{} layer is known to resemble Gaussian distribution~\cite{gobo};
%hence we can approximate the majority of values with a few representatives called centroids, while preserving the rest outliers (i.e. outside the Gaussian distribution). 
%The whole process resembles lossy compression and does not require fine tuning..

%We then partition each version into vertical slices by layers, which are model shards. 
%To address the challenges, our key insight is to leverage a dynamic \tfm{} with adaptive widths and depths (e.g. DynaBERT~\cite{dynabert}, HAT~\cite{hat}), and compress it into different fidelity versions using Gaussian-outlier-aware simulated quantization;
%we then partition each version into vertical slices by layers, which are model shards.

%Our rationale are as follows. 
%Dynamic \tfm{} allows for partial model execution;
%the parameter distribution of a \tfm{} layer 
%by approximating it with Gaussian distribution while preserving outliers resembles lossy compression which incurs little accuracy degradation. 

%integrating a novel combination of two known techniques: structured pruning \& outlier-aware quantization. 

%Compared with partitioning by layers, model shards bridges the gap between the skewed io vs compute (XXX vs XXX), allowing for efficient pipeline execution with small bubbles;
%their variable fidelity further enables elastic IO time.  %adapting to various deadlines on heterogeneous devices.
%\Note{merge below}
%% obsolete 
%\paragraph{\textit{Benefits}} are as follows.
%\begin{myitemize}
%	\item 
%	\textit{Partial model execution.}
%	First (cold) inference may start execution on only a few (e.g. 3) shards per layer, while subsequent inferences may incrementally load more.
%	
%	%Our rationale is as follows.
%	%First, an attention head is an atomic structure of the MHA mechanism~\cite{transformer}, which is learned at training time;
%	%shards conforming to the structure preserves the same mechanism.
%	%%shards can work seamlessly with each other. 
%	
%	\item 
%	\textit{Close and elastic IO/compute.}
%	A typical shard contains only one twelve-th parameter as a layer, thus having the same small portion of its IO (e.g. 40ms), approximating the compute time on a shard per layer (e.g. 30ms).
%	Mixed-precisions allow for multiple other devices..
%	
%\end{myitemize}

\input{fig-sharding}

%\xzlNote{each techniques below shall map back to challenges.}


%\Note{update Figure 5}
\paragraph{First, vertical partitioning per layer}
%\xzlNote{This this should go before quantization}
%The system then partitions each of $B$ fidelity versions into $M$ vertical slices by $K$ layers (in total $b\times m \times k$ such slices). 
The system adopts a pretrained \tfm{} model, which has already been fine-tuned on a downstream task. %(e.g. models from Huggingface~\cite{huggingface)}.
%such models they may be publicly accessible  
The model must have adaptive widths and depths, that is, at run time it may decide differently how many parameters of a layer to use (i.e. widths), as well as the number of layers (i.e. depths).
%The model must have adaptive widths and depths, that is, at run time it may decide differently how many number of attention heads and FFN neurons of a layer (i.e. widths), as well as the number of layers (i.e. depths) to use.
%The system adopts a pretrained dynamic \tfm{} model as the backbone network,  which is already fine-tuned on a downstream task (e.g. sentiment analysis) to have adaptive widths and depths. 
%That is, it can vary the number of attention heads and FFN neurons of a layer, as well as the number of layers.

For each of the $N$ layers, the system partitions it into $M$ vertical slices. %by total $N$ layers.
By construction, each vertical slice is independent, constituting one attention head plus $1/M$ of FFN neurons of the layer. %whose parameters compose a shard.
Table~\ref{tab:vertical_slice} shows the weight compositions of a vertical slice.
Each cell of the table describes the dimension of the weight matrix, where $d$ is hidden state size, $M$ is the number of attention heads, and $d_{ff}$ is the number of FFN neurons;
a shard is therefore one of the $M$ equal slices. 
%as can be seen, the partitioning equally slices the layer 
Doing so warrants model shards elasticity and the same capability to extract linguistic features from inputs, as done by the attention mechanism: 
%Doing so warrants model shards attending to linguistic features of input tokens: 
%Doing so warrants model shards with same attention mechanism linguistic features : 
of an individual shard, its attention head obtains one independent representation of input tokens, which is projected into a higher feature dimension by FFN neurons~\cite{attention-head-acl19,bert-acl19};
jointly, multiple shards attend to information from different representation subspace at different positions~\cite{transformer}.
%jointly, multiple shards recover full semantic features of inputs.
%A slice/shard $S$ can be uniquely identified by a three-tuple $S=(m,k,b)$, where $m, k$ are the indexes for the slice and layer respectively, and $b$ is its fidelity.
Therefore, an arbitrary subset of shards of a layer can be executed to produce meaningful results. % and their results can be combined to produce meaningful output.

%Doing so preserves the language features in the learned structure. \xzlNote{vague, find better rationales from prior work}

\begin{comment}
% below useful...merged 
\xzlNote{Compress the following two paragraphs into a table?}
Following~\cite{dynabert}, we define a shard's weight composition as follows. 
For a \tfm{} layer, 
%it is composed by five key weight matrix $W^Q, W^K, W^V, W^O$ and $FFN$, where
let $d$ denote the hidden state size, $M$ be the total number of attention heads (e.g. $M = 12$), $d_{ff}$ be the number of FFN neurons.
The size of each attention head $d_h$ is given by $d/{M}$, and the neurons of a shard $d_{ff'}$ is given by $d_{ff}/M$.
By equally partitioning the layer, we obtain $M$ vertical slices as model shards, indexed by $[0, M-1]$ from left to right.

The $j$-th shard is hence parameterized by six submatrix: $\{ W_{j}^Q, W_{j}^K, W_{j}^{V}, W_{j}^{O} \} \in \mathbb{R}^{d\times d_h}$ from an attention head, and two from FFN $W_{j}^{FFN1} \in \mathbb{R}^{d_{ff'}\times d},
	 W_{j}^{FFN2} \in \mathbb{R}^{d \times d_{ff'}}$.
The sub-matrix $W_{j}$ are selected by the $j$-th portion from respective $W$ along the non-feature dimension.
For instance, $W_{j}^{Q} = W_{:, j\cdot d_h:j\cdot(d_h+1)}^{Q}$.
Note that the index $j$ explicitly assigns the $j$-th slice of the weight matrix $W$ w.r.t. each shard in an non-overlapping manner.
\end{comment}

To execute a \tfm{} model using shards, \sys{} first decides a \textit{submodel} of $n$ layers; %$\times$ $m$ shards per layer.
mandated by the \tfm{} architecture~\cite{transformer}, each layer must have the same width (i.e. number of shards $m$) for an aligned number of output features.
Although it is possible for a shard to use 0s as placeholder weights, \sys{} expects all $m$ shards to have concrete weights for a good accuracy.
With $m$ shards, \sys{} computes the attention and FFN output of individual shards using the weight composition in Table~\ref{tab:vertical_slice}, concatenates their outputs, and proceeds to next layer.
The process therefore preserves the attention mechanism for producing meaningful results.
For more detailed mathematic formulation, an interested reader may refer to~\cite{16heads,dynabert}.


\input{tab-shard-param}

%The $j$-th model shard at $i$-th layer, $S(i,j)$, is parameterized by:
%%\Note{use a figure}
%
%\begin{equation}
%S(i,j) = \{W_{d_h}^{Q_i}, W_{d_h}^{K}, W_{d_h}^{V}, W_{d_h}^{O}\}\cup\{FFN_{d_h'}\}
%\end{equation}

%\xzlNote{clarify: which subset of a model shards are composable? why partial execution can still give meaningful inference result?}

%\xzlNote{where do we say that in a submodel, each layer must have the same number of shards, and why}

\xzlNote{much of the following (until the end of S4.3) can go to impl. Important things to mention: what is done at a high level; (typically) how many versions per shard; how are they stored on disk and how large (compression ratio); potential accuracy loss; model accuracy has different sensitivities to individual shards and their bitwidth; mixed precision: shards of different bitwidths can be combined in the same submodel; compute cost of compression/decompression..}

\paragraph{Second, simulated quantization per shard}
\label{sec:design:sharding:quantize}
%We next describe in detail how to quantize them into different precisions (bits).
The system compresses the each of the $N \times M$ shards into $K$ fidelity versions (e.g. 5 versions, $b=2\dots 6$). %each of which reduces the model size by a few $\times$.
The goal is to facilitate elastic IO, reduce IO/compute skewness, and give different fidelity per shard importance for maximizing resource utilization on different devices with diverse IO/compute capabilities. 
%\xzlNote{... and to give different fidelity (compression ratio) per shard importance...}

%of  : fidelity versions reduce their IO by a few $\times$, which can overlap with compute with small bubbles while adapting to .
%The goal is to facilitate elastic IO and amortize IO/compute skewness for maximizing resource utilization: fidelity versions reduce their IO by a few $\times$, which can overlap with compute with small bubbles while adapting to diverse IO/compute capability of different devices.


%The compression is feasible due to high parameter redundancy of \tfm{}, allowing accurate approximation via Gaussian distributions~\cite{tenarybert,gobo}.
%\Note{high level}
To compress, we use Gaussian outlier-aware quantization~\cite{gobo}.
%It exploits the Gaussian distribution of \tfm{} weights. 
The key idea is to replace the vast majority (i.e. 99.9\%) of weights which follow a Gaussin distribution with a $k$-bit indice pointing to one of the $2^k$ floating point numbers called \textit{centroids}, and preserve the very few \textit{outliers} (i.e. 0.01\%) as-is.
The process is shown in Figure~\ref{fig:design:shards} (2).
We choose it for its desirable properties as follows. % it satisfies following properties which we seek: 

\Note{property1: can have high compression ratio, minimum accuracy loss. greatly reduces IO... (no more skewness)}
how many versions per shard; how are they stored on disk and how large (compression ratio); potential accuracy loss;

\textit{Property I: high compression ratios, low accuracy loss.} 
For a K-bit version, the approach compresses a shard by 32/K, as 99.9\% of 32-bit weight are replaced by K-bit dictionary indexes.
For instance, at the lowest bitwidth we target (K=2), the shard is compressed by 16$\times$, whose file size is less than 200KB.
The high compression ratios correct IO/compute skewness and make storing all K versions cheap, e.g. for typically five versions, K=$2\dots6$, it adds only a few hundred MBs. %and is tunable to cater capabilities of diverse devices. 
Meanwhile, the accuracy loss is minimum, incurring less than 1\% accuracy degradation when K=6.
At lower K=2, the accuracy loss may be high, e.g. 10\%, but it can be remedied by \sys{}'s mechanism to load higher bitwidths shards, which we describe and evaluate later.

\Note{property2: resembles lossy compression. Work smoothly across different fidelity versions}
model accuracy has different sensitivities to individual shards and their bitwidth;
mixed precision: shards of different bitwidths can be combined in the same submodel

\textit{Property II: good compatibility between versions.}
%The dictionary compression resembles lossy compression.
The lossy compression nature of our quantization allows shards of different versions to work seamlessly with each other, assembling a submodel with \textit{mixed bitwidths}.
This is because shards still have the same distribution as the original layer weights, albeit in different fidelities. 
To use, the engine decompresses the shards by simply mass substituting dictionary indexes with centroids (i.e. floating point numbers) and computes on restored FP32 weights;
the decompression is efficient on a commodity SoC, less than 20ms for one layer.
%the inference only have floating point operations;
This differs from a traditional \textit{mixed-precision} network, which mixes floating point operations with integer operations~\Note{cite}.

More importantly, the good compatibility enables \sys{} to tune bitwidths for individual shards and prioritize those with per importance. 
For by giving them higher-bitwidths. 



\Note{property3: does not need fine tuning and hardware support}
We choose it because it incurs little accuracy loss (<1\%) even at $10\times$ compression ratio by accurately approximating \tfm{} weights which follow a Gaussian distribution~\cite{gobo,tenarybert}, and that it is dictionary compression (i.e. simulated), which does not require fine-tuning.
%We donot use fixed-point quantization~\cite{binarybert,q8bert} because it is less elastic (e.g. fixed 8/4/2bit versions), needs DSP extension which is only seen on microcontrollers (e.g. Cortex-M4~\cite{m4-dsp}), and requires fine-tuning. 
We donot use fixed-point quantization~\cite{binarybert,q8bert} because it is less elastic (e.g. fixed 8/4/2bit versions), needs DSP extension which is only available on microcontrollers (e.g. Cortex-M4~\cite{m4-dsp}), and requires fine-tuning. 
Alternatively, a model may be compressed by knowledge distillation~\cite{distilbert} or model pruning~\cite{layerdrop,mobilebert}. 
However, they also require fine-tuning for \textit{each} version, and they likely lead to severe accuracy degradation as they must remove over 90\% of weights to achieve the same compression ratio as ours.



%
%For minimal accuracy loss, \sys{} uses \textit{simulated quantization}, \Note{reasons for not using real quantziation, i.e. integer operation: require fine-tuning for performance, not friendly to hardware}... 
%It quantizes the full-fledged shards into different lower-bit representations, reducing sizes by up to 16 $\times$. %inspired by a Gaussian-outlier-based quantization technique~\cite{quantization-survey};
%%With model shards as the key building block, \sys{} constructs an elastic pipeline whose IO and compute time is dependent on number of shards and their respective precisions. 
%\Note{Our novelty comp. w/ prior mixed-precision transformer and dynamic transformer:} the first to combine them to achieve elasticity; our goal is not to find a supernet or an optimal mixed-precision net, but to find building blocks. 




%\xzlNote{clarify: impact on IO and compute. why compute remains unaffected. also compare to other compression techniques that reduce both IO and compute (like distillation, transfer learning. why aren't those desirable)}
%Since the vast majority ($99.9\%$) of 32-bit weights are substituted by $b$-bit indexes to centroids, simulated quantization reduces IO by $\lfloor 32/b \rfloor \times$.
%It, however, does not reduce computation delays because the model maintains the same GFLOPS by computing on floating point centroids and outliers. 
\begin{comment}
% --- old, can merge ---
For each layer, the system fits all its weights into a Gaussian distribution, based on which it divides weights into two groups, an outlier group and a Gaussian group;
it preserves the former in full 32-bit fidelity and represents the latter with $2^b$ centroids, which are 32-bit floating point numbers.
%for the latter, it represents them with $2^b$ centroids. 
A weight is deemed as an outlier if the probability of it belongs to the Gaussian distribution is below a configurable threshold;
the larger the threshold, the more full-fidelity outliers, hence the lower compression ratio.  

Following the same practice in~\cite{gobo}, we use $-4$ which is sufficient in maintaining accuracy while maximizing compression ratio;
under the threshold, the outlier group constitute less than $0.1\%$ of total weights. %which is preserved in full precision (i.e. 32-bit). %and incurring only 1\% accuracy degradation. 
For the Gaussian group which constitute the rest $99.9\%$, the system sorts and splits its weights into $2^b$ clusters with equal population;
each cluster has \textit{one} centroid to represent \textit{all} values within it. 
%It then represents \textit{all} values in each cluster with \textit{one} centroid, which is indexed by a $b$-bit integer.
%It then represents \textit{all} values in each cluster with \textit{one} cluster centroid by substituting them with a $b$-bit index to the centroid.
Doing so caters to the weight distribution: weight-concentrated regions deserve higher resolutions, hence having more clusters and centroids.
%the vast majority ($99.9\%$) of original 32-bit weights are represented by $b$-bit integers, reducing model size by $\lfloor 32/b \rfloor \times$.
To decide cluster centroids, prior work adopt K-means based approaches~\cite{deep-compression, zhaoImprovingNeuralNetwork}, which are time-consuming, e.g. it takes a few hours to converge on our server.
Differently, we have found the arithmetic mean of cluster weights suffices -- a 2-bit version takes a few minutes to converge and incurs only 7\% accuracy degradation compared with the full model. 
We will present more results in \sect{eval}.  
%It uses the Gaussian model to find out a group of ``outliers'' parameters and preserve them in full precision.
%For the rest, the system quantizes them into $n$-bit integers (e.g. typically 2 to 4) using \textit{simulated quantization}~\cite{quantization-survey}, where each integer points to a full-precision FP32 value called a centroid, representing a group of original weights.
%The system decides the centroids by dividing the non-outlier parameters into $2^n$ groups and calculating their arithmetic means.

%The rationale is ....
%\Note{quantization rationale..}
%Second, attention head weights are heavily redundant~\cite{16heads}.
%%Most need only a few bits~\cite{ibert,binarybert} while only outliers need high-precision.
%Preserving the few outliers (e.g. 0.01\%~\cite{gobo}) while representing the most others with a small number of values ensures performance.
\end{comment}

%The system repeats the process for each fidelity version and generates a dictionary as the compression metadata, which specifies the centroids and the outlier mapping of full-fidelity weights.

\Note{how are they stored..}
\Note{compute cost of compression/decompression..}
\paragraph{Third, generating shards per version}
%After partitioning, a shard contains $1/M$ of a layer's total parameters, each is a $b$-bit centroid index.
To generate shards, the system compresses the vertical slices using the dictionaries produced by simulated quantization: 
for \textit{all} 32-bit parameter, the system looks up the dictionary and uniformly substitutes them with $b$-bit integers, each pointing to one of the $2^b$ centroids.
It does not preserve the 32-bit outliers in the newly compressed weight matrix to avoid destroying the $b$-bit data alignment.
It stores the compressed weights as the data and dictionaries (centroids, outliers) as the metadata of model shards on disk.
This is shown in Figure~\ref{fig:design:shards}. %\xzlNote{Fig 4 needs update, showing the workflow}
The system generates $N \times M\times K$ such shards and stores them on disk by their identities using a three-tuple $S=(n, m, b)$, where $n$, $m$ are the indexes of the layer and vertical slice respectively, $b$ is the fidelity.
It co-locates their disk blocks for access locality.
%Instead, it stores the outlier mapping separately to the compressed weights, which specifies 

Note that model shards \xzlNote{quantization} reduces IO but not computation (GFLOPs). \xzlNote{as opposed to XXX techniques. By doing so we avoid tedious per-model retraining as opposed to XXX (is this right?) and ensure to generate adequate compute workloads for high accuracy}
This is because they only change the representations of model parameters but not their amount.
For instance, by substituting 99.9\% of 32-bit weights with $b$-bit centroid indexes, a shard reduces IO by $\lfloor 32/b \rfloor \times$.
At inference time, the model retains GFLOPS by computing on the same amount of floating points decompressed from centroids and outliers;
while being inevitable, the decompression is efficient (10-20ms per layer) and can be further alleviated by designated hardware accelerator~\cite{gobo}.

%In uncompressed, full-fidelity form, their sizes are $1/M$ of a layer (e.g. a few MBs), taking tens of ms to load; 
%in lower fidelities, their IOs are even smaller and elastic w.r.t. bit fidelity. 
%%Hence a model shard equally slices the $j$-th layer it belongs to.
%Note: when in lower fidelities, shards cannot be used directly -- the weights are only indexes. 
%They cannot be used interchangeably, e.g. a 1 in 2-bit and 6-bit shard points to different centroids.  
%For instance, for the 1st layer with 3 shards,  


%Since the vast majority ($99.9\%$) of 32-bit weights can map to centroids, which are indexed by $b$-bit integers, the model size is reduced by $\lfloor 32/b \rfloor \times$.

%Following~\cite{dynabert}, the attention score and output of a layer can be defined as:
%
%\begin{equation}
%	\label{eq:out}
%\end{equation}
%
%Therefore as listed in equation~\ref{eq:out}, the output of a \tfm{} layer can be regarded as the sum of independent model shards, allowing partial execution of the model.

%\paragraph{Storing model shards}
%The system stores all versions of shards and their corresponding centroids on disk. %and pick selectively at run time. 
%Unused ones (e.g. for other tasks) can be further compressed via lossless compression (e.g. Zip). 
%This is possible because of low entropy.
%%Will evaluate its size (smaller than a HD movie) and compression efficiency (>90\%). 
%\Note{why not only store 6bit and derive the others?} 
%Doing so requires to \textit{always} load 6-bit shard IO delays.
%Not elastic, may miss deadline.

%\xzlNote{need cost analysis? }
%At least mention prior work on hardware accelerator


 



==> design-sharding__Liwei_Guo_s_conflicted_copy_2022-12-11_.tex <==
% !TeX root = main.tex

\section{Elastic model sharding}
%\section{Managing the model in elastic shards}
%\section{Managing \Tfm{}s in fine elasticity}
%\section{Building an elastic IO/compute pipeline}
\label{sec:design:sharding}


%\textbf{Key points (structured around resident model):}1
%\begin{itemize}
%	\item 
%	Challenge: how to properly select a model shard? Must meet a list of criteria..
%	
%	\item
%	Model shards. Two things: partition by vertical slice (insights, formal definition), quantization technique (rationale, operation)
%	
%	\item
%	Resident model structure: in-memory representation, how to use, 
%	misc: activations (fixed high bits due to small, negligible).
%\end{itemize}


%\xzlNote{moved here, to merge}
%where each shard spans one Transformer attention head and $1/M$ FFN neurons of this layer. 
%For each shard, it creates $K$ fidelity versions, which are lower-bit representations of this shard's weights. 
%For instance, a full-fidelity version that represents each weight with 32 bits, a two-bit version that does so with 2 bits. 
%We therefore store $NxMxK$ shard versions on disk. 
%The preprocessing is a one-time effort per model; being light transformation of an existing model without pre-training, it can be done on device at the model installation time. 
%\Note{Model shards trade inexpensive disk storage for expensive, scarce memory... }


%The preprocessing is a one-time effort per model; 
%lightweight and requiring no model re-retraining, it can be done on mobile devices. 




%\Note{needed?}
\subsection{Key challenges}
%\Note{merge challenges to below}
%We solve a key challenge in constructing a resident model: how to choose the proper parameter composition of a shard? %(as a smallest tunable unit for resident model)? 
%We solve a key challenge in constructing a resident model: how to instantiate a model shard? %(as a smallest tunable unit for resident model)? 
%We solve a key challenge: how to instantiate an elastic shard? %(as a smallest tunable unit for resident model)? 
We solve a key challenge: how to partition the model into individual shards? %(as a smallest tunable unit for resident model)? 
%As they are set to enable the engine to manage resident model in fine-granularity: depths, width, and fidelity. \Note{why use multiple fidelity has to be motivated early on}
%As they are 
%Set to enable the elasticity of a model (i.e. depths, widths, fidelity) and management (i.e. IO/computation/memory), they must meet the following criteria: 
Set to enable the resource elasticity of a model (i.e. depths/widths/fidelity), the shards must meet the following criteria: 
\begin{myitemize}	
	\item 
	\textit{Elastic execution.}
	Shards must preserve the same expressiveness of the attention mechanism and can execute partially to produce meaningful results. 
%	Can execute partially (with existing shards) and incrementally (with newly loaded shards). %Independent, compatible with each other 
	
	\item
	\textit{Tunable IO.} 
	The IO delays of shards must be tunable to accommodate IO/compute capability of different hardware (e.g. due to diverse CPU/GPUs and DVFS). 
	%Compression should not require further fine-tuning for fast deployment.
%	must not starve computation. 
%	This is to counter skewed IO delays. 
%	\xzlNote{IO delays must be tunable -- accommodate different hardware}
	
%	\item 
%	Support variable compression ratio, no re-finetuning, minimum accuracy loss. 
%	\xzlNote{overlap with point 2? I can see the point of shard importance}
\end{myitemize}

%To exploit the pipeline parallelism and construct the io/compute pipeline, we face the following two challenges.
%\Note{skewed io/compute: within a model; across diff. devices...}

% obsolete 
%\textit{First, pipelining at what granularity?}
%The key requirement is to allow for partial model execution.
%I.e. the inference may start as soon as the small part of the model is loaded.
%In hindsight, one may partition and pipeline the model by layers. 
%Yet, due to large model size, the \tfm{} models have a highly \textit{skewed} io/compute time\Note{TODO: there are more fundamental reasons for this}.
%For instance, io and compute latency of a layer differs by over 10$\times$ as demonstrated in~\S\ref{sec:motiv:char}.
%The naive layerwise partitioning leads to excessive, large pipeline bubbles and starves the CPU;
%as a result, the pipeline is no different from serial execution, failing the deadline..
%This is demonstrated in Figure \Note{XXX}.

%\textit{Second, how to handle device heterogeneity?}
%\Note{Do not need much exposure...}
%Not only the model itself are skewed in io/compute, edge devices are also known to have diverse hardware\Note{cite}. 
%Due to their different io/compute capability, there is no silver-bullet partitioning strategy given a deadline.
%As shown in \sect{motiv:char}, Rpi3 has much slower io compared with Odroid -- one partitioning strategy may have small pipeline bubbles on the latter but much larger bubbles on the former, starving CPUs.

%The \underline{second} research question is how to compress the shards?
%Broadly, three techniques can be used to compress the shards:
%shards may be pruned and discarded~\cite{cnn-entropy-filter-pruning, cnn-prune-nvidia}; 

%We set to shard \textit{pretrained} language models (e.g. BERT) without retraining. 
%The \underline{first} research question is at 
%To do so, there are two design choices. 
%One is \textit{unstructured} sharding~\cite{gordonCompressingBERTStudying2020,ladabert}, that is, viewing the whole (over 100 million) parameters as a large flat data array and splitting it in trunks. % which is common in network pruning

%they may share weights with each other~\cite{transformer-attention-share,nn-weight-share};
%they may be quantized into a lower bitwidth~\cite{binarybert,ibert,bibert}.
%%Our system must navigate through the compression techniques to ensure that shards 
%Our system must shard a model cautiously, navigate through the compression techniques, and ensure a decent model performance. %shards should work well with each other



\subsection{Instantiating model shards on disk}
\label{sec:design:sharding:shard}
%For pretrained \tfm{} models, we propose a retraining-free sharding approach, which is a novel combination of width-adaptive \tfm{} and outlier-aware quantization.
%\textbf{structured}, \textbf{outlier-aware quantization} approach for sharding the pretrained \tfm{} model. 
%Our key idea is to shard the model by layers, and by their attention heads.
%\Note{Our key construct is ...}
%In response, our key construct is \textit{model shards}, where we partition the transformer layers into mixed-precision, finer grained pieces.
To address the challenges, our key idea is to combine two machine learning techniques -- dynamic \tfm{}~\cite{dynabert,hat} and dictionary-based quantization~\cite{deep-compression}, in a novel way.
%To address the challenges, our key idea is to leverage a novel combination of two techniques: dynamic \tfm{}~\cite{dynabert,hat} and dictionary-based quantization~\cite{deep-compression}. 
We next describe details.
%compress a dynamic \tfm{} (e.g. DynaBERT~\cite{dynabert}, HAT~\cite{hat}) with Gaussian-outlier-aware simulated quantization~\cite{quantization-survey}.
%To address the challenges, our key insight is to leverage a dynamic \tfm{} with adaptive widths and depths (e.g. DynaBERT~\cite{dynabert}, HAT~\cite{hat}), with Gaussian-outlier-aware simulated quantization~\cite{gobo}.
%Our rationale is dynamic \tfm{} enables partial and incremental model execution because sub\Tfm{}s (\xzlNote{??}) share weights with the super\Tfm{}; 
%Gaussian-based simulated quantization works with pretrained models and incurs little accuracy degradation by accurately approximating parameter distribution~\cite{gobo,deep-compression}.
%We next describe the details.
%\Note{rationale, merge}
%The former enables partial and incremental model execution because sub\Tfm{}s share weights with the super\Tfm{}; 
%the latter works with pretrained models and incurs little accuracy degradation by exploiting parameter redundancy (\S\ref{sec:motiv:primer}).
%\Note{rationale merge}
%We do so because the parameter distribution of a \tfm{} layer is known to resemble Gaussian distribution~\cite{gobo};
%hence we can approximate the majority of values with a few representatives called centroids, while preserving the rest outliers (i.e. outside the Gaussian distribution). 
%The whole process resembles lossy compression and does not require fine tuning..

%We then partition each version into vertical slices by layers, which are model shards. 
%To address the challenges, our key insight is to leverage a dynamic \tfm{} with adaptive widths and depths (e.g. DynaBERT~\cite{dynabert}, HAT~\cite{hat}), and compress it into different fidelity versions using Gaussian-outlier-aware simulated quantization;
%we then partition each version into vertical slices by layers, which are model shards.

%Our rationale are as follows. 
%Dynamic \tfm{} allows for partial model execution;
%the parameter distribution of a \tfm{} layer 
%by approximating it with Gaussian distribution while preserving outliers resembles lossy compression which incurs little accuracy degradation. 

%integrating a novel combination of two known techniques: structured pruning \& outlier-aware quantization. 

%Compared with partitioning by layers, model shards bridges the gap between the skewed io vs compute (XXX vs XXX), allowing for efficient pipeline execution with small bubbles;
%their variable fidelity further enables elastic IO time.  %adapting to various deadlines on heterogeneous devices.
%\Note{merge below}
%% obsolete 
%\paragraph{\textit{Benefits}} are as follows.
%\begin{myitemize}
%	\item 
%	\textit{Partial model execution.}
%	First (cold) inference may start execution on only a few (e.g. 3) shards per layer, while subsequent inferences may incrementally load more.
%	
%	%Our rationale is as follows.
%	%First, an attention head is an atomic structure of the MHA mechanism~\cite{transformer}, which is learned at training time;
%	%shards conforming to the structure preserves the same mechanism.
%	%%shards can work seamlessly with each other. 
%	
%	\item 
%	\textit{Close and elastic IO/compute.}
%	A typical shard contains only one twelve-th parameter as a layer, thus having the same small portion of its IO (e.g. 40ms), approximating the compute time on a shard per layer (e.g. 30ms).
%	Mixed-precisions allow for multiple other devices..
%	
%\end{myitemize}

\input{fig-sharding}

%\xzlNote{each techniques below shall map back to challenges.}


%\Note{update Figure 5}
\paragraph{First, vertical partitioning per layer}
%\xzlNote{This this should go before quantization}
%The system then partitions each of $B$ fidelity versions into $M$ vertical slices by $K$ layers (in total $b\times m \times k$ such slices). 
The system adopts a pretrained \tfm{} model, which has already been fine-tuned on a downstream task. %(e.g. models from Huggingface~\cite{huggingface)}.
%such models they may be publicly accessible  
%The model must have adaptive widths and depths, that is, at run time it may decide differently how many parameters of a layer to use (i.e. widths), as well as the number of layers (i.e. depths).
%The model must have adaptive widths and depths, that is, at run time it may decide differently how many number of attention heads and FFN neurons of a layer (i.e. widths), as well as the number of layers (i.e. depths) to use.
%The system adopts a pretrained dynamic \tfm{} model as the backbone network,  which is already fine-tuned on a downstream task (e.g. sentiment analysis) to have adaptive widths and depths. 
%That is, it can vary the number of attention heads and FFN neurons of a layer, as well as the number of layers.

For each of the $N$ layers, the system partitions it into $M$ vertical slices, as shown in Figure~\ref{fig:design:shards}~(\circled{1}). %by total $N$ layers.
By construction, each vertical slice is independent, constituting one attention head plus $1/M$ of FFN neurons of the layer; %whose parameters compose a shard.
the partitioning is inspired by dynamic \tfm{}s~\cite{hat,dynabert}.
Table~\ref{tab:vertical_slice} shows the weight compositions of a vertical slice.
Each cell of the table describes the dimension of the weight matrix, where $d$ is hidden state size, $M$ is the number of attention heads, and $d_{ff}$ is the number of FFN neurons;
a shard is therefore one of the $M$ equal slices of a layer. 
%as can be seen, the partitioning equally slices the layer 
Doing so warrants model shards the same capability to extract linguistic features from inputs, as done by the attention mechanism: 
%Doing so warrants model shards elasticity and the same capability to extract linguistic features from inputs, as done by the attention mechanism: 
%Doing so warrants model shards attending to linguistic features of input tokens: 
%Doing so warrants model shards with same attention mechanism linguistic features : 
of an individual shard, its attention head obtains one independent representation of input tokens, which is projected into a higher feature dimension by FFN neurons~\cite{attention-head-acl19,bert-acl19};
jointly, multiple shards attend to information from different representation subspace at different positions~\cite{transformer}.
%jointly, multiple shards recover full semantic features of inputs.
%A slice/shard $S$ can be uniquely identified by a three-tuple $S=(m,k,b)$, where $m, k$ are the indexes for the slice and layer respectively, and $b$ is its fidelity.
Therefore, an arbitrary subset of shards of a layer can be executed and still give meaningful results. % and their results can be combined to produce meaningful output.
%\Note{to add: say shard identity is relative to BERT model, e.g. shard at 2nd layer 1st slice...}

%Doing so preserves the language features in the learned structure. \xzlNote{vague, find better rationales from prior work}

\begin{comment}
% below useful...merged 
\xzlNote{Compress the following two paragraphs into a table?}
Following~\cite{dynabert}, we define a shard's weight composition as follows. 
For a \tfm{} layer, 
%it is composed by five key weight matrix $W^Q, W^K, W^V, W^O$ and $FFN$, where
let $d$ denote the hidden state size, $M$ be the total number of attention heads (e.g. $M = 12$), $d_{ff}$ be the number of FFN neurons.
The size of each attention head $d_h$ is given by $d/{M}$, and the neurons of a shard $d_{ff'}$ is given by $d_{ff}/M$.
By equally partitioning the layer, we obtain $M$ vertical slices as model shards, indexed by $[0, M-1]$ from left to right.

The $j$-th shard is hence parameterized by six submatrix: $\{ W_{j}^Q, W_{j}^K, W_{j}^{V}, W_{j}^{O} \} \in \mathbb{R}^{d\times d_h}$ from an attention head, and two from FFN $W_{j}^{FFN1} \in \mathbb{R}^{d_{ff'}\times d},
	 W_{j}^{FFN2} \in \mathbb{R}^{d \times d_{ff'}}$.
The sub-matrix $W_{j}$ are selected by the $j$-th portion from respective $W$ along the non-feature dimension.
For instance, $W_{j}^{Q} = W_{:, j\cdot d_h:j\cdot(d_h+1)}^{Q}$.
Note that the index $j$ explicitly assigns the $j$-th slice of the weight matrix $W$ w.r.t. each shard in an non-overlapping manner.
\end{comment}


\sys{} uses the \textit{submodel} to describe the \tfm{} model on shards, e.g. a  $n \times m$ submodel comprises $n$ layers, each layer having $m$ shards.
The number $m$ is the same across all layers, as mandated by the \tfm{} architecture~\cite{transformer}, which specifies each layer must have the same width (i.e. number of shards $m$) for aligning input/output features between layers.
Although it is possible for a shard to use 0s as dummy weights, \sys{} expects all $m$ shards to have concrete weights for a good accuracy.
%To execute a \tfm{} model using shards, \sys{} first decides a \textit{submodel} of $n$ layers; %$\times$ $m$ shards per layer.
%mandated by the \tfm{} architecture~\cite{transformer}, each layer must have the same width (i.e. number of shards $m$) for an aligned number of output features.
%Although it is possible for a shard to use 0s as placeholder weights, \sys{} expects all $m$ shards to have concrete weights for a good accuracy.
%With $m$ shards, \sys{} computes the attention and FFN output of individual shards using the weight composition in Table~\ref{tab:vertical_slice}, concatenates their outputs, and proceeds to next layer.
%The process therefore preserves the attention mechanism for producing meaningful results.
%For more detailed mathematic formulation, an interested reader may refer to~\cite{16heads,dynabert}.


\input{tab-shard-param}

%The $j$-th model shard at $i$-th layer, $S(i,j)$, is parameterized by:
%%\Note{use a figure}
%
%\begin{equation}
%S(i,j) = \{W_{d_h}^{Q_i}, W_{d_h}^{K}, W_{d_h}^{V}, W_{d_h}^{O}\}\cup\{FFN_{d_h'}\}
%\end{equation}

%\xzlNote{clarify: which subset of a model shards are composable? why partial execution can still give meaningful inference result?}

%\xzlNote{where do we say that in a submodel, each layer must have the same number of shards, and why}

%\xzlNote{much of the following (until the end of S4.3) can go to impl. Important things to mention: what is done at a high level; (typically) how many versions per shard; how are they stored on disk and how large (compression ratio); potential accuracy loss; model accuracy has different sensitivities to individual shards and their bitwidth; mixed precision: shards of different bitwidths can be combined in the same submodel; compute cost of compression/decompression..}
%\Note{this is our novelty. highlight what is ours and what is theirs..}
\paragraph{Second, quantization per shard}
\label{sec:design:sharding:quantize}
%We next describe in detail how to quantize them into different precisions (bits).
The system compresses each of the $N \times M$ shards into $K$ bitwidths versions (e.g. $K=2\dots 6$). %each of which reduces the model size by a few $\times$.
\sys{} is the first to bring quantization to \textit{shard} granularity, whereas prior work only explores layer granularity~\cite{mixed-quantization-energy,hawq,haq}.
Doing so reduces IO/compute skewness and facilitates elastic IO, allowing \sys{} to prioritize IO resources at a much finer granularity, e.g. by allocating higher bitwidths to more important shards, and catering to IO/compute capability of diverse devices.

%gives different fidelity per shard importance for maximizing resource utilization on different devices with diverse IO/compute capabilities. 
%\xzlNote{... and to give different fidelity (compression ratio) per shard importance...}

%of  : fidelity versions reduce their IO by a few $\times$, which can overlap with compute with small bubbles while adapting to .
%The goal is to facilitate elastic IO and amortize IO/compute skewness for maximizing resource utilization: fidelity versions reduce their IO by a few $\times$, which can overlap with compute with small bubbles while adapting to diverse IO/compute capability of different devices.


%The compression is feasible due to high parameter redundancy of \tfm{}, allowing accurate approximation via Gaussian distributions~\cite{tenarybert,gobo}.
%\Note{high level}
To compress, \sys{} uses Gaussian outlier-aware quantization~\cite{gobo}.
%It exploits the Gaussian distribution of \tfm{} weights. 
The key idea is to represent the vast majority of weights (e.g. 99.9\%) which follow a Gaussin distribution using $2^k$ floating point numbers called \textit{centroids};
doing so compresses the original weights into $k$-bit indexes pointing to centroids, thus reducing the parameter size by $$ 
For the very few \textit{outliers} (e.g. 0.1\%) which do not follow the Gaussian distribution, it preserves their weights as-is.
The process is shown in Figure~\ref{fig:design:shards}~(\circled{2}).
We will further describe the implementation details in \sect{impl}.

%\Note{property1: can have high compression ratio, minimum accuracy loss. greatly reduces IO... (no more skewness)}
%how many versions per shard; how are they stored on disk and how large (compression ratio); potential accuracy loss;

\begin{comment}
\Note{may hurt us -- making our design point insignificant}
\textit{Property I: high compression ratios, low accuracy loss.} 
For a K-bit version, the approach compresses a shard by 32/K, as 99.9\% of 32-bit weight are replaced by K-bit dictionary indexes.
For instance, at the lowest bitwidth we target (K=2), the shard is compressed by 16$\times$, whose file size is less than 200KB.
The high compression ratios correct IO/compute skewness and make storing all K versions cheap, e.g. for typically five versions, K=$2\dots6$, it adds only a few hundred MBs. %and is tunable to cater capabilities of diverse devices. 
Meanwhile, the accuracy loss is minimum, incurring less than 1\% accuracy degradation when K=6.
At lower K=2, the accuracy loss may be high, e.g. 10\%, but it can be remedied by \sys{}'s mechanism to load higher-bitwidths shards, which we will describe and evaluate later.
\end{comment}

%\Note{property2: resembles lossy compression. Work smoothly across different fidelity versions}
%model accuracy has different sensitivities to individual shards and their bitwidth;
%mixed precision: shards of different bitwidths can be combined in the same submodel

%\textit{Property II: good compatibility between shard versions.}
%The dictionary compression resembles lossy compression.
We choose it for two main reasons. % it satisfies following properties which we seek: 
1) It provides good compatibility between shards of different bitwidths, allowing \sys{} to tune their \bt{} individually per their importance and to assemble a \textit{mixed-bitwidth} submodel.
%1) Its lossy compression nature provides good compatibility between shards of different bitwidths;
%it allows \sys{} to tune the bitwidths of individual shards per their importance and to assemble a submodel with \textit{mixed-bitwidths}.
%allows shards of different versions to work seamlessly with each other, assembling a submodel with \textit{mixed bitwidths}.
This is due to its lossy compression nature -- shards still preserve the original distribution of layer weights, albeit in different fidelities.
Hence they can work with each other seamlessly.
%2) It has wide applicability without the need to fine-tune a model or additional hardware support.
2) It does not need to fine-tune a model or require additional hardware support.
The quantization analyzes the weight distribution of the pretrained model and is not specific to network structures; 
it hence does not require fine-tuning, as opposed to fixed-point quantization~\cite{q8bert,bibert}. 
The resultant  \textit{mixed-\bt{}} submodel also differs from a traditional \textit{mixed-precision} network~\cite{haq,hawq,mixed-quantization-energy}, 
%which mixes floating point operations with integer operations~\cite{mixed-precision-cnn-iclr18};
which requires DSP extensions for executing integer operations efficiently;
the extensions are often exclusive to microcontrollers on ARM devices, e.g. Cortex-M4~\cite{m4-dsp}.
%More importantly, the good compatibility enables \sys{} to tune the bitwidths of individual shards per their importance. 
%\sys{} prioritize important shards which have large impacts on accuracy and allocate higher bitwidths for them, s.t. they may recover the original weight distribution as precisely as possible.
%For less important ones, \sys{} uses lower bitwidths as they do not affect accuracy much.

%\xzlNote{as opposed to XXX techniques. By doing so we avoid tedious per-model retraining as opposed to XXX (is this right?) and ensure to generate adequate compute workloads for high accuracy}
Quantized shards are not meant to be used as-is.
Prior to use, \sys{} must decompress them, which is a mirror process of compression. 
\sys{} does so by substituting dictionary indexes with floating point centroids and outliers.
Therefore model shards quantization reduces IO but not computation (FLOPs) as the inference still executes on floating point numbers. %(i.e. centroids and outliers).
%To do so, it mass substitutes dictionary indexes with centroids (i.e. floating point numbers) and computes on restored FP32 weights.
%Fortunately, decompression is fast, less than 20ms per layer and can be further alleviated by using a designated accelerator~\cite{gobo}.

%\Note{property3: does not need fine tuning and hardware support}
%\textit{Property III: no fine-tuning nor hardware support required.}
%The quantization approximates the weight distribution of the pretrained model and is oblivious to 
%
%To use, the engine decompresses the shards by simply mass substituting dictionary indexes with centroids (i.e. floating point numbers) and computes on restored FP32 weights;
%the decompression is efficient on a commodity SoC, less than 20ms for one layer.
%%the inference only have floating point operations;
%This differs from a traditional \textit{mixed-precision} network, which mixes floating point operations with integer operations~\Note{cite}.


%We choose it because it incurs little accuracy loss (<1\%) even at $10\times$ compression ratio by accurately approximating \tfm{} weights which follow a Gaussian distribution~\cite{gobo,tenarybert}, and that it is dictionary compression (i.e. simulated), which does not require fine-tuning.
%%We donot use fixed-point quantization~\cite{binarybert,q8bert} because it is less elastic (e.g. fixed 8/4/2bit versions), needs DSP extension which is only seen on microcontrollers (e.g. Cortex-M4~\cite{m4-dsp}), and requires fine-tuning. 
%We donot use fixed-point quantization~\cite{binarybert,q8bert} because it is less elastic (e.g. fixed 8/4/2bit versions), needs DSP extension which is only available on microcontrollers (e.g. Cortex-M4~\cite{m4-dsp}), and requires fine-tuning. 
%Alternatively, a model may be compressed by knowledge distillation~\cite{distilbert} or model pruning~\cite{layerdrop,mobilebert}. 
%However, they also require fine-tuning for \textit{each} version, and they likely lead to severe accuracy degradation as they must remove over 90\% of weights to achieve the same compression ratio as ours.



%
%For minimal accuracy loss, \sys{} uses \textit{simulated quantization}, \Note{reasons for not using real quantziation, i.e. integer operation: require fine-tuning for performance, not friendly to hardware}... 
%It quantizes the full-fledged shards into different lower-bit representations, reducing sizes by up to 16 $\times$. %inspired by a Gaussian-outlier-based quantization technique~\cite{quantization-survey};
%%With model shards as the key building block, \sys{} constructs an elastic pipeline whose IO and compute time is dependent on number of shards and their respective precisions. 
%\Note{Our novelty comp. w/ prior mixed-precision transformer and dynamic transformer:} the first to combine them to achieve elasticity; our goal is not to find a supernet or an optimal mixed-precision net, but to find building blocks. 




%\xzlNote{clarify: impact on IO and compute. why compute remains unaffected. also compare to other compression techniques that reduce both IO and compute (like distillation, transfer learning. why aren't those desirable)}
%Since the vast majority ($99.9\%$) of 32-bit weights are substituted by $b$-bit indexes to centroids, simulated quantization reduces IO by $\lfloor 32/b \rfloor \times$.
%It, however, does not reduce computation delays because the model maintains the same GFLOPS by computing on floating point centroids and outliers. 
\begin{comment}
% --- old, can merge ---
For each layer, the system fits all its weights into a Gaussian distribution, based on which it divides weights into two groups, an outlier group and a Gaussian group;
it preserves the former in full 32-bit fidelity and represents the latter with $2^b$ centroids, which are 32-bit floating point numbers.
%for the latter, it represents them with $2^b$ centroids. 
A weight is deemed as an outlier if the probability of it belongs to the Gaussian distribution is below a configurable threshold;
the larger the threshold, the more full-fidelity outliers, hence the lower compression ratio.  

Following the same practice in~\cite{gobo}, we use $-4$ which is sufficient in maintaining accuracy while maximizing compression ratio;
under the threshold, the outlier group constitute less than $0.1\%$ of total weights. %which is preserved in full precision (i.e. 32-bit). %and incurring only 1\% accuracy degradation. 
For the Gaussian group which constitute the rest $99.9\%$, the system sorts and splits its weights into $2^b$ clusters with equal population;
each cluster has \textit{one} centroid to represent \textit{all} values within it. 
%It then represents \textit{all} values in each cluster with \textit{one} centroid, which is indexed by a $b$-bit integer.
%It then represents \textit{all} values in each cluster with \textit{one} cluster centroid by substituting them with a $b$-bit index to the centroid.
Doing so caters to the weight distribution: weight-concentrated regions deserve higher resolutions, hence having more clusters and centroids.
%the vast majority ($99.9\%$) of original 32-bit weights are represented by $b$-bit integers, reducing model size by $\lfloor 32/b \rfloor \times$.
To decide cluster centroids, prior work adopt K-means based approaches~\cite{deep-compression, zhaoImprovingNeuralNetwork}, which are time-consuming, e.g. it takes a few hours to converge on our server.
Differently, we have found the arithmetic mean of cluster weights suffices -- a 2-bit version takes a few minutes to converge and incurs only 7\% accuracy degradation compared with the full model. 
We will present more results in \sect{eval}.  
%It uses the Gaussian model to find out a group of ``outliers'' parameters and preserve them in full precision.
%For the rest, the system quantizes them into $n$-bit integers (e.g. typically 2 to 4) using \textit{simulated quantization}~\cite{quantization-survey}, where each integer points to a full-precision FP32 value called a centroid, representing a group of original weights.
%The system decides the centroids by dividing the non-outlier parameters into $2^n$ groups and calculating their arithmetic means.

%The rationale is ....
%\Note{quantization rationale..}
%Second, attention head weights are heavily redundant~\cite{16heads}.
%%Most need only a few bits~\cite{ibert,binarybert} while only outliers need high-precision.
%Preserving the few outliers (e.g. 0.01\%~\cite{gobo}) while representing the most others with a small number of values ensures performance.
\end{comment}

%The system repeats the process for each fidelity version and generates a dictionary as the compression metadata, which specifies the centroids and the outlier mapping of full-fidelity weights.

%\Note{how are they stored..}
%\Note{compute cost of compression/decompression..}
\paragraph{Third, storing shards per version}
%After partitioning, a shard contains $1/M$ of a layer's total parameters, each is a $b$-bit centroid index.
\sys{} stores each shard of every \bt{} on disk, in total $N\times M \times K$ shards (e.g. N=M=12, K=$2\dots6, 32$, where 32 is the uncompressed, full fidelity).
%For instance, (0,0,2) refers to the shard partitioned from the first layer and first slice 
Each shard contains a weight matrix of the same dimensions listed in Table~\ref{tab:vertical_slice}. 
Instead of original FP32 weights, the weight matrix now stores K-bit indexes, which reduces its file size by $32/K \times$. 
Additional to the weight matrix, it stores centroids and outliers as dictionaries to look up during decompression, as illustrated by Figure~\ref{fig:design:shards}~(\circled{3}).
To load, it refers to individual on-disk shards by their original layer/vertical slice indexes and \bt{}s. 

%Storing compressed shards is cheap, taking less than 300MB of disk space.

%For a K-bit version, the approach compresses a shard by 32/K, as 99.9\% of 32-bit weight are replaced by  dictionary indexes.
%To generate shards, the system compresses the vertical slices using the dictionaries produced by simulated quantization: 
%for \textit{all} 32-bit parameter, the system looks up the dictionary and uniformly substitutes them with $b$-bit integers, each pointing to one of the $2^b$ centroids.
%It does not preserve the 32-bit outliers in the newly compressed weight matrix to avoid destroying the $b$-bit data alignment.
%It stores the compressed weights as the data and dictionaries (centroids, outliers) as the metadata of model shards on disk.
%This is shown in Figure~\ref{fig:design:shards}. %\xzlNote{Fig 4 needs update, showing the workflow}


%The quantization approximates the weight distribution of the pretrained model using a dictionary and is not specific to network internals. 
%This is because they only change the representations of model parameters but not their amount.
%For instance, by substituting 99.9\% of 32-bit weights with $b$-bit centroid indexes, a shard reduces IO by $\lfloor 32/b \rfloor \times$.
%At inference time, the model retains GFLOPS by computing on the same amount of floating points decompressed from centroids and outliers;
%while being inevitable, the decompression is efficient (10-20ms per layer) and can be further alleviated by designated hardware accelerator~\cite{gobo}.

%In uncompressed, full-fidelity form, their sizes are $1/M$ of a layer (e.g. a few MBs), taking tens of ms to load; 
%in lower fidelities, their IOs are even smaller and elastic w.r.t. bit fidelity. 
%%Hence a model shard equally slices the $j$-th layer it belongs to.
%Note: when in lower fidelities, shards cannot be used directly -- the weights are only indexes. 
%They cannot be used interchangeably, e.g. a 1 in 2-bit and 6-bit shard points to different centroids.  
%For instance, for the 1st layer with 3 shards,  


%Since the vast majority ($99.9\%$) of 32-bit weights can map to centroids, which are indexed by $b$-bit integers, the model size is reduced by $\lfloor 32/b \rfloor \times$.

%Following~\cite{dynabert}, the attention score and output of a layer can be defined as:
%
%\begin{equation}
%	\label{eq:out}
%\end{equation}
%
%Therefore as listed in equation~\ref{eq:out}, the output of a \tfm{} layer can be regarded as the sum of independent model shards, allowing partial execution of the model.

%\paragraph{Storing model shards}
%The system stores all versions of shards and their corresponding centroids on disk. %and pick selectively at run time. 
%Unused ones (e.g. for other tasks) can be further compressed via lossless compression (e.g. Zip). 
%This is possible because of low entropy.
%%Will evaluate its size (smaller than a HD movie) and compression efficiency (>90\%). 
%\Note{why not only store 6bit and derive the others?} 
%Doing so requires to \textit{always} load 6-bit shard IO delays.
%Not elastic, may miss deadline.

%\xzlNote{need cost analysis? }
%At least mention prior work on hardware accelerator


 



==> eval-prelim.tex <==
%\paragraph{\textit{Preliminary results}}
%We have done preliminary experiments on the pretrained model from DynaBERT~\cite{dynabert}. 
%Figure~\ref{fig:prelim:sharding} validates the importance of outliers with SST-2 frrom GLUE benchmark~\cite{glue-benchmark}, a dual-class sentiment classification task. %to evaluate the model performance of the proposed sharding strategy.
%It shows our proposed quantization technique achieve near original model performance (less than 1\% degradation when quantized into 4 bits) while without outliers the quantized model performance drops to 50\% (i.e. random guess).
%Figure~\ref{fig:prelim:others} shows the proposed quantization technique also achieves decent performance in two other tasks (less than 1\% degradation when quantized into 5 bits), STS-B and MNLI in GLUE~\cite{glue-benchmark}.
%Figure~\ref{fig:prelim:heads} shows the attention-head granularity achieves a decent performance and scales with number of heads, as expected.
%
%
%\paragraph{\textit{Preliminary results}}
%Our principle is based on measured per-layer outlier distribution of pretrained DynaBERT model.
%As shown in Figure~\ref{fig:prelim:weight}, top layers have more outliers thus calling for higher precision.
%We have also characterized the IO and Compute time of BERT~\cite{bert} on an Odroid dev board~\cite{odroid-web} as a sample IO/Compute profile, shown in Figure~\ref{fig:prelim:load}.
%We have also profiled the per-component inference latency of BERT on an x86 machine for convenience, shown in Figure~\ref{fig:prelim:breakdown}. 
%These preliminary results suggest a sublinear increase in Compute time as the number of attention heads (i.e. the sharding granularity) increase.
%They will be as a key heuristic in planning the shard pipeline.
%
%\input{fig-prelim-planning}

==> fig-design-explore.tex <==
% !TeX root = main.tex

\begin{figure}[h]
	\centering
	\includegraphics[width=0.48\textwidth]{./figs/overlap}
%	\vspace{-2em}
	\subcaption{Naively layerwise overlap}
	\label{fig:motiv:overlap}
	
	\includegraphics[width=0.48\textwidth]{./figs/compress_overlap}
	\subcaption{Model compression on layers}
	\label{fig:motiv:compress-overlap}
%	\vspace{-5mm}
\end{figure}

==> fig-io-compute.tex <==
% !TeX root = main.tex
\begin{figure}[h]
	\centering
	\includegraphics[width=0.48\textwidth]{./figs/io_compute}
%	\vspace{-2em}
	\caption{IO/Compute latencies under different Compression ratios of DistilBert model}
	\label{fig:motiv:io-compute}
%	\vspace{-5mm}
\end{figure}

==> fig-lat-breakdown.tex <==
% !TeX root = main.tex

\begin{figure}[h]
	\centering
	\includegraphics[width=0.25\textwidth]{./figs/plot/motiv-lat/fig_lat}
%	\vspace*{-2em}
	\caption{Hot vs cold start inference latency of \textbf{Mob}ileBERT, \textbf{Dis}tilBERT, and BERT on Odroid dev board.}
%\caption{Hot vs cold start inference latency Breakdown of IO/Compute on different mobile platforms, showing IO dominates the latency and various IO/Compute ratio.
%	\textbf{TODO:} show BERT -- show hot inference latency for comparison}
	\label{fig:motiv:lat-breakdown}
%	\vspace{-5mm}
\end{figure}

==> fig-major-deadline.tex <==
% !TeX root = main.tex

\begin{figure}[h]
	\begin{minipage}[t]{0.15\textwidth}
		\centering
		\includegraphics[width=0.9\textwidth]{./figs/plot/major-deadline/fig_major_deadline}
		\subcaption{SST-2}	\label{fig:eval:deadline:sst2}			
	\end{minipage}\hfill
	\begin{minipage}[t]{0.15\textwidth}
		\centering
		\includegraphics[width=0.9\textwidth]{./figs/plot/major-deadline/fig_major_deadline}
		\subcaption{SST-2}	
	\end{minipage}\hfill
	\begin{minipage}[t]{0.15\textwidth}
		\centering
		\includegraphics[width=0.9\textwidth]{./figs/plot/major-deadline/fig_major_deadline}
		\subcaption{SST-2}	
	\end{minipage}\hfill
	%	\vspace*{-2em}
	\caption{\sys{} accuracy on GLUE benchmark. Each deadline variable is set by the system configuration. We assume that 1.5s is the upper limit for IRA. (need to confirm or cite)}
	\label{fig:eval:deadline}
	%	\vspace{-5mm}
\end{figure}

==> fig-memory-consumption.tex <==
% !TeX root = main.tex

\begin{figure}[h]
    \centering
	\begin{minipage}[t]{0.22\textwidth}
		\centering
		\includegraphics[width=0.9\textwidth]{./figs/plot/preloaded-memory/fig_preloaded_odroid}
		\subcaption{Odroid}	\label{fig:eval:preloaded:odroid}			
	\end{minipage}
	\begin{minipage}[t]{0.225\textwidth}
		\centering
		\includegraphics[width=0.9\textwidth]{./figs/plot/preloaded-memory/fig_preloaded_jetson}
		\subcaption{Jetson}	\label{fig:eval:preloaded:jetson}			
	\end{minipage}\hfill
	%	\vspace*{-2em}
	\caption{PreloadedModel vs. Ours of preloaded memory size at different latencies. Lower is better.}
	\label{fig:eval:memory-consumption}
	%	\vspace{-5mm}
\end{figure}

==> fig-planning.tex <==
% !TeX root = main.tex
\begin{figure*}
%	\begin{figure}{r}{0.5\textwidth}
	\centering
	\includegraphics[width=1\textwidth]{./figs/planning}
%	\vspace*{-2em}
	\caption{The proposed planning strategy. XXX:update}
%\caption{Hot vs cold start inference latency Breakdown of IO/Compute on different mobile platforms, showing IO dominates the latency and various IO/Compute ratio.
%	\textbf{TODO:} show BERT -- show hot inference latency for comparison}
	\label{fig:design:planning}
%	\vspace{-5mm}
\end{figure*}

==> fig-prelim-planning.tex <==
% !TeX root = main.tex

\begin{figure}[h]
%\begin{figure}{r}{0.3\textwidth}
%	\centering
	\begin{minipage}[t]{0.15\textwidth}
		\centering
		\includegraphics[width=0.9\textwidth]{./figs/plot/planning-weight/fig_weight}
		\subcaption{The outlier percentage of each layer in DynaBERT~\cite{dynabert} model. 
		Our planning strategy fits the outlier distribution.}
		\label{fig:prelim:weight}
	\end{minipage}\hfill
	\begin{minipage}[t]{0.15\textwidth}
		\centering
		\includegraphics[width=0.9\textwidth]{./figs/plot/planning-load/fig_load}
		\subcaption{Cold start inference latency of MobileBERT, DistilBERT, and BERT on Tensorflow and PyTorch.}	
		\label{fig:prelim:load}			
	\end{minipage}\hfill
	\begin{minipage}[t]{0.15\textwidth}
		\centering
		\includegraphics[width=0.9\textwidth]{./figs/plot/planning-breakdown/fig_breakdown}
		\subcaption{Per-component latency breakdown of a BERT layer with different number of attention heads on an x86 machine.}
		\label{fig:prelim:breakdown}
	\end{minipage}
	\caption{Preliminary results back up our proposed planning strategy.}
\end{figure}


==> fig-prelim-sharding.tex <==
% !TeX root = main.tex

\begin{figure}[h]
%\begin{figure}{r}{0.3\textwidth}
%	\centering
	\begin{minipage}[t]{0.15\textwidth}
		\centering
		\includegraphics[width=0.9\textwidth]{./figs/plot/shard-outlier/fig_sharding}
		\subcaption{SST-2~\cite{glue-benchmark} accuracy with our proposed quantization technique.}	\label{fig:prelim:sharding}			
	\end{minipage}\hfill
	\begin{minipage}[t]{0.15\textwidth}
		\centering
		\includegraphics[width=0.9\textwidth]{./figs/plot/shard-others/fig_others}
		\subcaption{Our propsoed quantization technique also works with MNLI and STS-B~\cite{glue-benchmark}.}
		\label{fig:prelim:others}
	\end{minipage}\hfill
	\begin{minipage}[t]{0.15\textwidth}
		\centering
		\includegraphics[width=0.9\textwidth]{./figs/plot/shard-heads/fig_heads}
		\subcaption{SST-2 accuracy increases as number of attention heads, the proposed sharding granulairty.}
		\label{fig:prelim:heads}
	\end{minipage}
	\caption{Preliminary results on our proposed sharding strategy on DynaBERT~\cite{dynabert}.}
\end{figure}


==> fig-res-model.tex <==
% !TeX root = main.tex

\begin{figure}[h]
%	\centering
	\includegraphics[width=0.45\textwidth]{./figs/pipeline}
%	\vspace*{-2em}
	\caption{IO/Compute pipeline execution... XXX need discussion}
%\caption{Hot vs cold start inference latency Breakdown of IO/Compute on different mobile platforms, showing IO dominates the latency and various IO/Compute ratio.
%	\textbf{TODO:} show BERT -- show hot inference latency for comparison}
	\label{fig:design:pipeline}
%	\vspace{-5mm}
\end{figure}

==> fig-thesis-overview.tex <==
% !TeX root = proposal_memo.tex
\begin{figure}[h]
	\centering
	\includegraphics[width=0.6\textwidth]{./figs/thesis_overview}
	\caption{My thesis comprises a series of systems design towards a more efficient and secure heterogeneous edge platform; the figure shows their corresponding positions in the software/hardware stack.
	\protect\circled{1}~: Psbox (\S\ref{sec:thesis:psbox}), \protect\circled{2}~: Transkernel (\S\ref{sec:thesis:dbt}), \protect\circled{3}~: Enigma (\S\ref{sec:thesis:enigma}), \protect\circled{4}~: Driverlet (\S\ref{sec:thesis:driverlet}), \protect\circled{5}~: STI (\S\ref{sec:thesis:sti})}
	\label{fig:thesis}
\end{figure}

==> intro-xzl-comment.tex <==
% !TeX root = main.tex

\xzlNote{---------- begin xzl ------------}: 


\begin{itemize}
\item 
upon user request (impromptu), model has to be loaded and executed; 
(upon request -- maximum inference accuracy under a deadline) load and execute  model; compute/IO pipelining (with high parallelism); 

\item 
in the background: opportunistically load  and unload (a fraction of model). 
(background -- responding to changes in available memory) 
OS could opportunistically preload/evict model parts subject to available memory (policy -- Not this paper's focus)
\end{itemize}


\textbf{Current:} 
% model and OS are designed in isolation; oblivious to each other. 
rigid resource management in isolation. 
Techniques (knobs...hyperparameters...) exist to adjust individual resources 
(compute: model compression -- NestDNN, DynaBERT; 
memory/IO: quantization ...)
But the OS lacks mechanisms to manage the resources in a joint fashion towards the aforementioned goal. 

As a result ... Model load and execution: layer-wise execution; no or limited pipelining. 
Reason: skewed compute/IO ratio. Compute starvation. 
Most notable example is cold inference: ...

Model memory management: page in/out (monolithic -- Android; prior research: by layers). Result: model weights are swapped regardless of their impact on accuracy. 

\xzlNote{---------- end xzl ------------}: 

==> memo_sti_motiv.tex <==
% !TeX root = proposal_memo.tex

\section{Supplementary materials for \textit{S}peedy \textit{T}ransformer \textit{I}nference (\sys{})}
\label{sec:thesis:sti}

\subsection{How does \sys{} fit into the thesis?}
\sys{} addresses the first challenge (i.e. poor energy efficiency) as stated in \sect{thesis:challenge}. 
Specifically, it eliminates the CPU idle due to waiting for model load, by forming a IO/compute pipeline with elastic IO shards. 
Doing so reduces the cold inference latency significantly and improves energy efficiency;
targeting user software, it complements the accomplished work, which is done in kernel software. 

\subsection{\sys{} motivations}

\paragraph{Motivating scenario.}
\sys{} targets an interactive NLP scenario with intelligent personal assistant (IPA) on a multi-tenant mobile device.
In the scenario, a user typically interacts with the IPA for querying weather/personal emails/medical records~\cite{ipa-survey}, managing tasks~\cite{myersIntelligentPersonalAssistant2007} etc.
A typical interaction takes 2-3 turns and lasts for a few seconds~\cite{ipa-study-denmark};
during the interaction, the length of each utterance is often 10-20 words~\cite{tsaiFasterResponsesAre2019}. 

Under the hood, the IPA may run the pretrained Transformer language model to directly generate responses by running downstream tasks such as question answering~\cite{dynabert}, and dialog generation~\cite{dialogpt}.
Alternatively, it may generate responses from templates. 
It does so by filling the blanks in the templates~\cite{mdfn-aaai21} or selecting existing answers from its knowledge base, based on intent classification~\cite{dbpedia-chatbot} and sentiment analysis~\cite{yasudaDesigningChatbotSystem2021} results of the Transformer model.

\input{fig-lat-breakdown}

\paragraph{Why cold inference matters?}
Mobile app interactions are brief, for less than a minute~\cite{livelab};
interactions with IPAs are even shorter, for only a few seconds~\cite{ipa-study-denmark,tsaiFasterResponsesAre2019}.
During such a short period, human attention is a scarce resource~\cite{proj-aura}.
It is vital that the system be responsive and rapid upon invocations, for a smooth user experience~\cite{falcon-mobisys12}. 

Existing cold inference latency of \tfm{} inference, however, is far from ideal.
As shown in Figure~\ref{fig:motiv:lat-breakdown}, on a commodity embedded SoC the cold inference is as high as 4 seconds, which has already exceeded the typical duration of interactions with IPAs.
This is unacceptable to user experience.

Hence for the interactive NLP tasks we target, \sys{} aims to reduce its cold inference latency to the same level as \textbf{human interactions}.
That is, the latency (i.e. set by the deadline) is only a few hundred milliseconds~\cite{human-latency-study}, with hundred-milliseconds breaks between utterances.



\paragraph{Existing techniques are inadequate.}
We consider two common approaches to reducing cold inference latency as follows.
\begin{myenumerate}
	\item 
	\textit{How about pinning the model files in memory for good?}
	The approach conceptually eliminates cold inference, as the model files are always in memory.
	Yet, it eschews the IO time waiting for storage at the cost of high memory pressure, and is undesirable. 
	This is because:
	1) transformer model files are as large as a few hundred MBs, which take a significant portion of memory space of commodity mobile devices (e.g. a few GBs~\cite{iphone13});
	2) in the constrained memory space, the OS of the device must accommodate multiple tenant apps~\cite{acclaim-atc20} and ensure fairness of responsiveness~\cite{asap-atc21}, too;
	it shall not sacrifice the user experience of other apps.
	As a result of resource contention, cold inference happens frequently on today's mobile devices, causes ``latency variability''~\cite{dnn-mobile-lat-var}, and degrades user experience.
	
	\item 
	\textit{How about compressing the models?}
	Alternatively, one may compress a \tfm{} model to reduce the number/precision of parameters, hence the file size. 
	Common techniques include \ul{structured pruning} which reduces the width and/or depths of a \tfm{}~\cite{distilbert,mobilebert,dynabert,layerdrop},
	\ul{weight sharing} which makes \tfm{} layers to share same set of parameters~\cite{albert, universal-transformer},
	and \ul{quantization} which reduces the full precision of parameters (often in 32 bits) to low-bit representations or integers~\cite{binarybert,bibert}.
	However, these approaches share a key inadequacy -- still, the (cold) inference can only start as soon as the model is loaded.
	They hence face a dilemma between latency and accuracy: a low compression ratio (e.g. DistilBERT~\cite{distilbert} is 2$\times$ smaller than BERT~\cite{bert}) cannot meet the latency goal (e.g. a few hundred milliseconds) because it still takes seconds to load the model;
	a high compression ratio (e.g. BinaryBERT~\cite{binarybert} is 24$\times$ smaller) meets the latency goal while suffering from inferior accuracy, e.g. a few full GLUE scores lower, which is deemed significant in NLP literature~\cite{bibert,binarybert}.

\end{myenumerate}

\subsection{Clarifications from Q\&A}

\paragraph{What are key innovations?}
The key contribution of \sys{} is: 
1) it identifies the model shards which have elastic IO time, as the proper building block for the IO/compute pipeline of transformer inference;
2) based on model shards, it proposes a novel planning algorithm that maximizes the inference accuracy while meeting a user-set deadline on different devices.

We do not claim: 1) quantization techniques used to generate shards, and 2) IO/compute pipeline as our contribution since these techniques are well-known. 

\paragraph{How does the IO/compute pipeline work with shards?}
The number of shards per layer can be regarded as the ``width'' of the \tfm{} model during an inference;
it is the same across all layers during one inference.
Prior to each inference, \sys{} decides how many shards and the bitwidth of each shard to be used, depending on the deadline and device-specific IO/compute capability. 
For one inference, \sys{} constructs the IO/compute pipeline in the following way: it first loads the initial set of shards for layer 1; it then begins computing on shards of layer 1, while overlapping shard loading for layer 2, and so on and so forth.

\paragraph{Why do partial model composed of shards give meaningful results?}
Because of the parameter redundancy of \tfm{} models: 
a \tfm{} model may still give meaningful results even if attention heads are reduced from full sixteen to a few~\cite{16heads}, or layers share the same set of parameters~\cite{albert}. 
In \sys{}, one shard is a vertical slice of the transformer layer, comprising one attention head plus a set of FFN neurons; 
it preserves the structure on which the model is trained and the learned features. 
By stacking them in layers, the resultant model resembles a partial model with a smaller width~\cite{dynabert, liDynamicSlimmableNetwork2021}, hence still giving meaningful results.



\paragraph{\sys{} seems a generic model compression technique, why target cold inference only?}
To clarify: the model compression technique used by \sys{} is not new~\cite{gobo};
it acts only as an enabling tool for \sys{} to generate shards as the IO/compute pipeline building block.

\sys{}'s key ideas are tailored to cold inference due to the deadline constraint, where IO is the bottleneck.
The compression, however, does not affect compute time w.r.t. a full-precision model.
It hence has little benefits in a hot inference scenario, i.e. same latency but inferior accuracy than a full-precision model.

\paragraph{Can a GPU help reduce cold inference latency?}
No. 
This is because during cold inference, IO is the bottleneck, dominating over 90\% of the latency.
By simply offloading the compute to GPU, the IO keeps blocking compute and still results in high cold inference latency.

\paragraph{Why not offload to cloud?}
First, on-device inference ensures better privacy. 
The query as well as content being queried (e.g. medical records) do not have to be exposed to cloud.
Second, it is more reliable where spotty network connections are common on mobile devices~\cite{livelab,backgnd-in-wild2}.
Third, cloud offloading is a complementary approach, e.g. for other non-private queries, the user can always offload to cloud.

\paragraph{Can we leverage idle intervals between IPA interactions to load model?}
This is an orthogonal approach.
The idea is to prefetch the model file prior to inference.
Its challenge is twofold: 1) it is unclear how well IPA invocations can be predicted, while misprediction leads to excessive memory usage and poor user experience.
2) coordinating with other apps which compete for memory may be challenging, e.g. the already prefetched model file may be swapped out due to contention.


\paragraph{Why sacrifice accuracy for latency?}
Because in the scenario we target, reducing the latency from seconds to milliseconds significantly improves user experience.
Meanwhile, the accuracy loss is only 1\%, which is considered negligible in NLP literature~\cite{albert,nagarajanOptimizingTransformersApproximate}.
Prior study on IPAs~\cite{tsaiFasterResponsesAre2019} support our design, advocating ``faster responses are better responses''. 





==> memo_stmt.tex <==
% !TeX root = proposal_memo.tex

\section{Thesis statement}
\label{sec:thesis}

Emerging edge platforms are equipped with increasingly abundant and heterogeneous computing resources.
Yet, its existing systems software is inadequate in fully utilizing them.
To this end, my thesis features a series of novel systems designs that help these edge platforms run more efficiently and securely.

\subsection{Background: heterogeneous edge platforms}

Emerging edge platforms\footnote{We use ``edge'' to refer to embedded/mobile Arm SoCs by convention} are armed with abundant, heterogeneous computing resources:
for energy efficiency, in addition to Arm CPUs they have microcontroller-like peripheral cores which run a few $\times$ slower than the CPU but are 100 $\times$ more efficient;
they are equipped with diverse IO devices and accelerators, including DSPs, GPUs, DMAs; 
for security, they are guarded by Arm TrustZone Trusted Execution Environment (TEE) which partitions the SoCs into secure/normal world and isolates security-sensitive execution from the normal world OS (e.g. Linux). 
Figure~\ref{fig:thesis} shows a typical software/hardware stack of the heterogeneous edge platform.

\input{fig-thesis-overview}

\subsection{Challenges to systems software (OS and Runtime)}
\label{sec:thesis:challenge}

Despite the rich hardware computing resources, existing systems software on edge platforms fails to fully utilizes them and faces two key inadequacies as follows.

\paragraph{First, poor energy efficiency.}
As edge platforms are often battery-powered, energy efficiency is crucial to them. 
However, as demonstrated by prior work~\cite{livelab,mobisys16-wear,central-pm-asplos}, they often suffer from energy drain and have poor energy efficiency. 
We discover two key bottlenecks: 
\begin{myitemize}
	\item 
	\textbf{Lack of system support for energy accounting.} 
	Existing systems provide no reliable, accurate energy accounting facilities. 
	As a result, there is no means for apps running on the edge platform to tell their actual power consumption and adapt towards better efficiency, which is a long desired goal~\cite{odyssey}. 
	
	\item
	\textbf{Large CPU idle epochs.} 
	CPU execution is not efficient, either.
	In many driver workloads, there exist small, yet accumulatively large CPU idle epochs~\cite{zhai17hotmobile};
	in ML inference, which is an increasingly important use case for edge platforms, a CPU also has to idle for long, waiting for IO~\cite{dnn-mobile-imc}.
	While the idle epochs being necessary, the edge platform wastes energy on doing nothing. 
	
\end{myitemize}

\paragraph{Second, compromised security goals.}
As an isolated execution environment, TrustZone TEE and its runtime kernel (e.g. OPTEE-OS~\cite{optee}) lacks filesystems and device driver support.
As a result, apps of TEE (i.e. trustlets) must forward the file calls, IO job requests to OS and rely on its software stack in the normal world for execution.
This creates two security risks which break the data integrity and confidentiality goal of TrustZone TEE:

\begin{myitemize}
	\item 
	\textbf{External IO as a side channel.}
	As forwarding must send the arguments of a request in the clear (e.g. file offsets), they can be used to infer the input data of the trustlet, creating a side channel.
	For instance, by inferring the accessed file offsets of a SQLite query, the attacker learns the query content~\cite{obliviate}.
	
	\item 
	\textbf{Possible data leak and tampering.}
	During execution of forwarded requests, the data passes through the OS. 
	For devices without end-to-end encryption, this leads to possible data leak and tampering: a malicious OS (including its drivers) may peek into the data content, tamper with it, and feed the trustlets with tampered data.
\end{myitemize} 

The above challenges are exacerbated by the ``ossification'' of existing systems software.
That is, the edge platforms run commodity Linux kernels and it is unlikely to see a full swap of the software stack.


\subsection{Accomplished work}

My thesis, comprising four accomplished pieces have addressed the above challenges from the angle of ``ossified'' kernel software, in a holistic manner -- they leverage the existing, mature interfaces between software/hardware, perform surgical modifications to kernel subsystems, and can easily integrate with Linux kernel.
In the remainder of the section, I will describe briefly each piece by answering the following questions:
\begin{itemize}
	\item 
	Why does it matter? 
	
	\item 
	What are the key innovations \& results? 
	
	\item 
	What are the contributions to the field?
\end{itemize} 

\subsubsection{Redefining power awareness (Eurosys'18~\cite{psbox})}
\label{sec:thesis:psbox}

\paragraph{Why important?}
Power awareness is desired by apps for long; 
by knowing its own power consumption, an app can dynamically adjust its runtime behavior (e.g. throttle data transmission bandwidth, vary streaming fidelity), thus achieving better energy efficiency.
However, in the existing approach an OS often meters system power and divides it among apps. 
Since the impacts of concurrent apps on system power are entangled, this approach not only makes it difficult to reason about power and but also results in power side channels, a serious vulnerability.

\paragraph{Key innovations.}
We contribute a novel kernel OS principal called \psb{} (psbox, \circled{1}), provided to apps.
A psbox enables one app to observe the fine-grained power consumption of itself running in its vertical slice of the hardware/software stack. 
The observed power is insulated from the impacts of other apps.
We support the psbox through two new kernel extensions: resource ballooning and power state virtualization. 
The former grants a psbox exclusive use of resource partitions at fine spatial or temporal granularities; it meters and reports the power of resource balloons. 
The latter virtualizes hardware power states for every single psbox upon exit and re-entry, eliminating power side channel.

\paragraph{Key results.}
We implement psbox for a variety of major hardware components, including CPU, GPU, DSP, and WiFi interface on two embedded platforms.
Psbox keeps an app's power observations highly consistent even when the app co-runs with other different apps. 
Across these runs, the app’s energy, as observed by the app itself, differs by less than 5\%; 
by contrast, energy shares reported by a prior approach differ by up to 60\%.

\paragraph{What matters to the field?}
Power sandbox is the first work that recognizes the power entanglement problem, which makes prior energy accounting approaches inadequate;
it is the first kernel mechanism to address the problem and empowers apps with their power consumption.

\subsubsection{Bridging monolithic kernels to peripheral cores (USENIX ATC'19~\cite{transkernel})}
\label{sec:thesis:dbt}

\paragraph{Why important?}
A major energy drain of smart devices is ephemeral tasks driven by background activities. 
To execute such a task, the OS kernel wakes up the platform beforehand and puts it back to sleep afterward. 
Such kernel executions are inefficient as they mismatch typical CPU hardware. 
They are better off running on a low-power, microcontroller-like core, i.e., peripheral core, relieving CPU from the inefficiency.

\paragraph{Key innovations.}
We contribute a new OS structure, in which a lightweight virtual executor called \dbt{} (\circled{2}) offloads specific phases from a monolithic kernel. 
The OS has a set of novel designs. It translates stateful kernel execution through cross-ISA, dynamic binary translation (DBT); it emulates a small set of stateless kernel services behind a narrow, stable binary interface; it specializes for hot paths; it exploits ISA similarities for lowering DBT cost.

\paragraph{Key results.}
In 10K SLoC, we implemented a transkernel prototype called ARK atop an ARM SoC.
ARK offers complete support for device suspend/resume in Linux, capable of executing diverse drivers that implement rich functionalities (e.g., DMA and firmware loading) and invoke sophisticated kernel services (e.g., scheduling and IRQ handling).
As compared to native kernel execution, transkernel only incurs 2.7× overhead, 5.2×
lower than a baseline of off-the-shelf DBT. 
It reduces system energy by 34\% under real-world usage.

\paragraph{What matters to the field?}
The transkernel represents a new OS design point for harnessing heterogeneous SoCs. 
It contributes a key insight: while cross-ISA DBT is typically used under the assumption of efficiency loss, it can enable efficiency gain, even on off-the-shelf hardware.

\subsubsection{Enabling private file services for TrustZone via deception (Under review)}
\label{sec:thesis:enigma}

\paragraph{Why important?}
As TrustZone TEE lacks filesystem implementations, the in-TEE apps (trustlets) often invoke external filesystems of a normal world OS for file services (e.g. persist the collected sensor data, access user credentials).
While filedata can be encrypted, the file activities, including file operation types (e.g. read/write), sizes/offsets, and access occurrence (e.g. “the trustlet just created a file”) must be sent in the clear.
From the received file activities, the OS can infer a truslet's secrets such as input data, compromising the trustlet's privacy. 

\paragraph{Key innovations.}
We propose Enigma (\circled{3}), a deception-based defense injecting sybil file activities as the cover of actual file activities.
Enigma contributes three new designs. 
(1) To make the deception credible, the TEE generates sybil calls by replaying file calls from the TEE code under protection. 
(2) To make sybil activities cheap, the TEE requests the OS to run K filesystem images simultaneously. Concealing the disk, the TEE backs only one image with the actual disk while backing other images by only storing their metadata. 
(3) To protect filesystem image identities, the TEE shuffles the images frequently, preventing the OS from observing any image for long.

\paragraph{Key results.}
We build Enigma on Raspberry Pi 3, which works with unmodified EXT4 and F2FS shipped with Linux. 
We show that Enigma can concurrently run as many as 50 filesystem images
with 37\% disk overhead (less than 1\% of disk overhead per image). 
Compared to common obfuscation for hiding addresses in a flat space, Enigma hides file activities with richer semantics. 
Its cost is lower by one order of magnitude while achieving the same level of probabilistic security guarantees.

\paragraph{What matters to the field?}
Enigma is the first system to guard the external IO of TrustZone.
Its deception approach opens the door for a TEE to external untrusted OS services.

\subsubsection{Enabling TrustZone secure IO via minimum viable device drivers (Eurosys'22~\cite{driverlet})}
\label{sec:thesis:driverlet}

\paragraph{Why important?}
Designed for IO-rich client devices, TrustZone features secure IO, allowing TrustZone apps (trustlets) to access IO devices without being known or tampered by the OS.
However, Secure IO remains largely untapped today due to the difficulty in implementing device drivers for TrustZone.

\paragraph{Key innovations.}
We present a new model called the driverlet (\circled{4}) for deriving device drivers for TrustZone.
It contributes a key insight: instead of reusing drivers \textit{code}, we may reuse driver/device \textit{interactions} from mature Linux driver via record and replay. 
Ahead of time, developers exercise a full driver and record the driver/device interactions; 
the processed recordings, called interaction templates, are replayed in the TEE at run time to access IO devices.
The interaction template ensures faithful reproduction of recorded IO jobs (albeit on new IO data);
it accepts dynamic input values; it tolerates nondeterministic device behaviors

\paragraph{Key results.}
We build driverlets for three devices MMC, USB Mass, and a CSI Camera on RaspberryPi 3.
We show driverlets are easy to build and have sufficient performance to trustlets: 
it only takes a few days to build a driverlet while porting/implementing a driver takes at least months;
with driverlets, trustlets can execute over 100 SQLite queries per second (1.4$\times$ slower than a full-fledged native driver) and
capture images at 2.1 FPS from a CSI camera (2.7$\times$ slower).

\paragraph{What matters to the field?}
Driverlets fix the key missing link for secure IO, and for the first time open a door for trustlets to access complex yet essential devices.




%6\subsection{Common principles}

==> motiv-memo.tex <==
% !TeX root = main.tex

\subsection{\sys{} motivations}


==> motiv-scenario.tex <==
% !TeX root = main.tex
\paragraph{Motivating scenario.}
\sys{} targets an interactive NLP scenario with intelligent personal assistant (IPA) on a multi-tenant mobile device.
In the scenario, a user typically interacts with the IPA for querying weather/personal emails/medical records~\cite{ipa-survey}, managing tasks~\cite{myersIntelligentPersonalAssistant2007} etc.
A typical interaction takes 2-3 turns and lasts for a few seconds~\cite{ipa-study-denmark};
during the interaction, the length of each utterance is often 10-20 words~\cite{tsaiFasterResponsesAre2019}. 

Under the hood, the IPA may run the pretrained Transformer language model to directly generate responses by running downstream tasks such as question answering~\cite{dynabert}, and dialog generation~\cite{dialogpt}.
Alternatively, it may generate responses from templates. 
It does so by filling the blanks in the templates~\cite{mdfn-aaai21} or selecting existing answers from its knowledge base, based on intent classification~\cite{dbpedia-chatbot} and sentiment analysis~\cite{yasudaDesigningChatbotSystem2021} results of the Transformer model.

==> plan.tex <==
% !TeX root = main.tex

\section{Project plan \& timeline}

\paragraph{\textit{Research milestones}}
We have set up the research milestones for the project as follows.
\begin{myitemize}
	\item 
	\textbf{Milestone I.}
	We have done preliminary experiments (\S\ref{sec:design:sharding}), which have shown the promise of the high accuracy of the proposed sharding strategy based on attention heads.
	We plan to further apply the proposed strategy to more pretrained models, such as RoBERTa~\cite{roberta} and DistilBERT~\cite{distilbert}. 
	
	\item 
	\textbf{Milestone II.}
	We plan to conduct more comprehensive experiments on different planning schedules. 
	Current preliminary results in \S\ref{sec:design:planning} have demonstrated feasibility. 
	It is yet to be explored if current strategy is already optimal and whether a better planning exists.
	The outcome is a concrete and detailed planning algorithm. 
\end{myitemize}

We plan to achieve the above milestones by \underline{April 30th, 2022}.


\paragraph{\textit{Implementation \& evaluation plan}}
We plan to implement the proposed system in Python with PyTorch framework~\cite{pytorch-web}, using DynaBERT~\cite{dynabert} as the backbone network.
\ul{For the model sharding task}, we plan to modify the existing modeling utility. 
Specifically, we will first quantize individual attention heads.
We will then introduce shards as a new abstraction and implement the new interface which operate on shards. 
\ul{For the shard planning task}, we will first implement the devised planning algorithm, which accepts the device's IO/Compute profile and a deadline as inputs, and generate an optimal IO/Compute plan. 
Second, we plan to refactor the PyTorch framework.
We will implement the proposed pipeline and integrate it with the planning algorithm. 

\ul{To evaluate,} we will answer two research questions.
1) How much time does the proposed system save for cold start inference? 
We plan to set a fixed accuracy and compare the cold start inference latency of the proposed system with SOTA models~\cite{bert,distilbert,mobilebert}. 
2) What is the tradeoff between accuracy and deadlines of the proposed system? 
First, we plan to evaluate the system with different planning strategies, which give insights into \ul{the accuracy-latency implication} of IO/Compute of attention heads with different bitwidths.
Second, we plan to set a similar deadline for SOTA models and compare the resultant accuracy with the proposed system;
we will consider popular compressed BERT variants such as DistilBERT~\cite{distilbert}, MobileBERT~\cite{mobilebert}, I-BERT~\cite{ibert}, BinaryBERT~\cite{binarybert} as well as EdgeBERT~\cite{edgebert}, a deadline-aware system based on early exits.

We plan to finish the implementation and evaluation by \underline{July 31st, 2022}.

\paragraph{\textit{Project outcome}}
We plan to summarize the project and send the paper to premier systems venues such as ASPLOS'23, Eurosys'23, and MobiSys'23. 
We plan to open source the code artifact to cultivate further research into the cold start inference problem, as well as potential deployment and integration in popular deep learning frameworks.




==> planner-formulation__Liwei_Guo_s_conflicted_copy_2022-07-05_.tex <==
% !TeX root = main.tex

\subsection{Overview}

%The engine's primary job is to serve inference requests under deadline $T$ from the user. 
%To this end, it leverages the existing shard buffer to bootstrap inference and co-schedules IO for \textit{next} layers with computation of \textit{current} layers in the pipeline.

%The key challenge of the engine is how to schedule the IO/compute pipeline for maximizing the accuracy, under the deadline $T$ and memory constraint $M$?
%The key role of the engine is to schedule the IO/compute pipeline for a maximum accuracy under the deadline $T$ and memory constraint $M$.
\paragraph{Planning goals}
Towards maximizing the accuracy under T, we have two planning goals:
%Towards maximizing the accuracy, we face a unique challenge: how to schedule the IO/compute pipeline under $T$? 
%The challenge incarnates as two planning goals:
\begin{myitemize}
	\item 
	\textit{First, minimize pipeline bubbles.} 
%	While a higher GFLOPs implies a higher accuracy, a more important question is how to spend it.
	We donot want to starve either compute or IO.
	On one hand, maxing out compute (FLOPs) drives the inference towards a higher accuracy. 
	On the other hand, the engine can always improve the bitwidths of shards as long as not all of them are not at full 32 bits. %to improve accuracy.
	%a higher accuracy, a more important question is how to spend it.
%	E.g. to spend more G%FLOPs on \textit{each} layer or on \textit{more} layers?
	
	\item 
	\textit{Second, prioritize IO/computation resources on important shards.}
%	The number of all possible shards to load under $T$ compose a combinatorial space, making it intractable. 
	The total scheduling of shards to load under $T$ compose a combinatorial space, making it intractable to enumerate.
	Yet, the engine must propose one which leads to maximum accuracy at run time. 	
%	\item 
%	\textit{First, how to saturate compute?} 
%%	While a higher GFLOPs implies a higher accuracy, a more important question is how to spend it.
%	While it is intuitive to max out GFLOPs for a higher accuracy, a more important question is how to spend it.
%	E.g. to spend more GFLOPs on \textit{each} layer or on \textit{more} layers?
%	
%	\item 
%	\textit{Second, how to schedule IO?}
%%	The number of all possible shards to load under $T$ compose a combinatorial space, making it intractable. 
%	The total scheduling of shards to load under $T$ compose a combinatorial space, making it intractable to enumerate.
%	Yet, the engine must propose one which leads to maximum accuracy at run time. 
\end{myitemize}

%\xzlNote{Can recast as planning goals}
% (1) non stalling (or minimizing bubble. "bubble" was extensively used in prior work) (2) more compute/IO resource spent on important shards

%The above challenges are unique to us and cannot be fully addressed by prior work, which does not explore the solution space in a pipeline constrained by $T,M$ at run time.

% -- useful recycle -- 
%\paragraph{Problem formulation}
%We formulate the engine inference process as follows.
%%Given a deadline $T$, a memory constraint $M$, and the existing shard buffer $R$, the engine searches for a new $R'$, such that $R'$ maximizes inference accuracy, its execution delay overlapped with $\delta(R',R)$is under $T$, and its memory consumption $R'$ is under $M$. 
%Given a deadline $T$, a memory constraint $M$, and the existing shard buffer $R$, the engine searches for a shard set $S'$ spanning $N$ layers to overlap their IO with computation, s.t. new $R'=R+S'$ achieves maximum accuracy, its execution is under $T$ and its memory consumption is under $M$ after inference.
%%outputs a list of IO tasks, specifying the new set of model shards configuration $S' = \{s'(n', d', b') \mid n',d' \leq 12, b' = 2\dots 6,32  \}$ to load, which overlap with compute of the incoming inference.
%%Note $n,d\leq 12$ due to BERT.
%%\Note{Be clear about three parameters referred later:} 
%%\begin{myitemize}
%%	\item 
%%	\textbf{N}. \# of layers. 
%%	
%%	\item 
%%	\textbf{D}. \# of shards per layer.
%%	
%%	\item 
%%	\textbf{S}. The shard configuration set.  
%%\end{myitemize}
%%\Note{following may be redundant, to merge with S4}
%%\paragraph{Shards \& model}
%%\xzlNote{what is the goal?}
%%Recall the formulation in \sect{design:sharding:shard}, a model $(N,D)$ of $D$ layers, each layer of $N$ shards can be uniquely identified by its shard set $S=\{s(n,d,b)\}$, where $n$, $d$ are the indexes and $b$ is the bit precision of a shard $s$.
%%In the model, at $d$-th layer, the $n$-th shard of $b$-bit precision can be uniquely identified by a 3-tuple $s = (n, d, b)$;
%%for convenience, unloaded shards can be regarded to have $0$-bit precision.
%%Hence the model $M$ can be uniquely identified by $d$ layers of $n$ shards, given by $M = (S_0, S_1, ..., S_d)$, where $S_d = \{s(0,d,b_0), s(1,d,b_1), ..., s(n, d, b_n)\}, n, d \leq 12$ (i.e. for BERT).
%%\textbf{Key points:}
%%\begin{myitemize}
%%	\item 
%%	Two constraints: T and M.
%%	
%%	\item
%%	Given the existing $R$, the engine searches for a new $R'$ to be used in the incoming inference, s.t. $R'$ achieves maximum accuracy, .
%%	
%%	\item 
%%	Given the existing $R$, the engine searches for $N$ layers of shard $S'$ to overlap their IO with computation, s.t. new $R'=R+S'$ achieves maximum accuracy, its execution is under $T$ and memory consumption under $M$.
%%\end{myitemize}
%%Given two constraints, deadline $T$ and memory $M$, and the existing shard configuration $S =\{s(n, d, b) \mid n,d\leq 12, b = 2\dots 6,32 \}$, \sys{}'s planner (``the planner'') outputs a list of IO tasks, specifying the new set of model shards configuration $S' = \{s'(n', d', b') \mid n',d' \leq 12, b' = 2\dots 6,32  \}$ to load, which overlap with compute of the incoming inference.
%%Note $n,d\leq 12$ due to BERT.
%
%%To the search problem, we face a key challenge: \textit{how to achieve an optimal accuracy under the deadline $T$}? 
%% the trade off between accuracy and latency...
%%Towards maximizing the accuracy, we face two challenges 
%%
%%Intuitively, the engine maximizes out the model GFLOPs  
%%The search problem is non-trivial due to the following reasons.
%%
%%
%%Uniqueness -- pipeline, runtime constraint. 
%%Planning searches for an optimal solution and respects the pipelining...
%
%\textbf{Key points}
%\begin{myitemize}
%	\item 
%	Principle: need to maximize it (by loading as many parameter as possible) for accuracy... 
% 	
%	\item 
%	Challenge is there are many (exponentially large) ways to spend the GFLOPS. 
%	
%	\item 
%	First, towards what direction? Should the engine spend more  GFLOPs on each layer or on more layers? 
%	
%	\item 
%	Second, for a $N \times M$ executable model, there exist $6^{N\times M}$ possible $S'$..
%	
%	\item 
%	Third, how to plan them in a way to meet $T, M$?
%\end{myitemize}
%\textbf{our novelty..}

%\Note{to merge below}
%The challenges are similar with those faced by Neural Architecture Search~\cite{haq,hat} and automated quantization~\cite{hawq}, which may also have similar constraints.
%Yet, the key differences are: 1) we are planning for a pipeline, whereas they are for hot inferences only (i.e. do not need to consider io/compute overlapping); 2) our allocations consider multiple shots of inferences while prior work is one-shot. 

%\begin{myitemize}
%	\item 
%	\textit{Complex trade-offs between accuracy and shard configurations.}
%	Under the same GFLOPs, there exist different $S'$ which 
%%	The engine must jointly determine a model structure whose execution saturates T, and $S'$ to fill the model..
%%	While it is true that more and higher-precision shards improve accuracy, some shards and layers have greater impacts than others~\cite{hawq,layers-equal}. 
%%	We will further show incorrect configurations may even deteriorate accuracy. 
%	
%	\item 
%	\textit{An exponential parameter search space.}
%	The number of possible shard configurations grow exponentially as each shard may have multiple precisions.  
%	The large space makes it hard, if not impossible to enumerate through the entire space (i.e. $6^{N\times D}$ possible configurations for each $N, D$).
%	It also must be online as it considers existing shard configuration, different from offline NAS~\cite{haq,hawqv2}.
%	
%	% below obsolete 
%	%	\item 
%	%	Third, allocations must fit io/compute pipeline.  
%	%	The shard allocations are bound by both latency goals (i.e. deadlines) as well as io/compute capability of a device.
%	%	Misfit allocation plans may cause large pipeline bubble and miss the deadline.
%	%	
%	%	\item 
%	%	\Note{This one may be bogus} Second, no one-shot, silver-bullet allocations.
%	%	As \sys{} loads shards incrementally during multiple shots of inferences, 
%	%	allocations \st{hence must consider already loaded shards, then plan accordingly what to load in next shots for maximizing accuracy. }
%	%	
%\end{myitemize}

%Second, how to schedule for low latency on different devices?
%As IO and Compute time is device-specific, it takes a cautious planning not to starve either for different devices, in order to meet the deadline timely. 
%The IO time of an uncompressed shard is a few $\times$ larger than the compute time on it, which we will show in preliminary results.

%First, how to schedule for a maximum accuracy? 
%As cold start inference latencies are amortized by loading and executing the model partially with shards, so is the model accuracy.
%Our system sets to ramp up the accuracy as fast as possible while maintaining the high accuracy. 
%First, how to schedule for low latency on different devices?
%As IO and Compute time is device-specific, it takes a cautious planning not to starve either for different devices, in order to meet the deadline timely. 
%%The IO time of an uncompressed shard is a few $\times$ larger than the compute time on it, which we will show in preliminary results.

==> planner-io__Liwei_Guo_s_conflicted_copy_2022-11-09_.tex <==
% !TeX root = main.tex


\subsection{IO planning}
\label{sec:design:planning:io}
In this stage, \sys{} selects the \bt{}s for individual shards of the $(n\times m)$ submodel. %to load and pipeline them with computation. 
Without stalling the pipeline, it seeks those that maximize accuracy. %as the execution plan.
%\Note{TODO: use a figure, demonstrating AIB}

%\textbf{Design points}
%\begin{myitemize}
%	\item 
%	Problem formulation: find an optimal $S$ set, s.t. $R(k) + S \to R'(n, d)$, 
%	Goal: $R'$ achieves maximum accuracy.
%	Two constraints: not exceeding T, no computation starvation \Note{XXX}. 
%
%	\item 
%	Solution: AIB + heuristic-based online shard allocation 
%	
%	\item 
%	AIB: formulate the constraints to mechanize the layerwise planning => AIB(n) $\to$ 0, AIB(n) $\geq$ 0. 
%	To allocate, substract corresponding AIB(n). Give Example. 
%	
%	\item
%	Allocation strategy design points:
%	\begin{itemize}
%		\item 
%		Num > Fidel. 
%		The implication is the engine prioritizes filling up the submodel (\Note{should compute planning gauge the delta? set a minimum ddl = 12x12 2-bit shard?}). %\Note{what if shard buffer too small? and submodel too large to be loaded?}
%		It then will consider upgrading others. 
%		
%		\item 
%		Important shards first. 
%		Progressively upgrade $K$ shards to a higher fidelity, then proceeds to next $K$ shards.  
%	\end{itemize}	
%\end{myitemize}

%To find an optimal IO scheduling of shards, the engine leverages the profiled shard importance and hardware capability to conduct an efficient, heuristics-based iterative search. 

\subsubsection{Problem formulation}
%\paragraph{Goal}
%\paragraph{Problem formulation}
Given the deadline $T$, $n \times m$ submodel $R$ determined by compute planning, and the preload buffer $S$, \sys{} plans for a shard configuration $S'$ to load during computation, s.t. 1) loading $S'$ does not stall the pipeline, and 2) $R=S+S'$ achieves maximum accuracy.


%\paragraph{Constraints}
%$S'$ is \textit{valid} if it does not stall the pipeline. 
%It satisfies the key data dependency constraint: before executing $k$-th layer, all shards of prior $k-1$ layers  must have been loaded to avoid starving computation.
%As a corollary, the total IO delay $\sum_{i=1}^{|S'|} T_{io}(S'_i)$ does not exceed deadline $T$. 

%Meanwhile, $S'$ is bound by two constraints: 
%1) total IO delay $\sum T_{io}(S'_i)$ does not exceed deadline $T$; 
%2) no stalling between layerwise computation. 

%\paragraph{Our idea} is to assign each $n$ layer an \textit{accumulated IO budget} (AIB) to encode the data dependency between across-layer shard loading and sequential layerwise execution, and iteratively selects shard fidelity based on their importance.

%\subsubsection{Tracking layerwise IO Budget}
\subsubsection{Accumulated IO budgets}
%The goal is to allow shards of $S'$ to be selected individually from different layers while ensuring they are valid, satisfying the planning constraints, i.e. $S'$ does not stall pipeline nor exceed $T$.
To ensure the planning $S'$ does not stall the pipline, \sys{} uses \textit{Accumulated IO Budgets} (AIB) to track fine-grained, per-layer available IO resources. %i.e. $S'$ does not stall pipeline nor exceed $T$.
%The AIBs quantify IO budget the engine can consume \textit{prior to} execution of current layers.
%An AIB quantifies the IO budget the engine can consume to load \textit{all prior layers} execution of current layers.
%AIBs specifies the internal deadlines for each layer, under which the layer must have loaded its shards needed for execution. %which must have already loaded shards ready for execution, to avoid breaking the data dependency constraint. 
%An AIB specifies the internal deadline for each layer, which must have already loaded shards ready for execution, to avoid breaking the data dependency constraint. 
%\paragraph{Our idea} is to assign each $n$ layer an \textit{accumulated IO budget} (AIB) to encode the data dependency between across-layer shard loading and sequential layerwise execution, and iteratively selects shard fidelity based on their importance.

\paragraph{Key ideas}
%The engine uses AIBs to quantify the data dependency constraint as internal deadlines from each layer's perspective.
%The engine uses AIBs to track internal IO budgets of each layer, which bookkeep how much time the \textit{current} layer has to load all \textit{prior} shards.
%The engine uses AIBs to bookkeep how much time a layer has to load all \textit{prior} shards; 
Our first idea is layerwise \textit{Accumulated IO Budgets} (AIBs). 
Our observation is that the pipeline does not stall \textit{iff} before executing $k$-th layer, all shards of $0\dots k$ layers are loaded.
To this end, we define AIBs as follows: %\textit{since the beginning}. 
%By doing so, the engine converts the planning constraints into AIBs: as long as each $AIB(k) \geq 0$, the planning satisfies the constraint and is valid.

\begin{quote}
%\xzlNote{AIB must be defined here. the intuition, etc.}
%\paragraph{Definition}
The AIB(k) of $k$-th layer is the available IO time the layer can leverage to load all shards from $0\dots k$ layers. %to be the remaining time the layer still has to load all necessary shards. \xzlNote{a bit formal?}
\end{quote}

%\xzlNote{improve the following}
%AIBs for all layers to track how much time a layer still has to load all needed shards prior to its execution. 
%The intuition is $k$-th layer must finish loading necessary shards \textit{during} the execution of previous $k-1$ layers. 
%A positive AIB(k) therefore means the layer k still has 
Therefore, by checking if all AIBs are non-negative (i.e. each layer still has available IO time), \sys{} deems the planning S' \textit{valid} as it does not stall the pipeline.  %satisfies the constraint and is therefore valid.
%converts the planning constraints into AIBs: as long as each $AIB(k) \geq 0$, the planning satisfies the constraint and is valid.

The second idea is to consider the preload buffer $S$ as bonus AIBs added to all AIB(k), hence unifying planning preloaded shards with that of the pipeline. 
AIB(k) is initialized to be the execution delays of all prior $(k-1)$ layers (hence ``accumulated'') plus the bonus AIBs provided by the preload buffer $S$. %the buffer is already preloaded, hence its IO is ``free''.
E.g. AIB(0) is 0 because loading any shards at the first layer incurs a compulsory pipeline stall; 
AIB(n-1) is the largest because it has all the time to load its shards during previous layers' executions.
Then, for each shard at $k$-th layer in the buffer $S$, its bonus AIB is added to AIB(k) and propagated to all subsequent layers. 
For instance, a shard at layer 0 from $S$ propagates its bonus AIBs to all AIB(k)s, k=$0\dots n-1$; 
the bonus AIB of a shard at layer 1 from $S$ is propagated to AIB(1) $\dots$ AIB(n-1), so long so forth. 
%of the last layer is the largest because it has all the time to load its shards during previous layers' executions.

To use, \sys{} initializes AIBs as described earlier, upon each planning. 
%Recursively, it accumulates AIBs of deeper layers from prior layers, i.e. $AIB(k) = AIB(k-1) + T_{comp}, k=1\dots n-1$.
%Figure~\ref{fig:design:aib} shows example AIBs for two layers, where $T_{comp}=1s$.
%Notably, $AIB(0)=T_{io}(S)=0.6s$, due to buffer $S$ is already preloaded, its IO being given as bonus to layer 0 and all subsequent layers, i.e. $AIB(1)=T_{comp} + T_{io}(S)=1.6s$.
%\xzlNote{the bonus budget is also added to AIBs of all subsequent layers}
%When the engine selects a shard at $k$-th layer, it deducts the shard IO from AIBs of $k$-th layer as well as all subsequent layers.
When \sys{} selects a shard at $k$-th layer, it deducts the shard IO from AIBs of $k$-th as well as all subsequent layers.
The is because loading such shards only affect \textit{yet-to-be-executed} layers but not the already executed ones. 
At the end of selection, \sys{} checks all AIBs to see if they are non-negative. 
If so, \sys{} deems the planning $S'$ valid, otherwise rejects it. 

%the planning constraints into AIBs: as long as each $AIB(k) \geq 0$, the planning satisfies the constraint and is valid.
%i.e. IO budgets not used up,
%AIBs track layerwise IO budget: whenever a shard at layer $k$ is to be selected, its IO will be deducted from $AIB(k)$ and from all AIBs of subsequent layers, i.e. $AIB(k+1), AIB(k+2), \dots, AIB(n)$. 
%To satisfy the constraint, the engine ensures at the end of selection, each AIB is above 0.


\input{fig-aib}

%By keeping each AIB above 0, i.e. IO budgets not used up, the engine ensures each layer satisfies the data dependency prior to execution, keeping IO busy and avoiding computation starvation.
%\Note{need better intuition}
%Under the deadline, each layer ensures 

%track individual usage...by respecting non-zero invariant...
%All layers must load their shards under respective AIBs to avoid breaking the constraint.
%have loaded its shards needed for execution. %which must have already loaded shards ready for execution, to avoid breaking the data dependency constraint. 

%\paragraph{Initialization}
%Each tiem when IO planning begins, the engine initializes the AIB(k) of $k$-th layer to be the execution delays of all prior $(k-1)$ layers (hence ``accumulated''), given by $AIB(k)=(k - 1)T_{comp}(l,d)$, where $k= 1\dots n$ and $T_{comp}(l,d)$ is a constant determined in compute planning stage (\S~\ref{sec:design:planning:compute}).
%It then inspects the preload buffer, calculates the IO delay $\Delta$ of loading the buffer, and adds $\Delta$ to each of AIB(k).
%%The rationale is to count $\Delta$ as ``free IO'' of the first layer to all AIBs, since the buffer is already loaded. 
%The rationale is, since the buffer has already been preloaded, its IO $\Delta$ can be counted as ``free IO'' towards the first layer (i.e. prior to execution), and can be accumulated to all subsequent AIBs. %since the buffer is already loaded. 
%For instance, the AIB of the very first layer is initialized to 0, i.e. $AIB(1)=0$, because there is no computation to overlap loading its shards, while the last layer has largest AIB $(n-1)T_{comp}$, all at its disposal to load its shards.
%Recursively, AIB(k) of $k$-th layer is defined as the AIB of the former layer (hence ``accumulated'') plus the layerwise computation delay, i.e. $AIB(k)=AIB(k-1) + T_{comp}(l,d), k=1 \dots n-1$. 

%is the time to load preload buffer of size $M$.

%\paragraph{Initialization} 
%To begin, the engine initializes AIBs from layer 0, and recursively to layer $(n-1)$. 
%Since for each layer the computation delay $T_{comp}$ is the same, AIBs are given by $AIB(n) = (n-1)T_{comp}$

\paragraph{Example}
Figure~\ref{fig:design:aib} shows a mini example of using AIBs to check the validity of $S'$, where it plans for a 2x3 submodel, targeting a 2s deadline with $T_{comp}=1s$.
The engine initializes AIBs recursively from L0, whose $AIB(0)=0.6s$ due to the three 2-bit shards in $S$.
%$AIB(1)=AIB(0)+T_{comp}=1.6s$
To plan, the engine first fills $S'$ with $S$, deducting $0.6s$ from both $AIB(0)$ and $AIB(1)$ because all shards in $S$ are in L0.
Since only L1 has spare AIB, the engine can only select shards for it.
We show three execution plan candidates A, B, and C.
In this case, both candidates A and B are valid because their AIBs are non-negative, meaning loading them does not stall computation L1. 
Yet, C is invalid, because $AIB(1)=-0.1s$, violating the constraint and stalling the pipeline.

%\Note{may not need}
%\paragraph{Why are AIBs effective?}
%Doing so urges the engine to respect data dependency: as IOs of earlier shards bill to directly to all subsequent layers, the engine must ensure by the time $k$ starts to execute it has spare IO to spend on loading its own shards..
%Like yearly fiscal budget?? (have a total spending budget  by the end of year, some saving in the beginning.. now needs to plan each month??)what is the analogy?
%The intuition of propagating the IO delays to later layers is the data dependency. 



\subsubsection{Selecting optimal shard versions}
For each $T$, there exist an enormous number of execution plans. 
The goal is to select an optimal configuration $S'$, which 1) is valid, and 2) maximizes accuracy.
For instance, both A and B in Figure~\ref{fig:design:aib} are valid, but which has the maximum accuracy?
%\textbf{TBD after exp.}


\paragraph{Key idea} 
%\sys{} follows two principles to generate an optimal execution plan: 
%1) to maximize accuracy, it attempts to increase \textit{average fidelity} and allocate full fidelities to a few most important ones; 
%2) to ensure validity, it respects the key invariant $AIB(k) \geq 0$ for each allocation attempt on layer $k$.
To ensure validity, \sys{} respects the key invariant $AIB(k) \geq 0$ for each allocation attempt on layer $k$.
%\xzlNote{guided by shard importance?.. and list 1-3 heuristics/principles}
To maximize accuracy, our key idea is to first uniformly increase \bt{}s for all shards, then with the rest AIBs it greedily and iteratively allocate highest possible \bt{}s to individual shards guided by shard importance.
%Our rationale for the allocation strategy is, by increasing the average fidelity, 
By doing so, we build an information passageway for most important shards, allowing their maximum activations to be preserved in highest fidelity as possible. 
% ... For instance, activations from 32bit shard incur more information loss on 2bit shard than a 6bit shard..
%By doing so, it builds a high-fidelity information passageway for most important shards, allowing their can provide maximum activations without
%increasing the average fidelity, 

The allocation process comprises two passes as follows.
In the first pass, \sys{} picks a uniform \bt{} for all unallocated shards in the submodel, i.e. those not in preload buffer.
%\Note{layerwise... select the shards from same layer..}
To do so, it enumerates from lowest \bt{} (i.e. 2-bit) and selects the highest \bt{}s while AIBs still satisfy the invariant.
Notably, it fills a submodel layer with the shards from the same original layer and does not mix up shards across layers, due to quantization preserves layerwise weight distribution (\S\ref{sec:design:sharding:quantize}).
If AIBs cannot even support 2-bit shards, e.g. due to $T$ and/or preload buffer $S$ too small, \sys{} still selects them as they are necessary for execution but aborts further allocation.
In the second pass, \sys{} iteratively upgrades the \bt{}s of individual shards to full 32 \bt{} guided by the shard importance profiled in \S\ref{sec:design:planning:pre}, until all AIBs are consumed. 

The allocation result is an optimal execution plan which instantiates the submodel with individual shard configurations, and is ready to be executed by the IO/compute pipeline.
%The planner then sends the plan to the IO/computation pipeline for execution. 

%\begin{myitemize}
%	\item 
%	Key points: 1) respect AIB > 0 constraint. 2) iterative allocation to most important shards. 
%	
%	\item
%	Heuristics
%	\begin{itemize}
%		\item 
%		Num > Fidel. 
%		The implication is the engine prioritizes filling up the submodel (\Note{should compute planning gauge the delta? set a minimum ddl = 12x12 2-bit shard?}). %\Note{what if shard buffer too small? and submodel too large to be loaded?}
%		It then will consider upgrading others. 
%		
%		\item 
%		Important shards first. 
%		Progressively upgrade $K$ shards to a higher fidelity, then proceeds to next $K$ shards.  
%	\end{itemize}	
%\end{myitemize}
%
%\paragraph{tradeoffs between \# of shards vs fidelity}
%The trade off is whether we want the majority of shards to be medium-to-low fidelity or we want to the majority to be low while some (important) to be high....
%Our idea is the latter. 
%Evidence: 3-bit full model has 91.4\% while 2-bit version with only 5 shards upgraded to 6-bit achieves 91.6\% accuracy...
%
%
%\paragraph{the case of 32-bit shard}
%It is a special case (uncompressed)... 
%\sys{} upgrades to 6bit and refrains from 32-bit, unless all other shards have been upgraded to 6 bits ...  
%This is because 32-bit is not cost effective ... due to the outstanding performance in 4-bit version which achieves <1\% accuracy loss.. 
%Comparing to upgrading one 32-bit shard, one may upgrade 8 more 4-bit shard...which has more impacts on accuracy... evaluation (?) shows evidence..
%
%\xzlNote{below obsoleted?}

\begin{comment}
The planner then allocates shard configurations for the scheduled tasks. 
It follows the heuristics: 

\begin{quote}
	\textit{Heuristics II: prioritize top layers and important shards.}
	The planner favors more ``important'' shards and layers.
\end{quote}

The planner allocates shards in a greedy manner: it starts from the top layers (i.e. closer to output) and allocates highest quantized precision (i.e. 6-bit) to more important shards, that is, shards that are more sensitive to accuracy. 
This is shown in the listing XXX to YYY lines...

The planner does so iteratively for every shard until $T$ specified in the scheduled tasks is used up, i.e. by subtracting $T$ with $T_{io}(B)$ for an individual shard in $B$-bit precision.
The planner then generates a list of IO tasks, each specifies loading a shard $s(N,D,B)$ into $N$-th index of $D$-th layer in $B$-bit, of the model.

Before issuing these IO tasks, the planner does a sanity check: whether they will stall the pipeline and exceed $T$. 
If so, the planner decreases the precisions of shards which stall the pipeline.

As we will show in \sect{eval}, the planning is efficient taking only XXX ms and can ramp up accuracy fast with the help of our heuristics.

%\Note{merge below heuristics}
%\begin{myitemize}
%	\item 
%	More bits to top layer (closer to output), less to bottom layers (closer to input). 
%	Two benefits: 1) higher accuracy, see ``are all layers created equal'' and preliminary results; 2) faster start, i.e. the 1st layer (bottom layer) is blocking (no compute overlapping), better reduce io as much as possible.
%	
%	\item 
%	Shard configuration per layer: some shards have better sensitivity than other, favor them...
%	
%\end{myitemize}

\Note{TODO: merge below}
\paragraph{Spare IO}
\Note{do not mention embedding, defer to S6}
\Note{IO budget vs spare IO}
We define spare IO as the amount of IO time that can be spent on loading model shards; 
it overlaps with compute, exploiting the missed opportunity (\S~\ref{sec:motiv:char}).
Given a deadline $T$, the spare IO is calculated via a simple formula $T_{spare} = T - T_{emb}$, where as $T_{emb}$ is the amount of time spent retrieving embedding vectors. 
While embedding table is in-memory, $T_{emb}$ is negligible (i.e. $<10$ms), and we can regard $T_{spare} \approx T$.

\paragraph{IO tasks} 
With spare IO $T$, there are two IO tasks. 
\begin{myitemize}
	\item 
	$\text{\textit{append}}(T, S, S')$ loads a shard set $S'$ and appends them to the existing shards $S$ in $T$ time, s.t. the model computes on \textit{more} shards.
	
	\item 
	$\text{\textit{upgrade}}(T, S)$ replaces existing shards $S$ in $T$ time, s.t. the model computes on \textit{higher-precision} shards.
\end{myitemize}


\paragraph{Toy examples} 
For the very first (cold) inference, the planner is given $T=500ms$. 
It subtracts $500ms$ with $T_{emb}$ and finds $T_{spare}=400ms$.
Since none shard has been loaded yet (i.e. $S=\emptyset$), the planner only schedules \textit{append} task, adding shards to the empty model.
In the second (warm) inference, the same $T=500ms$ is given and a similar $T_{spare}$ is found.
Since the model can execute on shards $S$ loaded by the first inference, the planner leverage $T_{spare}$ to schedule \textit{upgrade} to improve their precisions, hence model accuracy.
\end{comment}

%\Note{to merge}
%\sys{} profiles time for an IO and compute on the corresponding platform in an offline fashion, out of the execution path of the inferences. 
%For IO, the system measures the latency of loading an uncompressed shard from storage and derives the latency for the compressed shards, which is linear to their bitwidths.
%%from the uncompressed latency, the system derives IO time of compressed shards, which is linear to their bitwidths.
%For Compute, the system does a dry run with different number of heads and measures the layerwise latency. 
%The rationale of profiling IO and Compute offline is they are data-independent~\cite{driverlet,asymo,tinystack}, whose latency hence is deterministic at run time. 
%both model loading and NN inference depends , 
%execution is solely dependent on the NN model itself. 


\begin{comment}
\paragraph{Reshaping resident model}
\Note{reshaping models...}
The planner compares the new model structure $(N',D')$ with existing $(N,D)$ (note that an empty model of cold inference can be denoted by $(0, 0)$). 
As described, compute planning causes the model structure to grow monotonically with $T_{comp}$. 
Hence there are three cases:
\begin{myenumerate}
\item 
At least one of $N',D'$ is larger.
The planner calculates shard set $S'$ to load and schedules \textit{append}$(T_{comp}, S',S)$, where $S'$ contains the indexes $(n,d)$ of new shards but not their $b$-bit precisions.

\item
Both $N',D'$ are the same as $N,D$.
The planner does not change the existing model $S$, and hence only schedules \textit{upgrade}$(T_{comp}, S)$.

\item 
At least one of $N',D'$ is smaller.
The planner adopts a smaller model $S'$, and schedules \textit{upgrade}$(T_{comp}, S')$
\end{myenumerate}

In cases where $N',D'$ can no longer increase (i.e. $N'=D'=12$), only \textit{upgrade}$(T_{comp}, S)$ will be scheduled. 
\end{comment}

==> planner-io__Liwei_Guo_s_conflicted_copy_2022-11-10_.tex <==
% !TeX root = main.tex


\subsection{IO planning}
\label{sec:design:planning:io}
In this stage, \sys{} selects the \bt{}s for individual shards of the $(n\times m)$ submodel. %to load and pipeline them with computation. 
Without stalling the pipeline, it seeks those that maximize accuracy. %as the execution plan.
%\Note{TODO: use a figure, demonstrating AIB}

%\textbf{Design points}
%\begin{myitemize}
%	\item 
%	Problem formulation: find an optimal $S$ set, s.t. $R(k) + S \to R'(n, d)$, 
%	Goal: $R'$ achieves maximum accuracy.
%	Two constraints: not exceeding T, no computation starvation \Note{XXX}. 
%
%	\item 
%	Solution: AIB + heuristic-based online shard allocation 
%	
%	\item 
%	AIB: formulate the constraints to mechanize the layerwise planning => AIB(n) $\to$ 0, AIB(n) $\geq$ 0. 
%	To allocate, substract corresponding AIB(n). Give Example. 
%	
%	\item
%	Allocation strategy design points:
%	\begin{itemize}
%		\item 
%		Num > Fidel. 
%		The implication is the engine prioritizes filling up the submodel (\Note{should compute planning gauge the delta? set a minimum ddl = 12x12 2-bit shard?}). %\Note{what if shard buffer too small? and submodel too large to be loaded?}
%		It then will consider upgrading others. 
%		
%		\item 
%		Important shards first. 
%		Progressively upgrade $K$ shards to a higher fidelity, then proceeds to next $K$ shards.  
%	\end{itemize}	
%\end{myitemize}

%To find an optimal IO scheduling of shards, the engine leverages the profiled shard importance and hardware capability to conduct an efficient, heuristics-based iterative search. 

\subsubsection{Problem formulation}
%\paragraph{Goal}
%\paragraph{Problem formulation}
Given the deadline $T$, $n \times m$ submodel $R$ determined by compute planning, and the preload buffer $S$, \sys{} plans for a shard configuration $S'$ to load during computation, s.t. 1) loading $S'$ does not stall the pipeline, and 2) $R=S+S'$ achieves maximum accuracy.


%\paragraph{Constraints}
%$S'$ is \textit{valid} if it does not stall the pipeline. 
%It satisfies the key data dependency constraint: before executing $k$-th layer, all shards of prior $k-1$ layers  must have been loaded to avoid starving computation.
%As a corollary, the total IO delay $\sum_{i=1}^{|S'|} T_{io}(S'_i)$ does not exceed deadline $T$. 

%Meanwhile, $S'$ is bound by two constraints: 
%1) total IO delay $\sum T_{io}(S'_i)$ does not exceed deadline $T$; 
%2) no stalling between layerwise computation. 

%\paragraph{Our idea} is to assign each $n$ layer an \textit{accumulated IO budget} (AIB) to encode the data dependency between across-layer shard loading and sequential layerwise execution, and iteratively selects shard fidelity based on their importance.

%\subsubsection{Tracking layerwise IO Budget}
\subsubsection{Accumulated IO budgets}
%The goal is to allow shards of $S'$ to be selected individually from different layers while ensuring they are valid, satisfying the planning constraints, i.e. $S'$ does not stall pipeline nor exceed $T$.
To ensure the planning $S'$ does not stall the pipline, \sys{} uses \textit{Accumulated IO Budgets} (AIBs) to track fine-grained, per-layer available IO . %i.e. $S'$ does not stall pipeline nor exceed $T$.
%The AIBs quantify IO budget the engine can consume \textit{prior to} execution of current layers.
%An AIB quantifies the IO budget the engine can consume to load \textit{all prior layers} execution of current layers.
%AIBs specifies the internal deadlines for each layer, under which the layer must have loaded its shards needed for execution. %which must have already loaded shards ready for execution, to avoid breaking the data dependency constraint. 
%An AIB specifies the internal deadline for each layer, which must have already loaded shards ready for execution, to avoid breaking the data dependency constraint. 
%\paragraph{Our idea} is to assign each $n$ layer an \textit{accumulated IO budget} (AIB) to encode the data dependency between across-layer shard loading and sequential layerwise execution, and iteratively selects shard fidelity based on their importance.

\paragraph{Key ideas}
%The engine uses AIBs to quantify the data dependency constraint as internal deadlines from each layer's perspective.
%The engine uses AIBs to track internal IO budgets of each layer, which bookkeep how much time the \textit{current} layer has to load all \textit{prior} shards.
%The engine uses AIBs to bookkeep how much time a layer has to load all \textit{prior} shards; 
%Our first idea is layerwise \textit{Accumulated IO Budgets} (AIBs). 
%To define AIBs which encode the data dependency of the pipeline, our observation is that the pipeline does not stall \textit{iff} before executing $k$-th layer, all shards of $0\dots k$ layers are loaded.
To quantify AIBs, our observation is that the pipeline does not stall \textit{iff} before executing one layer, all shards of the current \textbf{and} prior layers are already loaded.
We hence define AIBs as follows: %\textit{since the beginning}. 
%By doing so, the engine converts the planning constraints into AIBs: as long as each $AIB(k) \geq 0$, the planning satisfies the constraint and is valid.

\begin{definition}[Accumulated IO Budgets]
The AIB(k) of $k^{th}$ layer is the available IO time the layer can leverage to load all shards from $0\dots k$ layers, written as %to be the remaining time the layer still has to load all necessary shards. \xzlNote{a bit formal?}
$AIB(k) = AIB(k-1) + T_{comp}(k-1)$, where $T_{comp}(k-1)$ is the computation delay of the $(k-1)^{th}$ layer.
\end{definition}

The recursive definition (i.e. hence \textit{accumulated}) encodes the data dependency between pipeline layers: each layer crucially depends on previous layers' available IO budgets and computation delays for overlapping the loading of its shards;
for the very first layer, its AIB is set to be IO time of loading up the preload buffer $S$. 
For instance, AIB of the second layer is up to the AIB \textit{plus} the computation delay of the first layer, i.e. $AIB(1)=AIB(0)+T_{comp}(0)$. 
Since


%\begin{quote}
%%\xzlNote{AIB must be defined here. the intuition, etc.}
%%\paragraph{Definition}
%The AIB(k) of $k$-th layer is the available IO time the layer can leverage to load all shards from $0\dots k$ layers. %to be the remaining time the layer still has to load all necessary shards. \xzlNote{a bit formal?}
%
%\end{quote}

%\xzlNote{improve the following}
%AIBs for all layers to track how much time a layer still has to load all needed shards prior to its execution. 
%The intuition is $k$-th layer must finish loading necessary shards \textit{during} the execution of previous $k-1$ layers. 
%A positive AIB(k) therefore means the layer k still has 
Therefore, by checking if all AIBs are non-negative (i.e. each layer still has available IO time), \sys{} deems the planning S' \textit{valid} as it does not stall the pipeline.  %satisfies the constraint and is therefore valid.
%converts the planning constraints into AIBs: as long as each $AIB(k) \geq 0$, the planning satisfies the constraint and is valid.

The second idea is to consider the preload buffer $S$ as \textit{bonus} AIBs added to all AIB(k), unifying planning preloaded shards with that of the pipeline. 
AIB(k) is initialized to be the execution delays of all prior $(k-1)$ layers (hence ``accumulated'') plus the bonus AIBs provided by the preload buffer $S$. %the buffer is already preloaded, hence its IO is ``free''.
E.g. AIB(0) = 0 since loading any shards at the first layer incurs a compulsory pipeline stall; 
AIB(n-1) is the largest because it has all the time to load its shards during previous layers' executions.
Then, for each shard at $k$-th layer in the buffer $S$, its bonus AIB is added to AIB(k) and propagated to all subsequent layers. 
For instance, a shard at layer 0 from $S$ propagates its bonus AIBs to all AIB(k)s, k=$0\dots n-1$; 
the bonus AIB of a shard at layer 1 from $S$ is propagated to AIB(1) $\dots$ AIB(n-1), so long so forth. 
%of the last layer is the largest because it has all the time to load its shards during previous layers' executions.

To use, \sys{} initializes AIBs as described earlier, upon each planning. 
%Recursively, it accumulates AIBs of deeper layers from prior layers, i.e. $AIB(k) = AIB(k-1) + T_{comp}, k=1\dots n-1$.
%Figure~\ref{fig:design:aib} shows example AIBs for two layers, where $T_{comp}=1s$.
%Notably, $AIB(0)=T_{io}(S)=0.6s$, due to buffer $S$ is already preloaded, its IO being given as bonus to layer 0 and all subsequent layers, i.e. $AIB(1)=T_{comp} + T_{io}(S)=1.6s$.
%\xzlNote{the bonus budget is also added to AIBs of all subsequent layers}
%When the engine selects a shard at $k$-th layer, it deducts the shard IO from AIBs of $k$-th layer as well as all subsequent layers.
When \sys{} selects a shard at $k$-th layer, it deducts the shard IO from AIBs of $k$-th as well as all subsequent layers.
The is because loading such shards only affect \textit{yet-to-be-executed} layers but not the already executed ones. 
At the end of selection, \sys{} checks all AIBs to see if they are non-negative. 
If so, \sys{} deems the planning $S'$ valid, otherwise rejects it. 

%the planning constraints into AIBs: as long as each $AIB(k) \geq 0$, the planning satisfies the constraint and is valid.
%i.e. IO budgets not used up,
%AIBs track layerwise IO budget: whenever a shard at layer $k$ is to be selected, its IO will be deducted from $AIB(k)$ and from all AIBs of subsequent layers, i.e. $AIB(k+1), AIB(k+2), \dots, AIB(n)$. 
%To satisfy the constraint, the engine ensures at the end of selection, each AIB is above 0.


\begin{comment}
\paragraph{Key ideas}
%The engine uses AIBs to quantify the data dependency constraint as internal deadlines from each layer's perspective.
%The engine uses AIBs to track internal IO budgets of each layer, which bookkeep how much time the \textit{current} layer has to load all \textit{prior} shards.
%The engine uses AIBs to bookkeep how much time a layer has to load all \textit{prior} shards; 
%Our first idea is layerwise \textit{Accumulated IO Budgets} (AIBs). 
%To define AIBs which encode the data dependency of the pipeline, our observation is that the pipeline does not stall \textit{iff} before executing $k$-th layer, all shards of $0\dots k$ layers are loaded.
To quantify AIBs, our observation is that the pipeline does not stall \textit{iff} before executing one layer, all shards of the current \textbf{and} prior layers are already loaded.
We hence define AIBs as follows: %\textit{since the beginning}. 
%By doing so, the engine converts the planning constraints into AIBs: as long as each $AIB(k) \geq 0$, the planning satisfies the constraint and is valid.

\begin{definition}[AIBs]
The AIB(k) of $k^{th}$ layer is the available IO time the layer can leverage to load all shards from $0\dots k$ layers, written as %to be the remaining time the layer still has to load all necessary shards. \xzlNote{a bit formal?}
$AIB(k) = AIB(k-1) + T_{comp}(k-1)$, where $T_{comp}(k-1)$ is the computation delay of the $(k-1)^{th}$ layer.
\end{definition}

The definition is recursive, encoding the data dependency between pipeline layers: each layer crucially depends on previous layers' available IO budgets and computation delays for overlapping the loading of its shards. 
For instance, AIB of the second layer is up to the AIB plus computation delay of the first layer, i.e. $AIB(1)=AIB(0)+T_{comp}(0)$. 

%\begin{quote}
%%\xzlNote{AIB must be defined here. the intuition, etc.}
%%\paragraph{Definition}
%The AIB(k) of $k$-th layer is the available IO time the layer can leverage to load all shards from $0\dots k$ layers. %to be the remaining time the layer still has to load all necessary shards. \xzlNote{a bit formal?}
%
%\end{quote}

%\xzlNote{improve the following}
%AIBs for all layers to track how much time a layer still has to load all needed shards prior to its execution. 
%The intuition is $k$-th layer must finish loading necessary shards \textit{during} the execution of previous $k-1$ layers. 
%A positive AIB(k) therefore means the layer k still has 
Therefore, by checking if all AIBs are non-negative (i.e. each layer still has available IO time), \sys{} deems the planning S' \textit{valid} as it does not stall the pipeline.  %satisfies the constraint and is therefore valid.
%converts the planning constraints into AIBs: as long as each $AIB(k) \geq 0$, the planning satisfies the constraint and is valid.

The second idea is to consider the preload buffer $S$ as \textit{bonus} AIBs added to all AIB(k), unifying planning preloaded shards with that of the pipeline. 
AIB(k) is initialized to be the execution delays of all prior $(k-1)$ layers (hence ``accumulated'') plus the bonus AIBs provided by the preload buffer $S$. %the buffer is already preloaded, hence its IO is ``free''.
E.g. AIB(0) = 0 since loading any shards at the first layer incurs a compulsory pipeline stall; 
AIB(n-1) is the largest because it has all the time to load its shards during previous layers' executions.
Then, for each shard at $k$-th layer in the buffer $S$, its bonus AIB is added to AIB(k) and propagated to all subsequent layers. 
For instance, a shard at layer 0 from $S$ propagates its bonus AIBs to all AIB(k)s, k=$0\dots n-1$; 
the bonus AIB of a shard at layer 1 from $S$ is propagated to AIB(1) $\dots$ AIB(n-1), so long so forth. 
%of the last layer is the largest because it has all the time to load its shards during previous layers' executions.

To use, \sys{} initializes AIBs as described earlier, upon each planning. 
%Recursively, it accumulates AIBs of deeper layers from prior layers, i.e. $AIB(k) = AIB(k-1) + T_{comp}, k=1\dots n-1$.
%Figure~\ref{fig:design:aib} shows example AIBs for two layers, where $T_{comp}=1s$.
%Notably, $AIB(0)=T_{io}(S)=0.6s$, due to buffer $S$ is already preloaded, its IO being given as bonus to layer 0 and all subsequent layers, i.e. $AIB(1)=T_{comp} + T_{io}(S)=1.6s$.
%\xzlNote{the bonus budget is also added to AIBs of all subsequent layers}
%When the engine selects a shard at $k$-th layer, it deducts the shard IO from AIBs of $k$-th layer as well as all subsequent layers.
When \sys{} selects a shard at $k$-th layer, it deducts the shard IO from AIBs of $k$-th as well as all subsequent layers.
The is because loading such shards only affect \textit{yet-to-be-executed} layers but not the already executed ones. 
At the end of selection, \sys{} checks all AIBs to see if they are non-negative. 
If so, \sys{} deems the planning $S'$ valid, otherwise rejects it. 
\end{comment}


\input{fig-aib}

%By keeping each AIB above 0, i.e. IO budgets not used up, the engine ensures each layer satisfies the data dependency prior to execution, keeping IO busy and avoiding computation starvation.
%\Note{need better intuition}
%Under the deadline, each layer ensures 

%track individual usage...by respecting non-zero invariant...
%All layers must load their shards under respective AIBs to avoid breaking the constraint.
%have loaded its shards needed for execution. %which must have already loaded shards ready for execution, to avoid breaking the data dependency constraint. 

%\paragraph{Initialization}
%Each tiem when IO planning begins, the engine initializes the AIB(k) of $k$-th layer to be the execution delays of all prior $(k-1)$ layers (hence ``accumulated''), given by $AIB(k)=(k - 1)T_{comp}(l,d)$, where $k= 1\dots n$ and $T_{comp}(l,d)$ is a constant determined in compute planning stage (\S~\ref{sec:design:planning:compute}).
%It then inspects the preload buffer, calculates the IO delay $\Delta$ of loading the buffer, and adds $\Delta$ to each of AIB(k).
%%The rationale is to count $\Delta$ as ``free IO'' of the first layer to all AIBs, since the buffer is already loaded. 
%The rationale is, since the buffer has already been preloaded, its IO $\Delta$ can be counted as ``free IO'' towards the first layer (i.e. prior to execution), and can be accumulated to all subsequent AIBs. %since the buffer is already loaded. 
%For instance, the AIB of the very first layer is initialized to 0, i.e. $AIB(1)=0$, because there is no computation to overlap loading its shards, while the last layer has largest AIB $(n-1)T_{comp}$, all at its disposal to load its shards.
%Recursively, AIB(k) of $k$-th layer is defined as the AIB of the former layer (hence ``accumulated'') plus the layerwise computation delay, i.e. $AIB(k)=AIB(k-1) + T_{comp}(l,d), k=1 \dots n-1$. 

%is the time to load preload buffer of size $M$.

%\paragraph{Initialization} 
%To begin, the engine initializes AIBs from layer 0, and recursively to layer $(n-1)$. 
%Since for each layer the computation delay $T_{comp}$ is the same, AIBs are given by $AIB(n) = (n-1)T_{comp}$

\paragraph{Example}
Figure~\ref{fig:design:aib} shows a mini example of using AIBs to check the validity of $S'$, where it plans for a 2x3 submodel, targeting a 2s deadline with $T_{comp}=1s$.
The engine initializes AIBs recursively from L0, whose $AIB(0)=0.6s$ due to the three 2-bit shards in $S$.
%$AIB(1)=AIB(0)+T_{comp}=1.6s$
To plan, the engine first fills $S'$ with $S$, deducting $0.6s$ from both $AIB(0)$ and $AIB(1)$ because all shards in $S$ are in L0.
Since only L1 has spare AIB, the engine can only select shards for it.
We show three execution plan candidates A, B, and C.
In this case, both candidates A and B are valid because their AIBs are non-negative, meaning loading them does not stall computation L1. 
Yet, C is invalid, because $AIB(1)=-0.1s$, violating the constraint and stalling the pipeline.

%\Note{may not need}
%\paragraph{Why are AIBs effective?}
%Doing so urges the engine to respect data dependency: as IOs of earlier shards bill to directly to all subsequent layers, the engine must ensure by the time $k$ starts to execute it has spare IO to spend on loading its own shards..
%Like yearly fiscal budget?? (have a total spending budget  by the end of year, some saving in the beginning.. now needs to plan each month??)what is the analogy?
%The intuition of propagating the IO delays to later layers is the data dependency. 



\subsubsection{Selecting optimal shard versions}
For each $T$, there exist an enormous number of execution plans. 
The goal is to select an optimal configuration $S'$, which 1) is valid, and 2) maximizes accuracy.
For instance, both A and B in Figure~\ref{fig:design:aib} are valid, but which has the maximum accuracy?
%\textbf{TBD after exp.}


\paragraph{Key idea} 
%\sys{} follows two principles to generate an optimal execution plan: 
%1) to maximize accuracy, it attempts to increase \textit{average fidelity} and allocate full fidelities to a few most important ones; 
%2) to ensure validity, it respects the key invariant $AIB(k) \geq 0$ for each allocation attempt on layer $k$.
To ensure validity, \sys{} respects the key invariant $AIB(k) \geq 0$ for each allocation attempt on layer $k$.
%\xzlNote{guided by shard importance?.. and list 1-3 heuristics/principles}
To maximize accuracy, our key idea is to first uniformly increase \bt{}s for all shards, then with the rest AIBs it greedily and iteratively allocate highest possible \bt{}s to individual shards guided by shard importance.
%Our rationale for the allocation strategy is, by increasing the average fidelity, 
By doing so, we build an information passageway for most important shards, allowing their maximum activations to be preserved in highest fidelity as possible. 
% ... For instance, activations from 32bit shard incur more information loss on 2bit shard than a 6bit shard..
%By doing so, it builds a high-fidelity information passageway for most important shards, allowing their can provide maximum activations without
%increasing the average fidelity, 

The allocation process comprises two passes as follows.
In the first pass, \sys{} picks a uniform \bt{} for all unallocated shards in the submodel, i.e. those not in preload buffer.
%\Note{layerwise... select the shards from same layer..}
To do so, it enumerates from lowest \bt{} (i.e. 2-bit) and selects the highest \bt{}s while AIBs still satisfy the invariant.
Notably, it fills a submodel layer with the shards from the same original layer and does not mix up shards across layers, due to quantization preserves layerwise weight distribution (\S\ref{sec:design:sharding:quantize}).
If AIBs cannot even support 2-bit shards, e.g. due to $T$ and/or preload buffer $S$ too small, \sys{} still selects them as they are necessary for execution but aborts further allocation.
In the second pass, \sys{} iteratively upgrades the \bt{}s of individual shards to full 32 \bt{} guided by the shard importance profiled in \S\ref{sec:design:planning:pre}, until all AIBs are consumed. 

The allocation result is an optimal execution plan which instantiates the submodel with individual shard configurations, and is ready to be executed by the IO/compute pipeline.
%The planner then sends the plan to the IO/computation pipeline for execution. 

%\begin{myitemize}
%	\item 
%	Key points: 1) respect AIB > 0 constraint. 2) iterative allocation to most important shards. 
%	
%	\item
%	Heuristics
%	\begin{itemize}
%		\item 
%		Num > Fidel. 
%		The implication is the engine prioritizes filling up the submodel (\Note{should compute planning gauge the delta? set a minimum ddl = 12x12 2-bit shard?}). %\Note{what if shard buffer too small? and submodel too large to be loaded?}
%		It then will consider upgrading others. 
%		
%		\item 
%		Important shards first. 
%		Progressively upgrade $K$ shards to a higher fidelity, then proceeds to next $K$ shards.  
%	\end{itemize}	
%\end{myitemize}
%
%\paragraph{tradeoffs between \# of shards vs fidelity}
%The trade off is whether we want the majority of shards to be medium-to-low fidelity or we want to the majority to be low while some (important) to be high....
%Our idea is the latter. 
%Evidence: 3-bit full model has 91.4\% while 2-bit version with only 5 shards upgraded to 6-bit achieves 91.6\% accuracy...
%
%
%\paragraph{the case of 32-bit shard}
%It is a special case (uncompressed)... 
%\sys{} upgrades to 6bit and refrains from 32-bit, unless all other shards have been upgraded to 6 bits ...  
%This is because 32-bit is not cost effective ... due to the outstanding performance in 4-bit version which achieves <1\% accuracy loss.. 
%Comparing to upgrading one 32-bit shard, one may upgrade 8 more 4-bit shard...which has more impacts on accuracy... evaluation (?) shows evidence..
%
%\xzlNote{below obsoleted?}

\begin{comment}
The planner then allocates shard configurations for the scheduled tasks. 
It follows the heuristics: 

\begin{quote}
	\textit{Heuristics II: prioritize top layers and important shards.}
	The planner favors more ``important'' shards and layers.
\end{quote}

The planner allocates shards in a greedy manner: it starts from the top layers (i.e. closer to output) and allocates highest quantized precision (i.e. 6-bit) to more important shards, that is, shards that are more sensitive to accuracy. 
This is shown in the listing XXX to YYY lines...

The planner does so iteratively for every shard until $T$ specified in the scheduled tasks is used up, i.e. by subtracting $T$ with $T_{io}(B)$ for an individual shard in $B$-bit precision.
The planner then generates a list of IO tasks, each specifies loading a shard $s(N,D,B)$ into $N$-th index of $D$-th layer in $B$-bit, of the model.

Before issuing these IO tasks, the planner does a sanity check: whether they will stall the pipeline and exceed $T$. 
If so, the planner decreases the precisions of shards which stall the pipeline.

As we will show in \sect{eval}, the planning is efficient taking only XXX ms and can ramp up accuracy fast with the help of our heuristics.

%\Note{merge below heuristics}
%\begin{myitemize}
%	\item 
%	More bits to top layer (closer to output), less to bottom layers (closer to input). 
%	Two benefits: 1) higher accuracy, see ``are all layers created equal'' and preliminary results; 2) faster start, i.e. the 1st layer (bottom layer) is blocking (no compute overlapping), better reduce io as much as possible.
%	
%	\item 
%	Shard configuration per layer: some shards have better sensitivity than other, favor them...
%	
%\end{myitemize}

\Note{TODO: merge below}
\paragraph{Spare IO}
\Note{do not mention embedding, defer to S6}
\Note{IO budget vs spare IO}
We define spare IO as the amount of IO time that can be spent on loading model shards; 
it overlaps with compute, exploiting the missed opportunity (\S~\ref{sec:motiv:char}).
Given a deadline $T$, the spare IO is calculated via a simple formula $T_{spare} = T - T_{emb}$, where as $T_{emb}$ is the amount of time spent retrieving embedding vectors. 
While embedding table is in-memory, $T_{emb}$ is negligible (i.e. $<10$ms), and we can regard $T_{spare} \approx T$.

\paragraph{IO tasks} 
With spare IO $T$, there are two IO tasks. 
\begin{myitemize}
	\item 
	$\text{\textit{append}}(T, S, S')$ loads a shard set $S'$ and appends them to the existing shards $S$ in $T$ time, s.t. the model computes on \textit{more} shards.
	
	\item 
	$\text{\textit{upgrade}}(T, S)$ replaces existing shards $S$ in $T$ time, s.t. the model computes on \textit{higher-precision} shards.
\end{myitemize}


\paragraph{Toy examples} 
For the very first (cold) inference, the planner is given $T=500ms$. 
It subtracts $500ms$ with $T_{emb}$ and finds $T_{spare}=400ms$.
Since none shard has been loaded yet (i.e. $S=\emptyset$), the planner only schedules \textit{append} task, adding shards to the empty model.
In the second (warm) inference, the same $T=500ms$ is given and a similar $T_{spare}$ is found.
Since the model can execute on shards $S$ loaded by the first inference, the planner leverage $T_{spare}$ to schedule \textit{upgrade} to improve their precisions, hence model accuracy.
\end{comment}

%\Note{to merge}
%\sys{} profiles time for an IO and compute on the corresponding platform in an offline fashion, out of the execution path of the inferences. 
%For IO, the system measures the latency of loading an uncompressed shard from storage and derives the latency for the compressed shards, which is linear to their bitwidths.
%%from the uncompressed latency, the system derives IO time of compressed shards, which is linear to their bitwidths.
%For Compute, the system does a dry run with different number of heads and measures the layerwise latency. 
%The rationale of profiling IO and Compute offline is they are data-independent~\cite{driverlet,asymo,tinystack}, whose latency hence is deterministic at run time. 
%both model loading and NN inference depends , 
%execution is solely dependent on the NN model itself. 


\begin{comment}
\paragraph{Reshaping resident model}
\Note{reshaping models...}
The planner compares the new model structure $(N',D')$ with existing $(N,D)$ (note that an empty model of cold inference can be denoted by $(0, 0)$). 
As described, compute planning causes the model structure to grow monotonically with $T_{comp}$. 
Hence there are three cases:
\begin{myenumerate}
\item 
At least one of $N',D'$ is larger.
The planner calculates shard set $S'$ to load and schedules \textit{append}$(T_{comp}, S',S)$, where $S'$ contains the indexes $(n,d)$ of new shards but not their $b$-bit precisions.

\item
Both $N',D'$ are the same as $N,D$.
The planner does not change the existing model $S$, and hence only schedules \textit{upgrade}$(T_{comp}, S)$.

\item 
At least one of $N',D'$ is smaller.
The planner adopts a smaller model $S'$, and schedules \textit{upgrade}$(T_{comp}, S')$
\end{myenumerate}

In cases where $N',D'$ can no longer increase (i.e. $N'=D'=12$), only \textit{upgrade}$(T_{comp}, S)$ will be scheduled. 
\end{comment}

==> planner-pipeline__Liwei_Guo_s_conflicted_copy_2022-11-13_.tex <==
% !TeX root = main.tex
\subsection{Submodel execution}
\label{sec:design:planning:pipeline}

%\input{fig-res-model}

%Despite \sys{} partitions the model into shards, it still executes the plan (submodel) in a layerwise, pipelined manner from layer 0 to layer n-1.
\sys{} executes the plan (i.e. submodel with selected shards) in a layerwise, pipelined manner from layer 0 to layer n-1.
While conceptually it is possible to pipeline shard computation within the same layer, \sys{} does not do so due to limited benefits -- within a layer there exists data dependency between the FFNs and attention module, where FFNs must wait for an aggregated attention output to execute. 
%This is because although attention heads can be computed individually, FFN neurons must wait until all shards are loaded to execute. 
%Hence it does not pipeline loading and execution of individual shards because 

\sys{} executes both IO and computation as fast as possible;
it does not reorder the loading of individual shards in order to meet data dependency between execution, because by design AIBs have already ensured so.  
To compute, \sys{} decompresses the shards into the working buffer using the dictionaries stored along with them;
the working buffer is enough to hold one layer of FP32 weights and shared by all layers during their ongoing execution. 
After execution, \sys{} evicts loaded shards from top to bottom layers until preload buffer is filled. 
It does so because shards at bottom layers (i.e. closer to input) are needed early during inference.
Preserving as many of them as possible avoids compulsory pipeline stalls in early stages.
%Bottom layer to top layers, because bottom layers are first needed during inference...
%
%\textbf{Key points}
%\begin{myitemize}
%	\item 
%	\xzlNote{compress \& move to S3 ``overview''}
%	How to execute: Overall layerwise, load shards specified in exec. plan and overlap computation.
%%	By design the first layer is already in buffer. 
%	Why layerwise not shard-wise? data parallelism is limited in small amount of data.
%	
%	\item 
%	No need to re-order IO because data dependencies have been respected during IO planning through AIBs.
%	
%	\item 
%	Computation includes decompression + compute on 32-bit weights, shown in Figure~\ref{fig:design:pipeline}.
%	Decompression -- fast, can be done concurrently. 
%	Further acceleration is possible~\cite{gobo}.
%	
%	\item 
%	After execution, evict loaded shards from submodel until $M$ is reached. 
%	Bottom layer to top layers, because bottom layers are first needed during inference...
%\end{myitemize}



==> planning-flow.tex <==
% !TeX root = main.tex

\textbf{Key theme:} how to leverage spare IO (IO budget) for maximizing  the model accuracy.
Structure the section around the idea....

\textbf{Flow of the section:}
\begin{myenumerate}
	\item 
	\textbf{Problem formulation.} 
	A search problem: given a deadline $t$, existing loaded shard $s$, decide what shards to overlap with compute during this immediate inference.
	
	\item
	\textbf{Key question:} how to maximize the accuracy? 
	
	Key challenges are: 
	1) complex tradeoffs between accuracy vs shard configurations.. While it is true more and/or higher-precision shards increase the accuracy, some shards have larger impacts on accuracy.. 
	2) exponential search space.. Search can not all be done ahead of time, due to it must consider runtime loaded shards. 


	\item 
	\textbf{Our key ideas for the online planner are as follows.}
	\begin{myitemize}	
		\item
		First, identify \textit{spare IO}, an IO budget: $io_{spare} = t - io_{emb}$. \Note{Note spare IO is our new, core idea}.
		With the spare IO, there are two IO tasks to do: \textit{append} and \textit{upgrade}.
		
		Give two examples on spare IO and two tasks: 1) full cold inference (append), 2) warm inference (upgrade). 
		
		\item 
		Second, IO task planning. 
		Two key steps: 
		\begin{myenumerate}
			\item 
			\textbf{Compute planning.}
			Key idea: let compute bound deadline for maximizing accuracy. 
			Decide IO tasks based on spare IO (calculate model structure, schedule IO tasks accordingly);  
			
			 
			\item 
			\textbf{IO planning.} 	
			Heuristics-guided shard allocation. Overall greedy, but will prioritize layers/shards with higher importance (done at an offline stage). 
			Describe the heuristics and present the algorithm in full.
			\Note{more details in slides}		
		\end{myenumerate}

		\item 
		Third, issue IO tasks. Do not need to completely re-order them; explain why in-order might just be fine (the data dependency exists for each layer of the pipeline, unlike CPU instructions -- out-of-order executed ones have no dependency XXX). Check constraint: stalling will not exceed deadline. 
	\end{myitemize}
	
	\item 
	To obtain the platform io/compute capability and shard importance, which are needed by the algorithm. 
	We conduct offline profiling, which is out of inference critical path:
	\begin{myitemize}
		\item 
		We measure:	IO: disk access delay for loading one shard in $b$ bits, $b=2,3,4,5,6$; 
		Compute: how many ms for computing on $w$ shards? Total inference latency can be deduced by multiplying it by number of layers $d$
		
		\item 
		We enumerate shards/layers to figure out which are most sensitive to accuracy. Mark them..
	\end{myitemize}	

	\item 
	Handling misc. parameters. 
	Those are not part of model shards but essential for inference, including layer normalization, pooler, and head for the downstream task. 
	These are small enough to be loaded once in fixed precisions. 
	
\end{myenumerate}

==> prelim-explore.tex <==
% !TeX root = main.tex
%\subsection{Model compression is inadequate}
\subsubsection{Design space exploration}
\label{sec:motiv:design-explore}
%\textbf{Carefully discuss: can existing models/methods fit into our approach of overlapping IO vs Compute}

\textbf{TODO: review the complete landscape of weight sharing status of supertransformers}

%\textbf{Discuss the IO/Compute task in model compression techniques which reduce latency}

\textbf{Does early exit have a place here?}

Towards reducing cold inference latency of transformer, we set to overlap IO with Compute and take into account the architectural differences of different platforms. 
We explore the following designs. 

\input{fig-design-explore}

\input{fig-io-compute}


\paragraph{Why Post-training Quantization?}

There are two quantization techniques: quantization-aware training (QAT) and post-training quantization (PTQ). 
We set for the latter (PTQ) for two key benefits:
1. faster deployment. 
PTQ does not require to fine-tune the pretrained models on downstream tasks, which is time-consuming, e.g. one epoch takes a few hours on a GTX1080 Ti GPU~\cite{XXX}.
2. better data privacy.
As QAT fine tunes the model, it needs access to the whole training set, which is often not accessible due to privacy and proprietary concerns. 


\paragraph{Can we pipeline transformer layers as-is?}
As described in \sect{motiv:primer}, transformer models are stacked in layers. 
A naive approach is to take a transformer model as-is (e.g. BERT~\cite{bert}) and pipeline the compute of one layer with IO of \textit{next} layer. 

The design is shown in Figure~\ref{fig:motiv:overlap}.
While being intuitive, unfortunately, this approach barely reduces the latency: due to the disproportionate IO vs Compute time of a transformer, e.g. IO time is 6$\times$ larger than Compute on Odroid, pipelining them as-is incurs large pipeline stall, rendering it ineffectively. 
\sect{eval} will present a quantitative evaluation.

\paragraph{How about pipelining compressed layers?}
To mitigate large pipeline stalls, one may want to compress the layers instead of pipelining them as-is, which brings the IO vs Compute time closer.
Figure~\ref{fig:motiv:compress-overlap} shows the idea.

We consider the following compression techniques.
\begin{myitemize}
	\item 
	\textit{width reduction}, which can be either static~\cite{distilbert} or dynamic~\cite{dynabert}.
	However, to fully close the gap between IO vs Compute, both MHA and FFN feature dimensions need to be compressed significantly. 
	For instance, per our measurement on Odroid in Figure~\ref{fig:motiv:io-compute}, they need to be compressed by 4$\times$ -- from 768 to 192, 3172 to 793. 
	Later we show in \sect{eval} that the compression greatly limits the expressiveness of a transformer block and leads to persistent performance degradation (XX\% in SQuad for same number of layers), even for hot inference. 
	
	\item
	Other techniques such as quantization~\cite{q8bert,tenarybert}, low-rank matrix factorization~\cite{groupreduce} share the same drawback: it requires to compress a full layer to close the IO vs Compute gap; 
	the inferior performance is persistent. 
\end{myitemize}

\paragraph{Design implication:}
Coarse-grained layerwise pipelining won't work for either uncompressed or compressed;
persistent performance degradation is undesirable.
\Note{the key is not to do layerwise pipelining -- but finer grained, attention head wise pipelining.}

\begin{comment}
\Note{merge below -- note the idea of overlapping is not introduced yet, whether it is dynamic or static does not matter...}
While \textit{cold inference} receives only scant attention in literature, there are a primary body of work targeting at reducing \textit{inference} latency using model compression: by making the transformer model parameter- and compute-efficient, its IO and Compute time can thus both be reduced.

%\Note{why static vs dynamic matters}
%One may compress a transformer model to make it parameter- and compute-efficient, thus reducing both the IO and Compute time. 

To this end, common compression techniques include reducing model depth~\cite{distilbert} and/or width~\cite{mobilebert}, quantization~\cite{q8bert,tenarybert}, low-rank matrix factorization~\cite{groupreduce}, weight sharing~\cite{albert}.
Compression can also be dynamic and adaptive. 
For instance, each sentence can have a subtransformer/subnet with smaller width and depth~\cite{dynabert,layerdrop}; 
even for individual tokens, they can have different depths~\cite{spatten,ltp}. 

\paragraph{Missed opportunities.}
While being effective, model compression alone is inadequate: 

\textit{Does not overlap IO vs Compute.} 
It still waits for the full model loading completion before continuing. 
Despite the compressed models are a few times smaller than the original, IO is still the key bottleneck.
For instance, Distilbert is 4$\times$ smaller than BERT, but still taking 3 seconds in IO task. 

\textit{Poor performance.} 
Esp. for static model compression -- the performance is consistently low, compared with a full model. 
To make it worse, if one wants to reduce the IO time significantly, he has to make the model 4$\times$ narrower in MHA and includes only 2-3 layers. 
This greatly limits the expressiveness of MHA~\cite{XXX}.


\paragraph{What about \textit{static} model compression?}
One may statically compress BERT, e.g. via simplified structure~\cite{distilbert,mobilebert}, quantization~\cite{q8bert,tenarybert}.
To fit in our scenario, one may compress a layer such that its IO overlaps with Compute. 

This approach faces a key drawback of poor performance.
To overlap, it requires large compression ratio per layer. 
We show the IO/Compute vs transformer layer compression ratio in Figure~\ref{fig:motiv:io-compute}.
To effectively overlap IO with Compute, one needs to compress both dim and hidden dim so that IO may meet compute.
E.g. for Odroid, they need to be compressed by 4$\times$ -- from 768 to 192, 3172 to 793. 
The compression greatly limits the expressiveness of a transformer block and leads to performance degradation (even for hot inference). 
\Note{key argument: at the end, there is only one model in which you can overlap IO/Compute at the cost of bad performance}



\paragraph{What about \textit{dynamic} model pruning?} 
It selects a part of model parameters (subnet) from a supernet at inference time. 
There are two directions along the selection depth and width.
\begin{myitemize}
	\item \textbf{Depth}. 
	\cite{layerdrop,universal-transformer,edgebert} adaptively change the number of layers at runtime.
	
	\item 
	\textbf{Width}. 
	\cite{dynabert,hat} adjusts the width by varying the feature dimensions of attentions and FFNs. 
	%number of attention heads and neurons an FFN layer, i.e. leftmost attention heads and FFN neurons.
%		~\cite{dynabert} adjusts width by varying the number of attention heads and neurons an FFN layer, i.e. leftmost attention heads and FFN neurons.
\end{myitemize} 

The key drawbacks are: 
1) a width/depth is selected at each inference time, forming a subtransformer.
subtransformers are independent and disconnected from each other -- this does not solve cold inference because the model is always loaded fresh.
Some networks have shared weights, e.g. \cite{hat} shares FFN, \cite{dynabert} shares important attention heads and neurons in FFN;
ad hoc optimization helps accelerating loading shared parameters, but the reduction is minor (compared with).
2)\Note{Merge below}
key argument: some dynamic networks exploit the weight sharing opportunities of a supernet and its subnets but not all; the weight sharing decision is ad hoc and is not tied to hardware.
\end{comment}

% Below useful about Dynabert 
\begin{comment}
The implication is one may incrementally load parameters from subnets of the mentioned supernets;
starting from the smallest width and depth, the parameters can be gradually loaded and become the whole model.


Back of envelope calculation, $m_w, m_d$ as width and depth multiplier:

Let $m_w = \frac{1}{12}, m_d=1$. 
The pipelining strategy being load one attention head at a time. 
Load one layer takes $320ms/12 \simeq 30ms$. 
Compute on one head takes roughly same time, i.e. $30ms$, 12 full heads takes $50ms$.
This case the IO and Compute overlaps well. 
W/o considering word embedding, end-to-end latency is $30+30*12=390ms$. 
Doing this for 11 more inferences we can achieve the accuracy of $m_w=1, m_d=1$.
	
On accuracy -- on a 3-head subnet, the SST accuracy seems quite high ($91 \sim 92$), which is higher than all-shared albert. 

A challenge might be: how to choose overlapping strategies for different platforms, where the IO vs Compute is different. 
Odroid (our platform) is an ideal, coincidental case -- we can load one full slice of attention head \& FFN per time.
What if IO is slower? I.e. cannot fully load the slice within the compute boundary. 
Can our system adjust overlapping strategy? 
For instance, load one slice of attention, share its weights with FFN.
\end{comment}

\begin{comment}
\Note{bewlow for completeness, can omit}
\paragraph{Why not offload to cloud?}
This work focuses on \textit{on-device} inference.
We discuss \textit{cloud offloading} as an alternative approach for completeness.
Cloud offloading~\cite{deepcod,edgepipe} trades off the cost of compute and model loading of cold inference for network latency, where the inference is always hot in the cloud. 

%We do not aim to settle the debate which is better.
First, offloading is complementary.
It is valuable when applications need strong results because cloud is more computationally-capable. 
This does not diminish the need for on-device inference. 
Second, on-device inference guarantees (stable?)lower latency (better QoS?). 
Mobile networks are often spotty with fluctuating latencies;
in contrast, on-device NN inference latency is almost stable/deterministic due to the workload nature of matrix multiplications. 
Third, on-device inference offers higher privacy assurance, because data is never uploaded to the cloud. 
It has become increasingly popular\Note{cite}.

%If we do cloud offloading, the latency is largely bound by network roundtrip time (tens of ms), assuming a serving scenario in the cloud (more computationally-capable);
%larger models are deployed in the cloud, as well.
\end{comment}



==> prior.tex <==
% !TeX root = main.tex

\section{Accomplished work from the student}

\textbf{Liwei Guo} is a 6-th year Ph.D. student of the Computer Science Department at University of Virginia (UVA).
He was a direct Ph.D. student of the school of Electrical and Computer Engineering at Purdue University and transferred to UVA from Purdue with his advisor Prof. Felix Xiaozhu Lin in his 5th year. 

He has been focusing on making edge devices more efficient and secure, using a systematic and principled approach. 
To this end, his prior work took the angle of kernel softwares, including redesigning kernel structures~\cite{transkernel,psbox}, refactoring the storage stack~\cite{enigma,overwatch}, and reusing mature drivers via record-and-replay~\cite{driverlet}.
His work has been seen on premier systems venues such as Eurosys~\cite{psbox,driverlet} and USENIX ATC~\cite{transkernel}. 

Complementary to his prior work, the proposed project takes the angle of user software and case studies an important NLP user application, i.e. Transformer.
Together with his prior work, the proposed project completes his thesis (i.e. making edge devices more efficient and secure) in a holistic manner, covering both kernel and user software. 
 

==> recycle-next.tex <==
% !TeX root = main.tex

\subsection{Next steps}

==> recycle-prelim.tex <==
% !TeX root = main.tex

\subsection{Preliminary experiments}
\label{sec:motiv:char}

We have done the following preliminary experiments which support our design choice. 

\input{prelim-char}

\input{prelim-explore}

==> tab-eval-distilbert.tex <==
% !TeX root = main.tex

\begin{table}
	\centering
	\begin{tabular}{llllll} 
		\hline
		& SST-2 & RTE  & QNLI & QQP &  Time (s) \\ 
		\hline
		Vanilla-Distil & 91.3  & 59.9 & 89.2 & 88.5  &  >3
	\end{tabular}
	\caption{Vanilla DisilBERT results. It takes over 3s to finish execution on both Odroid and Jetson due to large IO. 
	It fails to meet all target latencies due to its size is not configurable.}
	\label{tab:eval:distil}
\end{table}

==> tab-shards-size.tex <==
% !TeX root = main.tex

\begin{table}[h!]
	\centering
	\begin{tabular}{llllll} 
		\hline
		Fidel. ver. (bit) & 2     & 3     & 4    & 5    & 6     \\ 
		\hline
		Comp. ratio ($\times$)   & 15.66 & 10.52 & 7.92 & 6.35 & 5.30 
	\end{tabular}
	\caption{SST-2 model compression ratios at different fidelities (0.15\% outliers).
	Others have similar compression ratios (CoLa, RTE outliers: 0.14\%, QQP outliers: 0.17\%).}
\label{tab:eval:shard-size}
\end{table}

==> thoughts.tex <==
% !TeX root = main.tex

\section*{Thoughts}

\paragraph{Benefits of being retraining free}
No need to fine tune, which is time-consuming. 
Does not need access to training data, which is often private and proprietary. 
\Note{needs to be careful about this:} we cannot do arbitrary pretrained model. Need to use dynabert as a backbone network. 


\paragraph{What are key innovations?}
The key contribution of \sys{} is: 
1) it identifies the model shards which have elastic IO time, as the proper building block for the IO/compute pipeline of transformer inference \Note{novel approach for constructing the elastic pipeline};
2) based on model shards, it proposes a novel planning algorithm that maximizes the inference accuracy while meeting a user-set deadline on different devices.

We do not claim: 1) quantization techniques used to generate shards, and 2) IO/compute pipeline as our contribution since these techniques are well-known. 

\paragraph{How does the IO/compute pipeline work with shards?}
The number of shards per layer can be regarded as the ``width'' of the \tfm{} model during an inference;
it is the same across all layers during one inference.
Prior to each inference, \sys{} decides how many shards and the bitwidth of each shard to be used, depending on the deadline and device-specific IO/compute capability. 
For one inference, \sys{} constructs the IO/compute pipeline in the following way: it first loads the initial set of shards for layer 1; it then begins computing on shards of layer 1, while overlapping shard loading for layer 2, and so on and so forth.

\paragraph{Why do partial model composed of shards give meaningful results?}
Because of the parameter redundancy of \tfm{} models: 
a \tfm{} model may still give meaningful results even if attention heads are reduced from full sixteen to a few~\cite{16heads}, or layers share the same set of parameters~\cite{albert}. 
In \sys{}, one shard is a vertical slice of the transformer layer, comprising one attention head plus a set of FFN neurons; 
it preserves the structure on which the model is trained and the learned features. 
By stacking them in layers, the resultant model resembles a partial model with a smaller width~\cite{dynabert, liDynamicSlimmableNetwork2021}, hence still giving meaningful results.



\paragraph{\sys{} seems a generic model compression technique, why target cold inference only?}
To clarify: the model compression technique used by \sys{} is not new~\cite{gobo};
it acts only as an enabling tool for \sys{} to generate shards as the IO/compute pipeline building block.

\sys{}'s key ideas are tailored to cold inference due to the deadline constraint, where IO is the bottleneck.
The compression, however, does not affect compute time w.r.t. a full-precision model.
It hence has little benefits in a hot inference scenario, i.e. same latency but inferior accuracy than a full-precision model.

\paragraph{Can a GPU help reduce cold inference latency?}
No. 
This is because during cold inference, IO is the bottleneck, dominating over 90\% of the latency.
By simply offloading the compute to GPU, the IO keeps blocking compute and still results in high cold inference latency.

\paragraph{Why not offload to cloud?}
First, on-device inference ensures better privacy. 
The query as well as content being queried (e.g. medical records) do not have to be exposed to cloud.
Second, it is more reliable where spotty network connections are common on mobile devices~\cite{livelab,backgnd-in-wild2}.
Third, cloud offloading is a complementary approach, e.g. for other non-private queries, the user can always offload to cloud.

\paragraph{Can we leverage idle intervals between IPA interactions to load model?}
This is an orthogonal approach.
The idea is to prefetch the model file prior to inference.
Its challenge is twofold: 1) it is unclear how well IPA invocations can be predicted, while misprediction leads to excessive memory usage and poor user experience.
2) coordinating with other apps which compete for memory may be challenging, e.g. the already prefetched model file may be swapped out due to contention.


\paragraph{Why sacrifice accuracy for latency?}
Because in the scenario we target, reducing the latency from seconds to milliseconds significantly improves user experience.
Meanwhile, the accuracy loss is only 1\%, which is considered negligible in NLP literature~\cite{albert,nagarajanOptimizingTransformersApproximate}.
Prior study on IPAs~\cite{tsaiFasterResponsesAre2019} support our design, advocating ``faster responses are better responses''. 

==> todo.tex <==
% !TeX root = main.tex

TODO: 
1. decompession time... not universal. depending on bitwidth
2. our use of board.. pretty wimpy. so our target delays are higher than prior work (edgebert which uses jetson...)


\Note{High level ideas}
\begin{myitemize}
	\item 
	Memory-resident model. 
	A high level ``specification'' -- depths \& widths. 
	
	\item 
	Resource-elasticity. Can respond to 
	1. diff. latency constraint (thru tuning specification); 2. diff. memory constraints: deflating/inflating like VMM memory balloon.
\end{myitemize}



\Note{Thoughts on spare IO:}
The key theme of \sys{} is how to leverage the spare IO, which is the key missing component in prior work.
Cold inference problem is a only small entry point -- because it does not leverage spare IO, it suffers from long delay.

``Resource-elastic'', tied to IO (key difference, an IO planner)
In-memory state transformer -- give bits to different parameters, depending on spare IO or not, can upgrade or throw away accordingly. 

Do not have to consider model always in memory -- our solution provides a middle ground in between

\Note{selection of quantization granularity}
Weird for odd-bit? E.g. 3-bit seems rarely used.
May use 2,4,8,16? Albeit more coarse-grained.
But keep in mind this ties to the pipeline elasticity and should fit what the device needs (what its io/compute capability is)


\Note{STI reconciles accuracy with latency...}

\Note{todo:} make a case for suboptimal accuracy during first inferences

\Note{Critical vs non-critical path:}
Critical path (i.e. during during inference): 
1. overlap io/compute. 
2. for those do not have compute or multiple stages to overlap (e.g. embedding) -- minimize io (e.g. fixed-precision embedding). 

non-critical path (i.e. background thread) can allow for some  extra work. 
Examples include:
1. embedding matrix update. 
Based on frequency, update the corresponding block positions.
2. shards upgrade.
Existing already loaded shards can be replaced by full-precision. 


